GraphMini: Accelerating Graph Pattern Matching Using Auxiliary Graphs

Graph pattern matching is a fundamental problem encountered by many common graph mining tasks and the basic building block of several graph mining systems. This paper explores for the first time how to proactively prune graphs to speed up graph pattern matching by leveraging the structure of the query pattern and the input graph. We propose building auxiliary graphs, which are different pruned versions of the graph, during query execution. This requires careful balancing between the upfront cost of building and managing auxiliary graphs and the gains of faster set operations. To this end, we propose GraphMini, a new system that uses query compilation and a new cost model to minimize the cost of building and maintaining auxiliary graphs and maximize gains. Our evaluation shows that using GraphMini can achieve one order of magnitude speedup compared to state-of-the-art subgraph enumeration systems on commonly used benchmarks.

==> algorithms-old/build_mini_graph.tex <==
\begin{algorithm}
    \caption{BuildMiniGraph}\label{algo:buildMiniGraph}
    \begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input: } $D, S$\\
    \hspace*{\algorithmicindent} \textbf{Output: } $G_{min}$
    \end{flushleft}
    \begin{algorithmic}[1]
    \Function{buildMiniGraph}{D, S}
    \State $G_{min} = empty$
    \State $i = 0$
    \State $G_{min} \! \rightarrow \! dataPos.set(i) = 0$
    \For{$u \in D$}
        \State $N_{new}(u) =  S \cap N(u)$
        \State $G_{min} \! \rightarrow \! data.append( N_{new}(u) )$
        \State $G_{min} \! \rightarrow \! dataPos.set(i+1) = |N_{new}(u)|$
        \State $i = i + 1$
    \EndFor
    \State \Return $G_{min}$
    \EndFunction
    \end{algorithmic}
\end{algorithm}



==> algorithms-old/cache4clique.tex <==
\begin{algorithm}
    \caption{\cache{} 4Clique Count}\label{algo:cache4clique}
    \begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input: } graph $G(V, E)$\\
    \hspace*{\algorithmicindent} \textbf{Output: } 4cliqueNum
    \end{flushleft}
    \begin{algorithmic}[1]
    \Function{Count4Clique}{G}
    \State $s \gets 0$
    \State $V_1 = V$
    \For{vertex $v_1 \in V_1$}
        \State $V_2 = N(v_1)$
        \State $G_{min} = empty$
        \For{$v_3 \in N(v_1)$}
            \State $T(v_3) = N(v_1) \cap N(v_3)$
            \State $G_{min}.add(v_3, T(v_3))$
        \EndFor
        \For{ $v_2 \in V_2$}
            \State $V_3 = G_{min}.get(v_2)$
            \For{$v_3 \in V_3$}
                \State $T(v_3) = G_{min}.get(v_3) $
                \State $V_4 = V_4^2 \cap T(v_3)$
                \State $s = s + |V_4|$
            \EndFor
        \EndFor
    \EndFor
    \State \Return $s$
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> algorithms-old/cacheq2.tex <==
\begin{algorithm}
    \caption{ Mini-Graph Q2 }\label{algo:cacheq2}
    \begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input: } graph $G(V, E)$\\
    \hspace*{\algorithmicindent} \textbf{Output: } Q2\_num
    \end{flushleft}
    \begin{algorithmic}[1]
    \Function{CountQ2}{G}
    \State $s \gets 0$
    \State $V_1 = V$
    \For{vertex $v_1 \in V_1$}
        \State $V_2 = N(v_1), V_3^{1} = N(v_1), V_4^{1} = N(v_1), V_5^{1} = N(v_1)$
        \For{ $v_2 \in V_2$}
            \State $V_3 = V_3^{1} \cap N(v_2)$,  $\:V_4^{2} = V_4^{1} \cap N(v_2)$
            \State $V_5^{2} = V_5^{1} - N(v_2)$, $V_6^{2} = N(v_2) - N(v_1)$
            \State $G_{min} = empty$
            \For{$v_5 \in V_5^{2}$}
                \State $T(v_5) = V_6^{2} \cap N(v_5)$
                \State $G_{min}.add(v_5, T(v_5))$
            \EndFor
            \For{$v_3 \in V_3$}
                \State $V_4 = V_4^{2} - N(v_3)$, $V_5^{3} = V_5^{2} \cap N(v_3)$
                \State $V_6^{3} = V_6^{2} \cap N(v_3)$
                \For{$v_4 \in V_4$}
                    \State $V_5 = V_5^{3} - N(v_4)$, $V_6^4 = V_6^{3} - N(v_4)$
                    \For{$v_5 \in V_5$}
                        \State $T(v_5) = G_{min}.get(v_5)$
                        \State $V_6 = V_6^{4} - T(v_5)$
                        \State $Q2\_num = Q2\_num + | V_6 |$
                    \EndFor
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \State \Return $Q2\_num$
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> algorithms-old/naive4clique.tex <==
\begin{algorithm}
    \caption{Naive 4Clique Count}\label{algo:naive4clique}
    \begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input: } graph $G(V, E)$\\
    \hspace*{\algorithmicindent} \textbf{Output: } 4cliqueNum
    \end{flushleft}
    \begin{algorithmic}[1]
    \Function{Count4Clique}{G}
    \State $s \gets 0$
    \State $V_1 = V$
    \For{vertex $v_1 \in V_1$}
        \State $V_2 = N(v_1)$
        \For{ $v_2 \in V_2$}
            \State $V_3 = N(v_1) \cap N(v_2)$
            \For{$v_3 \in V_3$}
                \State $V_4 = N(v_1) \cap N(v_2) \cap N(v_3)$
                \State $s = s + |V_4|$
                \For {$v_4 \in V_4$}
                    \State $\{v_1, v_2, v_3, v_4\}$ is a 4-clique
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \State \Return $s$
    \EndFunction
    \end{algorithmic}
\end{algorithm}
% \begin{minipage}{0.5\textwidth}
%     \begin{algorithm}[H]
%         \small
%         \begin{algorithmic}[1]
%         \For{$v_1 \in V_1$}
%             \State $V_2 = N(v_1)$
%             \For{ $v_2 \in V_2$ }
%                 \State $V_3 = N(v_1) \cap N(v_2)$
%                 \For{$v_3 \in V_3$}
%                     \State $V_4 = N(v_1) \cap N(v_2) \cap N(v_3)$
%                     \For{$v_4 \in V_4$}
%                         \State out $(v_1, v_2, v_3, v_4)$ 
%                     \EndFor
%                 \EndFor
%             \EndFor
%         \EndFor
%         \end{algorithmic}
%     \end{algorithm}  
% \end{minipage}


==> algorithms-old/prefix4clique.tex <==
\begin{algorithm}
    \caption{Prefix Optimization 4Clique Count}\label{algo:prefix4clique}
    \begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input: } graph $G(V, E)$\\
    \hspace*{\algorithmicindent} \textbf{Output: } 4cliqueNum
    \end{flushleft}
    \begin{algorithmic}[1]
    \Function{Count4Clique}{G}
    \State $s \gets 0$
    \State $V_1 = V$
    \For{vertex $v_1 \in V_1$}
        \State $V_2 = N(v_1)$
        \State $V_3^1 = V_2$
        \State $V_4^1 = V_2$
        \For{ $v_2 \in V_2$}
            \State $V_3 = V_3^1 \cap N(v_2)$
            \State $V_4^2 = V_3$
            \For{$v_3 \in V_3$}
                \State $V_4 = V_4^2 \cap N(v_3)$
                \State $s = s + |V_4|$
                \For {$v_4 \in V_4$}
                    \State $\{v_1, v_2, v_3, v_4\}$ is a 4-clique
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \State \Return $s$
    \EndFunction
    \end{algorithmic}
\end{algorithm}
% \begin{algorithm}
%     \begin{algorithmic}
%     \State $s \gets 0$
%     \For{vertex $v_1 \in V_1$}
%         \State $V_2 = N(v_1)$
%         \State $V_3^{1} = N(v_1)$
%         \For{ $v_2 \in V_2$}
%             \State $V_3 = V_3^{1} \cap N(v_2)$
%             \State $V_4^{2} = V_3$
%             \For{$v_3 \in V_3$}
%                 \State $V_4 = V_4^{2} \cap N(v_3)$
%                 \State $s = s + |V_4|$
%             \EndFor
%         \EndFor
%     \EndFor
%     \end{algorithmic}
% \end{algorithm}

==> algorithms-old/prefixq2.tex <==
\begin{algorithm}
    \caption{ Prefix Optimization Q2 }\label{algo:prefixq2}
    \begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input: } graph $G(V, E)$\\
    \hspace*{\algorithmicindent} \textbf{Output: } Q2\_num
    \end{flushleft}
    \begin{algorithmic}[1]
    \Function{CountQ2}{G}
    \State $s \gets 0$
    \State $V_1 = V$
    \For{vertex $v_1 \in V_1$}
        \State $V_2 = N(v_1), V_3^{1} = N(v_1), V_4^{1} = N(v_1), V_5^{1} = N(v_1)$
        \For{ $v_2 \in V_2$}
            \State $V_3 = V_3^{1} \cap N(v_2)$,  $\:V_4^{2} = V_4^{1} \cap N(v_2)$
            \State $V_5^{2} = V_5^{1} - N(v_2)$, $V_6^{2} = N(v_2) - N(v_1)$
            \For{$v_3 \in V_3$}
                \State $V_4 = V_4^{2} - N(v_3)$, $V_5^{3} = V_5^{2} \cap N(v_3)$
                \State $V_6^{3} = V_6^{2} \cap N(v_3)$
                \For{$v_4 \in V_4$}
                    \State $V_5 = V_5^{3} - N(v_4)$, $V_6^4 = V_6^{3} - N(v_4)$
                    \For{$v_5 \in V_5$}
                        \State $V_6 = V_6^{4} - N(v_5)$
                        \State $Q2\_num = Q2\_num + | V_6 |$
                    \EndFor
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \State \Return $Q2\_num$
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> algorithms-old/q2.tex <==
\begin{algorithm}
    \caption{ Q2 }\label{algo:q2}
    \begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input: } graph $G(V, E)$\\
    \hspace*{\algorithmicindent} \textbf{Output: } Q2\_num
    \end{flushleft}
    \begin{algorithmic}[1]
    \Function{CountQ2}{G}
    \State $s \gets 0$
    \State $V_1 = V$
    \For{vertex $v_1 \in V_1$}
        \State $V_2 = N(v_1)$
        \For{ $v_2 \in V_2$}
            \State $V_3 = N(v_1) \cap N(v_2)$
            \For{$v_3 \in V_3$}
                \State $V_4 = N(v_1) \cap N(v_2) - N(v_3)$
                \For{$v_4 \in V_4$}
                    \State $V_5 = N(v_1) \cap N(v_3) - N(v_2) - N(v_4)$
                    \For{$v_5 \in V_5$}
                        \State {\small $V_6 = N(v_2) \cap N(v_3) - N(v_1) - N(v_4) - N(v_5)$}
                        \State $Q2\_num = Q2\_num + | V_6 |$
                    \EndFor
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \State \Return $Q2\_num$
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> algorithms/Q1-GraphMini.tex <==
\begin{algorithm}[t]
    \caption{ Query Execution with GraphMini}
    \label{algorithms:Q1-GraphMini}
    \begin{algorithmic}[1]
    \Function{Emit-Matches-GraphMini}{G}
    \State $S_1 = V$
    \For{ $u_1 \in S_1$}
        \State $S_2 = S_3^1 = S_4^1= N(u_1) $
        \State \emph{MiniG}$(S_4^1, S_3^1) = empty$
        \For{ $w \in S_3^1$} \label{ln:mini-start}
            \State $N_{4, 3}^1(w) = S_4^1 \cap N(w) $
            \State \emph{MiniG}$(S_4^1, S_3^1).add( N_{4, 3}^1(w) )$
        \EndFor \label{ln:mini-end}
        \For{ $u_2 \in S_2$}
            \State $N_{4, 3}^1(u_2) = $ \emph{MiniG}$(S_4^1, S_3^1).get(u_2)$ \label{ln:mini-retrieve}
            \State $S_4^2 = S_3 = N_{4, 3}^1(u_2)$ \label{ln:mini-compute}
            \For{$u_3 \in S_3$}
                \State $N_{4, 3}^1(u_3) =$ \emph{MiniG}$(S_4^1, S_3^1).get(u_3)$
                \State $S_4 = S_4^2 - N_{4, 3}^1(u_3)$ \label{ln:mini-s4}
                \For {$u_4 \in S_4$ }
                    \State \emph{emit}$(u_1, u_2, u_3, u_4)$
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> algorithms/Q1-Minigraph.tex <==
\begin{algorithm}[ht]
    \small
    \caption{Example of Query Execution with Minigraph}
    \label{algorithms:Q1-Minigraph}
    \begin{algorithmic}[1]
    \Require{$G$ data graph} 
    \Ensure{depends on \emph{emit}}
    \Function{EmitMatchesMinigraph}{G}
    \State $C(v_1) = V(G)$
    \For{ $u_1 \in C(v_1)$}
        \State $C(v_2) = C_1(v_3) = C_1(v_4)= N(u_1) $ 
        \State \emph{/* materialize auxiliary graph */}
        \State $A_1(v_3,v_4) = empty$ \label{ln:mini-start}
        % \jl{TODO: add checking condition}
       \For{$u \in C_1(v_3)$}  \emph{/* scan filtering set */}
            \State $P_{1,3}(u | v_4) = C_1(v_4) \cap N(u) $
            \State $A_1(v_3,v_4).add( P_{1,3}(u | v_4 ) )$
        \EndFor \label{ln:mini-end}
        \For{ $u_2 \in C(v_2), \: u_2 < u_1$}
            \State \emph{/* use auxiliary graph */}
            \State $P_{1,3}(u_2 | v_4) = A_1(v_3,v_4).get(u_2)$ \label{ln:mini-retrieve}
            \State $C(v_3) = C_2(v_4) = N(u_1) \cap N(u_2) = P_{1,3}(u_2 | v_4)$ \label{ln:mini-compute}
            % \begin{align*}
            %     C(v_3) &= C_1(v_3) \cap N(u_2) \\
            %         &= C_1(v_4) \cap N(u_2) = P_{1,3}(u_2 | v_4)
            % \end{align*}
            \For{$u_3 \in C(v_3)$}
                \State $P_{1,3}(u_3 | v_4) =  A_1(v_3,v_4).get(u_3)$\label{ln:mini-s4-begin}
                \State $C(v_4) = C_2(v_4) -$ $P_{1,3}(u_3 | v_4)$ \label{ln:mini-s4}
                \For {$u_4 \in C(v_4),\: u_4 < u_3$ }
                    \State \emph{emit}$(u_1, u_2, u_3, u_4)$
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> algorithms/Q1-Prefix.tex <==
\begin{algorithm}[ht]
    \small
    \caption{Optimized Pseudo-Code Using Prefix Sets } \label{algorithms:Q1-Prefix}
    \begin{algorithmic}[1]
    \Require{$G$ data graph} 
    \Ensure{depends on \emph{emit}}
    \Function{EmitMatchedPrefix}{G}
    \State $C(v_1) = V(G)$
    \For{ $u_1 \in C(v_1)$}
        \State $C(v_2) = C_1(v_3) = C_1(v_4)= \: N(u_1) $
        \For{ $u_2 \in C(v_2), \: u_2 < u_1$}
            \State $C(v_3) = C_2(v_4) = \: C_1(v_3) \cap N(u_2)$\label{ln:reuse}
            \For{$u_3 \in C(v_3)$}
                \State $C(v_4) = \: C_2(v_4) - N(u_3)$
                \For {$u_4 \in C(v_4), \: u_4 < u_3$ }
                    \State \emph{emit}$(u_1, u_2, u_3, u_4)$
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> algorithms/Q1.tex <==
\begin{algorithm}[t]
    \caption{Example of Generated Query Execution Code}\label{algorithms:Q1}
    \begin{algorithmic}[1]
    \Procedure{Emit-Matches}{G}
    \State $S_1 = V$
    \For{ $u_1 \in S_1$}
        \State $S_2 = N(u_1) $
        % \State $U_2 = U_2 - [u_1]$
        \For{ $u_2 \in S_2$}
            \State $S_3 = N(u_1) \cap N(u_2)$
            % \State $U_3 = U_3 - [u_1, u_2]$
            \For{$u_3 \in S_3$}
                \State $S_4 = N(u_1) \cap N(u_2) - N(u_3)$
                \For {$u_4 \in S_4$ }
                    \State \emph{emit}$(u_1, u_2, u_3, u_4)$
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \EndProcedure
    \end{algorithmic}
\end{algorithm}

==> algorithms/prefix-query-2.tex <==
\begin{algorithm}[t]
    \caption{ Count $P_6$ with Prefix Optimization }\label{algorithms:prefix-pattern-2}
    \begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input: } graph $G(V, E)$\\
    \hspace*{\algorithmicindent} \textbf{Output: } counter
    \end{flushleft}
    \begin{algorithmic}[1]
    \Function{Count-$P_6$-Prefix}{G}
    \State $counter \gets 0$
    \State $U_1 = V$
    \For{vertex $u_1 \in U_1$}
        \State $U_2 = N(u_1), U_3^{1} = N(u_1), U_4^{1} = N(u_1), U_5^{1} = N(u_1)$
        \For{ $u_2 \in U_2$}
            \State $U_3 = U_3^{1} \cap N(u_2)$,  $\:U_4^{2} = U_4^{1} \cap N(u_2)$
            \State $U_5^{2} = U_5^{1} - N(u_2)$, $U_6^{2} = N(u_2) - N(u_1)$
            \For{$u_3 \in U_3$}
                \State $U_4 = U_4^{2} - N(u_3)$, $U_5^{3} = U_5^{2} \cap N(u_3)$
                \State $U_6^{3} = U_6^{2} \cap N(u_3)$
                \For{$u_4 \in U_4$}
                    \State $U_5 = U_5^{3} - N(u_4)$, $U_6^4 = U_6^{3} - N(u_4)$
                    \For{$u_5 \in U_5$}
                        \State $U_6 = U_6^{4} - N(u_5)$
                        \State $counter = counter + | U_6 |$
                    \EndFor
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \State \Return $counter$
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> algorithms/query-2.tex <==
\begin{algorithm}[t]
    \caption{ Count $P_6$ }\label{algorithms:query-2}
    \begin{flushleft}
    \hspace*{\algorithmicindent} \textbf{Input: } graph $G(V, E)$\\
    \hspace*{\algorithmicindent} \textbf{Output: } counter (number of subgraphs that match P2)
    \end{flushleft}
    \begin{algorithmic}[1]
    \Function{Count-$P_6$}{G}
    \State $counter \gets 0$
    \State $U_1 = V$
    \For{ $u_1 \in U_1$}
        \State $U_2 = N(u_1) $
        % \State $U_2 = U_2 - [u_1]$
        \For{ $u_2 \in U_2$}
            \State $U_3 = N(u_1) \cap N(u_2)$
            % \State $U_3 = U_3 - [u_1, u_2]$
            \For{$u_3 \in U_3$}
                \State $U_4 = N(u_1) \cap N(u_2) - N(u_3)$
                % \State $U_4 = U_4 - [u_1, u_2, u_3]$
                \For{$u_4 \in U_4$}
                    \State $U_5 = N(u_1) \cap N(u_3) - N(u_2) - N(u_4)$
                    % \State $U_5 = U_5 - [u_1, u_2, u_3, u_4]$ 
                    \For{$u_5 \in U_5$}
                        \State \scalebox{0.8}{$U_6 = N(u_2) \cap N(u_3) - N(u_1) - N(u_4) - N(u_5)$}
                        % \State $U_6 = U_6 - [u_1, u_2, u_3, u_4, u_5]$
                        \State $counter = counter + | U_6 |$
                    \EndFor
                \EndFor
            \EndFor
        \EndFor
    \EndFor
    \State \Return $counter$
    \EndFunction
    \end{algorithmic}
\end{algorithm}

==> sections-old/0-abstract.tex <==
\begin{abstract}
    The study of structural patterns in graphs is fundamental to graph mining. Existing work has proposed a compilation-based system for handling graph mining problems. Here, the system takes an abstract graph pattern and produces a schedule with restrictions and a corresponding computation plan. This approach suffers as the generated code from the existed system does not use structural patterns to reduce redundant computation.

    Rather than use this a posteriori compilation-based system, we adopt an a priori approach. We leverage common patterns \ao{specifically?} in real world graphs \jl{that the degree of vertexes in the graph often follow a power-law distribution} to generate faster code.  We propose \optimizer{}, which uses \cache{} to generate faster computations. We find that \optimizer{} brings significant speed-ups over the state-of-the-art algorithms on supported patterns.

\end{abstract}

==> sections-old/1-introduction.tex <==
\section{Introduction}
Graphs represent and integrate large amounts of data in domains such as knowledge bases, finances, user recommendations, social networks, and biology. Pattern matching is considered one of the most important fields of study for graph mining. In the pattern matching problem, we find all subgraphs of an input graph that match a given pattern. Compared to graph problems like shortest path discovery, BFS, and DFS, graph pattern matching is notoriously difficult as it involves intensive computation and generates a large amount of intermediate data.

Although a generalized mining algorithm can handle arbitrary patterns, it usually suffers from poor performance and large memory consumption. While hard coding algorithms remains popular, it is unscalable when the input patterns have a large domain.

Many recent works (\cite{EmptyHeaded}, \cite{Graphflow}, \cite{AutoMine}, \cite{GraphZero}, \cite{GraphPi}) focused on building high performance systems that can handle arbitrary patterns. These systems generate efficient low-level code for handling each input pattern instead of using a generalized algorithm. They have shown that a compilation-based system in which we turn subgraph queries into efficient low level code often outperforms a generalized algorithm by several orders of magnitudes. 

AutoMine, GraphZero, and GraphPi represent the state-of-the-art of such systems. They addressed three challenges that existed in previous works. 

\begin{enumerate}
    \item Avoiding excessive intermediate results 
    \item Pruning automorphisms, discussed in detail in Section \ref{sec:back}
    \item Optimizing the schedule and restrictions, discussed in detail in Section \ref{sec:back}
\end{enumerate}
%  A schedule is an order for traversing the vertices in the pattern, whereas the restrictions are rules that correspond to the schedule for removing all the automorphisms. Each schedule can have different restriction sets for pruning automorphism. Choosing the optimal combination of the schedule and its restrictions can substantially improve the performance. AutoMine uses a loop-based model to estimate the cost of each schedule. GraphZero further generates a set of restrictions to avoid the redundant computation caused by automorphism, addressing the problem that AutoMine can only handle root symmetry. GraphPi considers the influence of both the schedules and the restrictions and selects the best combination of the two.

These systems separate the schedules from the algorithms. They use a scheduler to decide the order for traversing the vertices in the input pattern. Then, they use the best schedule to generate efficient C++ code. 

All three systems use the same methodology proposed in AutoMine to generate efficient low-level code. 

We observe that AutoMine implements a conservative strategy for storing the intermediate results, which will be discussed in the following section.
This strategy allows AutoMine to handle very large graphs using minimized memory consumption. 
However, it also prevents AutoMine from exploring the optimization opportunities in the schedule.
We find that by analyzing the input schedule and by proactively caching instead of waiting until the algorithm begins to run, we can generate faster algorithms than in the online approach.
Although this strategy consumes a little \ao{data?} \jl{will be discussed in evaluation section} more memory, it can significantly improves the performance for complex queries on large graphs.
We generalize the idea of active caching and use this methodology to build \optimizer, which matches a given schedule into efficient C++ code. 
This paper makes the following contributions: 
\begin{itemize}
    \item	We present \cache, a new methodology for actively caching the intermediate results for graph mining.
    \item	We build \optimizer{} based on this methodology. The results from evaluation show that it significantly outperforms state-of-the-art algorithms. 
\end{itemize}


==> sections-old/2-background.tex <==
\section{Background}
\label{sec:back}
\subsection{Problem Definition}

We are given a data graph $G(V,E)$ with vertices $V$ and edges $E$ such that an edge $E(v_1,v_2)$ implies an edge between $v_1,v_2 \in V$.
We define subgraph queries in the format $G_q(V_q,E_q)$ with vertices $V_q$ and edges $E_q$ such that an edge $E_q(u_1,u_2)$ represents an edge between query vertex in $u_1,u_2 \in V_q$.
For example: \\
\begin{multline}
  4clique(u_1,u_2,u_3,u_4) = E(u_1,u_2), E(u_1, u_3), E(u_1,u_4), \\
  E(u_2,u_3), E(u_2,u_4), E(u_3,u_4)
\end{multline}

We define a subgraph $ G_s(V_s, E_s) $ of $G$ as isomorphic to $G_q$ if there exists a bijection between $G_q$ and $G_s$ such that:
$$ \forall u_i, u_j \in V_q: (u_i, u_j) \in E_q \iff (v_i, v_j) \in E_s $$
Here, $u_i$ and $u_j$ are matched to $v_i$ and $v_j$ respectively. We say $G_s$ matches $G_q$ if they are isomorphic.
A partial query $P(V_p,E_p)$ is defined such that:
$$V_p \subset V_q \: \& \: E_p \subset E_q$$
The partial match is incrementally extended by adding edges and vertexes till the whole query is matched.
Enumeration order is defined as the order in which edges or vertexes are added.
A connected enumeration order is an enumeration order in which every edge or vertex that is added has an edge or vertex which has been previously added to our partial match.
We call a connected enumeration order a schedule.
The result of a subgraph query is the set of all unique subgraphs of the data graph that are isomorphic to the query graph.
We note that we define unique subgraphs as those subgraphs that are not automorphic to each other.
Two graphs are automorphic if they are symmetric to each other.
Automorphic matches to the same query graph are typically considered redundant and are filtered.
To do so, we can include a \emph{canonicality constraint}.
Canonicality constraints impose a partial ordering among the ids of the vertices in a match.
The purpose of these constraints is to eliminate redundant matches to the same pattern.
For example, suppose that the query graph is a triangle and that the data graph $G$ has three data vertices $v_1, v_2, v_3$ forming a triangle.
Each permutation of the three vertices corresponds to a valid bijection matching the query vertices $q_1, q_2, q_3$, all automorphic to each other.
To select only one among them, we can impose the canonicality constraint $q_1 < q_2 < q_3$.
Canonicality constraints define a partial order among the identifiers of the data vertices matching the query vertices.
In the case of this constraint, only $v_1, v_2, v_3$ can match $q_1, q2, q_3$, respectively.
Thus, matches that do not respect the canonicality constraints of a query are not returned and so automorphic results are filtered. %maybe we can cut later?
In this paper, we focused on vertex-induced patterns but the techniques also apply to edge-induced patterns.
If we represent the graph as a table $T$ of $(s,d)$ edges having two attributes (source vertex, destination vertex), matching one edge corresponds to performing a standard binary join operator between the table containing the partial matches and the graph table $T$.
A subgraph query executor that uses only binary joins uses an ``edge-at-a-time" approach.
This is in contrast to multi-way joins, which induce a ``vertex-at-a-time'' approach.

When the next query vertex to be matched has edges to two or more query vertices that have already been matched, matching one vertex requires matching multiple edges at the same time.
This corresponds to performing one multi-way join on the graph table.
% We define a match for the query Q as one-one(could be many-one) function between query vertex and data vertices.
% \begin{equation*}
%   {M:V_q \to V: \forall (v_i,v_j) \in E_q \exists (M(v_i),M(v_j)) \in E}
% \end{equation*}


\subsection{AutoMine's Methodology}

Systems before AutoMine used an algorithm that can be described as a sequence of binary self-joins over the edge table of a database, where each join matches one edge of the query graph.
This approach needs to store many dependent results, and their size increases exponentially as the pattern becomes more complex.

AutoMine uses a different approach. To find matches, it matches the query graph to subgraphs that include a fixed vertex.
We call this vertex the root vertex.
In other words, AutoMine extends edges and vertexes in the graph to the sub-pattern that contains the root vertex until it matches the query.

To explain how AutoMine generalize this idea, we denote $P_k$ as a connected pattern of size k, $P_{k-1}$ as its sub-pattern of size k-1, $E_{P_k}$ as an instance of $P_k$, and $E_{P_{k-1}})$ as an instance of $P_{k-1}$.
To match a pattern $P_k$, it first fixes one vertex $v_1$. This single vertex can be considered as $E_{P_1}$, an instance of the sub-pattern $P_1$.
Then, it computes the candidate set $V_2$ which contains all vertices that can extend $E_{P_1}$ to some $E_{P_2}$.
It then fixes $v_2$ and $(v_1, v_2)$ can be considered as a $E_{P_2}$. It then computes $V_3$, which can extend the $E_{P_2}$ to some $E_{P_3}$.
It keeps doing so until a set of $V_n$ is computed. The candidates in $V_n$, together with previously fixed vertices $[v_1, v_2, \ldots  v_{n-1}]$ form a set of $E_{P_k}$.
Each $E_{P_k}$ is an unique subgraph that matches the given pattern.

Naturally, this algorithm can be implemented in a nested loop structure.  I.E., if matching pattern $P_k$, AutoMine would generate $k$ nested loops where each nested loop computes the candidate set to iterate in the next nested loop.

AutoMine uses function $F_k$ on to compute the set $V_k$. $F_k$ defines the relation of neighbor set of $v_k$ and those of $[v_1, v_2,\ldots v_{k-1}]$.
Suppose $E_{P_{k-1}} = [v_1, v_2, \ldots  v_{k-1}]$, AutoMine partitions the vertices in this embedding into two sets $V_T$ and $V_F$ such that:
% $V_T$ contains all the vertices that are neighbors of $v_k$ and $V_F$ contains all the vertices that are not neighbors of $v_k$. 
% In other words, 
$$\forall v \in V_T: v_k \in N(v) $$
$$\forall u \in V_F: v_k \notin N(u) $$
It follows that:
$$V_k = F_k(E_{P_{k-1}}) = \bigcap_{v \in V_T}N(v)-\bigcup_{u \in V_F} N(u)$$
(The base function $F_1$ returns the set of all vertexes in the graph.)

This algorithm allows AutoMine to discover instances of complex pattern $P_k$ based on any embedding of $P_{k-1}$, hence it can handle any connected pattern.

Note that instead of using set union shown in the above formula, AutoMine computes the result of the set intersections first. Then it subtracts the neighbor sets of the vertices in $V_F$ one after another.
In this way, AutoMine only uses set intersection and set subtraction to compute the new results.
This reduces memory consumption.
For set intersection, the output set is no larger than the smaller input set.
For set subtraction, the output set is no larger than the input set being subtracted.
This allows AutoMine to pre-allocate memory based on the largest degree of any vertex in the graph, as the size of $V_k$ cannot be larger than this number.

\subsection{Prefix Optimization}
However, naively implement this algorithm brings redundant computation and data access. This can be seen in the 4-clique counting example.
This algorithm counts the number of cliques in the input graph $G(V, E)$. \ao{explain eventually}
Each loop add one more vertex to the sub-matching and compute the candidates for the next iteration.
\input{algorithms-old/naive4clique.tex}


In this naive implementation, the innermost loop needs to scan $N(v_1)$, $N(v_2)$ and $N(v_3)$ to compute $V_4$.
However, the result of $N(v_1) \cap N(v_2)$ is not affected by the value of $v_3$. It can be obtained before iterating through $V_3$.
We call this result loop invariant to the innermost loop.
Ideally, we only need to compute this result once and reuse it in the deeper nested loops for multiple times.
In this case, $V_3$ happens to store the result of $N(v_1) \cap N(v_2)$ so we can use it in the innermost loop.
\input{algorithms-old/prefix4clique.tex} \ao{same comment as above}

AutoMine generalized this idea and proposed a technique called prefix optimization to avoid redundant computation and data access.
The main idea of prefix optimization is to store the results from loop invariant computation and reuse them in the inner nested loops.
AutoMine uses function $F_k^p$ as the prefix function for $F_k$. $F_k^p$ defines all $F_k$’s operation on $[v_1, v_2, \ldots, v_{p}] (1<p<k)$.
AutoMine aggressively apply this optimization when generate code.
For a pattern of size n, AutoMine would compute prefix functions $[F_{k+1}^{k-1}, F_{k+2}^{k-1}, \ldots ,F_{n}^{k-1}]$ in addition to $F_k$ at loop level k-1.
We denote the results from prefix function $F_k^p$ as $V_k^p$.
This algorithm allows AutoMine generalizes the idea of prefix optimization and uses it extensively during code generation.

% \subsection{Motivation of LOVE}
% The set intersection and set subtraction take the majority of running time for this algorithm. 
% The common set intersection and set subtraction algorithm assume that the input sets are sorted. 

% Set intersection algorithm takes two sorted sets (A and B) as input and outputs a sorted set (C) that contains the common elements in both A and B. 
% To do so, it keeps two pointers pointing to the start of the two input sets (A and B). 
% Each time it compares the data pointed and increment the pointer with the smaller data. It increment both pointers when the data are the same (and write it to the output C).  
% It repeatedly doing so until one of the sets is traversed from start to end. 
% The set subtraction algorithm differs only in the selection of data to output. 
% It also needs to scan one of the sets to the end. 
% In terms of time complexity, both algorithms are linear to the size of the input sets. 

% We observe that even with prefix optimization, AutoMine might need to scan the neighbor sets entirely. 
% Moreover, the total access cost of accessing a given vertex’s neighbor sets is super-linear to its degree in power-law graphs. 
% In the case of 4-clique counting, this cost is cubic to the vertex degree. 
% This means that AutoMine’s generated algorithm needs to frequently scan the large neighbor sets. 
% This observation encourages us to ask a question: How can reduce the size of the input sets while preserving the results? 

% (Explain LOVE's intuition.)
\subsection{Pruning Automorphisms}
The automorphic graphs contain the same nodes that preserve the edge and non-edge relationship of the query pattern. The only difference is the order to traverse the nodes.

Take 4-clique pattern as an example.
Suppose we discover one match of the pattern with vertex ids: $\{v_0=0, v_1=1, v_2=2, v_3=3\}$.
It implies the four vertexes are pair-wise connected in the input graph.
We will find other valid matchings like $\{ \{v_0=0, v_1=1, v_2=3, v_3=2\}, \{v_0=0, v_1=2, v_2=1, v_3=3\}, \ldots\}$.
These extra matchings provide no additional information and we want to remove them from the output.
We can remove them at the end of execution but this can introduce significant amount of redundant computation.
The common approach is by applying restrictions on the vertex ids.
For example, ensuring $v_0 > v_1 > v_2 > v_3$ can exclude the extra matchings.
Suppose the set that contains candidate $v_1$ is sorted, when iterate through the set.
When we find a $v_1$ that is not smaller than $v_0$, we can safely avoid iterating through the remaining $v_1$s because they must be greater than $v_0$ too.
Doing so also avoids materializing the candidate sets for $v_2$ and $v_3$.
GraphZero has generalized this idea. It sorts all neighbor sets and applies the restrictions during set intersections.
GraphZero modified the set operations so it can terminate when it finds a vertex id that violates the constraint.
This further reduces unnecessary data access for it avoids scanning the remaining vertex ids in the input sets.
We adopt GraphZero's approach to apply restrictions.

\subsection{Optimal Schedule}
Two main factors significant influence the performance of a pattern's schedule:
1) The restrictions to apply. 2) The matching order of the vertexes in the pattern.
Intuitively, we prefer to apply restrictions at an early stage of the computation, which avoids materializing subsequent candidate sets if a restriction is violated.
Also, we might want to materialize the vertex with the most edges first if the data graph is sparse.
Even if it is not associated with any restriction.
For example, if one vertex $v_0$ is connected to all the other vertexes in the pattern, materializing it can limit the scope of other vertexes' candidate set.
All the other vertexes in the matching must be found in $v_0$'s neighbor set, which helps the algorithm to scan less vertexes.

GraphZero proposed an algorithm that can automatically generate restrictions for any (connected) pattern.
It can generate one set of restrictions that completely prune the automorphisms for the input pattern.
However, there might exists more than one sets of restrictions that can completely prune the automorphisms for an given pattern.
GraphPi is able to find all of them, which is crucial for choosing the optimal schedule.

GraphPi uses the information of the data graph to choose the optimal combination of matching order and restrictions in the schedule.
It generates the optimal schedule based on the graph pattern, the number of vertexes, edges, and triangles in the graph.
We use GraphPi's algorithm to generate the optimal matching order and the restrictions for code compilation since it is the current state-of-the-arts.

\subsection{Bottlenecks of state-of-the-arts}
Both GraphPi and GraphZero use AutoMine's methodology to compile C++ code in the low level.
AutoMine's compilation methodology heavily uses set intersection and set subtraction.
In 4-clique counting, the set intersections take up more than 90\% of the running time.

The common set intersection and set subtraction algorithm for graph pattern matching problems can be implemented as a linear scan of two sorted vertex sets.
It has a complexity that is linear to the size of the input sets.

For example, the set intersection algorithm takes two sorted sets as input and outputs a sorted set that contains the common elements.
It keeps two pointers pointing to the start of the two input sets. Each time it compares the data pointed by the pointers and increment the one that points to the smaller data. It increments both pointers when the data they point to are the same and outputs the data. It keeps doing so until one of the sets is traversed from start to end. (Can change it to figure.)

The set subtraction algorithm is like the set intersection but differs in the selection of data to output.
It also needs to scan one of the sets to the end. In terms of time complexity, both algorithms are O(|A|+|B|) where A and B represent the input sets.
The observation here is the size of the input will strongly influence the time taken to complete the computation.
This encourage us to think about potential methods to reduce the input size through active caching.

AutoMine can cache the loop invariant results, but it cannot cache the results that have not been computed.
Take 4-clique counting as an example. The innermost loop computes $N(v_1) \cap N(v_2) \cap N(v_3)$ to get $V_4$.
AutoMine would use prefix optimization and store the result of $N(v_1) \cap N(v_2)$ in $V_4^2$ at loop level 2 (see Algorithm \ref{algo:prefix4clique}, line 8).
It remains to compute the set intersection of $V_4^2$ and $N(v_3)$.
AutoMine might need to scan the whole $N(v_3)$ if it contains the largest element in the two sets. Prefix optimization does not optimize $N(v_3)$ in this case.

This is exaggerated by the super-linear relation of the total access cost of a given vertex’s neighbor sets and the degree of the vertex and to the loop level.
The total access cost of a given vertex's neighbor set can be estimated by the number of times the neighbor set being accessed multiplied by its cardinality.
The actual total cost is difficult to predict. However, we can use a simplified model to illustrate the intuition.

Assume we have a random graph $G(V, E)$. The probability that a vertex $u$ is connected to a random vertex $y$ in the graph is:
$$p = \frac{|N(u)|}{|V|}$$
For a given pattern of size n, AutoMine's algorithm iterates through $V_k$ at loop level $k \: (k < n)$ exploring the subgraphs of the root vertex.
The expected number of times that $u$ in $V_k$ is $p \times V_k$.
Also take into consideration that $V_k$ is accessed for $\prod_{1 \leq i < k} |V_i|$ times for a given root vertex.
At loop level k, the total number becomes in $p \times \prod_{1 \leq i \leq k}|V_i|$.
Multiply this by the cardinality of the neighbor set we get the cost of x at loop level k to be:
$$Cost(u, k) = |N(u)| \times p \times \prod_{1 <= i <= k}|V_i| = \frac{|N(u)|^2 }{|V|} \times \prod_{1 <= i <= k}|V_i| $$
In this simplified model, the total cost is quadratic to the degree of the vertex. Also, it can increase exponentially as the loop depth increases.


% Notice that the new approach needs to scan $N(v_1)$ twice (one for y1y2, another time for y1y3) for computing one V4, whereas AutoMine’s straightforward schedule only needs to scan $N(v_1)$ once. 
% Note that the result in y1y3 must be reused multiple times to bring a speedup. We achieve this by making friend with the super-linear relation. 
% Ideally, we want to discover all such optimization opportunities for an arbitrary schedule at compile time. We now discuss the generalization this idea.


==> sections-old/3-overview.tex <==
\section{Overview of Graph Mini}
In this paper, we propose graph mini, a methodology to generate faster graph mining algorithms. 

We use GraphPi to choose the optimal schedule for matching the pattern.
It has a real time scheduler that can generate optimal schedules for each input pattern based on the structural information of the data graph. 

Both AutoMine and graph mini can generate faster algorithm using GraphPi's optimal schedule.
Like AutoMine, graph mini automatically generates efficient C++ code based on the input pattern, its matching order and restrictions. 
We further utilize a property of set to aggressively predict the computation and cache the intermediate results on the fly.
This allow us to significantly reduce the time for running queries on large graphs.

% The key insight is we can reduce the time of set intersections and set subtractions by actively caching before the actual computation begins. 
We next describe the key techniques in our code generator. 

\jl{Working on: add a graph to illustrate its structure}
\ao{this is super short right now, let's definitely add some of the later ideas and discussion from background here}

==> sections-old/4-methodology.tex <==
\section{Methodology of \optimizer{}}
\jl{This new section discuss the intuition behind mini-graph. Needs comments here}
\subsection{Terminology}
In the following discussion, we assume the input pattern graph $G_p(V_p, E_p)$ and its optimal schedule are given.
We also represent the schedule as a list of prefix functions described in AutoMine's methodology. 
We use $F_k$ and $V_k$ to represent the abstract computation and the materialized data for the candidate set of $v_k$ respectively.
More specifically, $F_k^i$ computes the prefix of $V_k$ based on the edge relations between $v_k$ and $\{v_1, v_2, \ldots, v_i\}$, and it does not reflect the edge relation between $v_k$ and $\{v_{i+1}, v_{i+2}, \ldots, v_{k-1}\}$
Similarly, we use $V_k^i$ to denote the materialized data set for the prefix function $F_k^i$.
We use $N(v_i)$ to represent the $v_i$'s neighbor set. 

\subsection{Property of The Prefix Functions}
We first analyze the property of prefix function to highlight the main property we used to build \cache{}.
Like AutoMine, we use prefix optimization extensively.
This means a prefix function will be partially computed by its own prefix function.

We define that the prefix function $F_k^0$ always return all vertices in the graph.
In other words $V_k^0 = V$. 
Although $V_k^0$ is not used for actual computation, having this notion is helpful to show that: 
$$V_k^{i+1} \subseteq V_k^{i} (i \geq 0)$$ 

This is because $V_k^{i}$ is obtained by set intersection or set subtraction between $V_k^{i}$ and $N(v_{i+1})$. 
Consequently, $V_k^{i+1}$ cannot have any vertex that is not in $V_k^{i}$.

As $i$ increases, $V_k^i$ becomes more selective as $F_k^i$ reflects more edge relations between $v_k$ and the other vertexes in the partial match $\{v_1, v_2, \ldots, v_i\}$.
Each additional edge relationship "filters" out some vertexes without introducing any new vertex.
To generalize it, we have:
\begin{lemma}
    $$V_k^{j} \subseteq V_k^{i} (j \geq i )$$ 
\end{lemma}
This observation is the core property of the prefix functions we use when we build \cache{}.
We will also use the following observation:
\begin{lemma}
For three finite sets $A$, $B$ and $S$, the following statements hold: \\
When $A \subseteq S$:
$$ A - B = A - (A \cap B) = A - (S \cap B) $$
$$ A \cap B = A \cap (A \cap B) = A \cap (S \cap B) $$
\end{lemma}  

\subsection{Graph Mini Introduction}
We use prefix optimization extensively so a prefix function can be partially computed by its own prefix function.
\begin{equation*}
    V_k^{i+1} = \begin{cases}
        V_k^i \cap N(v_{i+1}) &  E(v_k, v_{i+1}) \in E_p\\
        V_k^i - N(v_{i+1}) &  E(v_k, v_{i+1}) \notin E_p
    \end{cases}
\end{equation*}

The main idea of graph mini is to build a mini-graph for each prefix function.
The mini-graph stores a set of filtered neighbor sets and using the filtered neighbor sets will not affect the result of the prefix function.
We use $T$ to represent the materialized vertex sets in the mini-graph.
The first goal is to find $T(v_{i+1})$ such that it can replace $N(v_{i+1})$ as input for the computation while still preseving the results.
\begin{equation*}
    V_k^{i+1} = \begin{cases}
        V_k^i \cap T(v_{i+1}) &  E(v_k, v_{i+1}) \in E_p\\
        V_k^i - T(v_{i+1}) &  E(v_k, v_{i+1}) \notin E_p
    \end{cases}
\end{equation*}
Also, materializing $T(v_{i+1})$ will introduce overhead and the second goal is to ensure the benefits of using $T(v_{i+1})$ outweight its overhead.

% Each function can use an unique mini-graph or share a mini-graph with other functions.
% When compute the function, using the neighbor sets in the mini-graph as input should generate the same results compared to using the neighbor sets in the original graph as input.

% We implement \optimizer{} to do this automatically for a given schedule. 
% It traverses the prefix functions in the input schedule and determine if a function can use \cache{} and how. 
\subsection{Build Mini-Graph}
\begin{figure}
    \centering
    \includegraphics[width=.15\textwidth]{figures/Q2.pdf}
    \includegraphics[width=.15\textwidth]{figures/Q2am.pdf}
    \caption{Q2 Pattern and Schedule}
    \label{fig:Q2}
\end{figure}

\input{algorithms-old/prefixq2.tex}

We use one schedule for pattern $P_2$ as an example to discuss the methodology of building mini-graph. 
In this example, we follow the order specified in the figure \ref{fig:Q2} to match the pattern. 
(Note that the schedule is generated by GraphPi based on the input pattern and information of the graph data. 
For a given pattern, GraphPi might generate different schedules for different graphs.)

The black lines in the figure \ref{fig:Q2} connect vertexes with edges in the pattern graph and red lines connect vertexes without an edge in the pattern graph.
Intuitively. they represent the computation in the prefix function where a black line corresponds to a set intersection and a red line corresponds to set subtraction.
Its pseudo code can be found in algorithm \ref{algo:prefixq2}.
% Consider the computation required for materializing $V_6$: $$V_6 = N(v_2) \cap N(v_3) - N(v_1) - N(v_4) - N(v_5)$$
% With prefix optimization, we will materialize the loop invariant results $N(v_2) \cap N(v_3) - N(v_1) - N(v_4)$ and store them in $V_6^{4}$.

The first goal is to determine how to materialize the vertex sets in the mini-graph.
We use the computation for materializing $V_6$ at line 15 as an example to illustrate how we achieved this:
$$V_6 = V_6^{4} - N(v_5)$$ 
We need to find a vertex set $T(v_5)$ that can replace $N(v_5)$ for this computation while: 
$$|T(v_5)| \leq |N(v_5)| \: and \: V_6 = V_6^4 - T(v_5)$$
The key insight is we can build $T(v_5)$ by filtering $N(v_5)$ based on the prefix of $V_6$.
We can choose $T(v_5) = V_6^{i} \cap N(v_5) \: (i \leq 4)$ because:
\begin{proof}
    % \begin{lemma} 
    % For three finite sets $A$, $B$ and $S$, the following statements hold:
    % $$ A \subseteq S \implies A - B = A - (S \cap B) $$
    % \end{lemma}
    Given that $ V_6^4 \subseteq V_6^i \: (i \leq 4) $
    $$ V_6^{4} - N(v_5) = V_6^4 - (V_6^i \cap N(v_5)) = V_6^4 - T(v_5) $$
\end{proof}

Notice that this seemingly arbitrary filtering method turns out to be the optimal method for reducing the size of $T(v_5)$.
$V_6^{i}$ is the most selective set that contains all elements in $V_6^{4}$ when $v_{i+1}$ has not been added to the partial match.
This is because prefix set $V_6^{4}$ is computed based on the edge relationship between $v_6$ and $[v_1, \ldots, v_4]$.
We cannot further reduce the size of $V_6^i$ without knowing $v_{i+1}$.  
% This observation is also true for why $V_5^{j}$ is the most selective set that contains all elements of $V_5$ at the $j^{th}$ loop.
% \item $T(v_5)$ is the smallest replacement we can choose: 
% \begin{proof}
%     If there exists a vertex x such that: $x \in  V_6^{4} \cap N(v_5)$ and $ x \notin T(v_5)$.
%     It implies that $x \in V_6 - T(v_5) \: and \: x \notin V_6 - N(v_5)$ and $T(v_5)$ cannot preserve the results.
% \end{proof}
The second goal we have is to ensure the benefit of using $T(v_5)$ outweighs the overhead of materializing $T(v_5)$.
We need to materialize $T(v_5)$ by computing $T(v_5) = V_6^{i} \cap N(v_5)$ and this computation can be more expensive than computing $V_6 = V_6^{4} - N(v_5)$ directly.

If we set $i = 4$, we can only use each $T(v_5)$ for materializing one instance of $V_6$.
This is because $V_6^{4}$ is computed based on edge relations between $v_6$ and the partial matching $\{v_1=a, v_2=b, v_3=c, v_4=d\}$.
We might have the same vertex id assigned to $v_5$ in the partial match but that can only happen if the partial matching of $\{v_1, v_2, v_3, v_4\}$ get changed.
We will need to compute $T(v_5) = V_6^{4} \cap N(v_5)$ again for the same $v_5$ because $V_6^{4}$ becomes different.

Intuitively, we want to materialize $T(v_5)$ inside an upper loop to reuse the results for multiple times.
We can set $i < 3$ so we might be able to use it when we materialize $V_6$ with the same $v_5$ in the partial match but different $\{v_{i+1}, v_{i+2}, \ldots, v_{4}\}$. 

% We now face two challenges: 
% \begin{enumerate}
%     \item $V_5$ and $V_6^{4}$ have not been computed at an upper loop. We need to use other information to compute $T(v_5)$.
%     \item Which $v_5$ will be used for multiple times when materialize $V_6$ is difficult to predict.
% \end{enumerate}
We have partially achieved our two main goals. 
The remaining question is which $v_5$ we will encounter when we materialize $V_6$.
In fact, it is difficult to predict this because we haven't compute $V_5$ yet when materialize $T(v_5)$.
However, we can obtain the range of $v_5$ when we build the mini-graph.
We know that $V_5 \subseteq V_5^{i} \: (i \leq 3)$ as shown in lemma 1.
Instead of guessing which $v_5$ will be used to materialize $V_6$, we simply materialize $T(v_5)$ for all vertexes in $V_5^i$.
We use a mini-graph instance to store and manage all the materialized $T(v_5)$. 
This mini-graph guarantees to contain all the vertex sets required to replace $N(v_5)$ for computing $V_6$. 
% $$E(v_k, v_j) \in E_q \implies V_k^{j+1} = V_k^{j} \cap N(v_j) \:\:\: (k > j + 1)$$
% $$E(v_k, v_j) \notin E_q \implies V_k^{j+1} = V_k^{j} - N(v_j) \:\:\: (k > j + 1)$$
% The way we compute the prefix set shows that for the vertex set $V_k$, its prefix set at an upper loop must contains all the elements of its prefix set in the inner loop.
% The key observation is we can use prefix of $V_5$ to determine the range of $v_5$.
% Claim 1: $\forall v_5 \in V_5 : v_5 \in V_5^{i} (i \leq 3)$
% \begin{proof}
%     $$V_5 \subseteq V_5^{i} \implies \forall v_5 \in V_5 : v_5 \in V_5^{i} $$
% \end{proof}
% Claim 2: $V_6^{4} - (V_6^4 \cap N(v_5)) = V_6^{4} - (V_6^j \cap N(v_5)) (j < 4)$
% \begin{proof}
%     Using lemma 1
% \end{proof}

\input{algorithms-old/cacheq2.tex}
One possible implementation with mini-graph enabled is illustrated in Algorithm \ref{algo:cacheq2}.

We have discussed a particular prefix function that computes set subtraction of two sets $V_6^{4}$ and $N(v_5)$.
We now generalize the use of mini-graph to any prefix function.

We observe that a prefix functions can only involve set intersection and set subtraction. 
Given a prefix function that materialize $V_k^i$
The method we used to accelerate set subtraction in the case of materializing $V_6$ can be used to accelerate set intersection too.
In fact, all prefix functions in the schedule can be expressed as set intersection or set subtraction between some sets and therefore can potentially be accelerated using this method.
\begin{equation*}
    V_k^{i+1} = \begin{cases}
        V_k^i \cap N(v_{i+1})   = V_k^i \cap (V_k^j \cap N(v_{i+1})) \: (j \leq i) &  E(v_k, v_{i+1}) \in E_p \\
        V_k^i - N(v_{i+1})      = V_k^i \cap (V_k^j \cap N(v_{i+1})) \: (j \leq i) &  E(v_k, v_{i+1}) \notin E_p
    \end{cases}
\end{equation*}
To accelerate the computation of $V_k^i$, we first compute $T(v_{i+1}) = V_k^j \cap N(v_{i+1})$.
To allow reuse of the results, we set $j \leq i - 1$. 
That concludes the basis methodology for building the mini-graph.

\subsection{Heuristic Model}
We use a simple heuristic model to decide how to build mini-graph when there are multiple valid choices. 
In the above example, when building mini-graph for storing $T(v_5) = V_k^j \cap N(v_{i+1}) \: (j \leq i)$, we can let $j = 1, 2, 3$.
We observe that $i=1$ is not a valid choice because we won't materialize $V_6^1$ in the first place.
This is because $V_6^1 = V - N(v_1)$ and $V_6^1$ might contain all the vertexes in the graph, which does little help for computing $V_6^2$.
Similarly we need to check $V_5^{i}$ has been materialized as well.
Both $i=2$ and $i=3$ can be valid choice. 
We would always set $i$ to be the larger value because it ensures the result of $T$ is most selective.
However, this method does not guarantee the best performance as we will build the mini-graph more frequently.
We leave this part to the future work.

\subsection{Mini-Graph}
When build the mini-graph, its domain set $D$ and the superset $S$ must have been materialized.

We use the CSR layout to represent mini-graphs in the main memory. 
This means the neighbor sets of the mini-graph are stored in a contiguous array.

We implement the intersection algorithm using the scan and merge method, hence the output is also sorted.
To build a mini-graph, we iterate through the vertexes in the domain set and retrieve each vertex's neighbor set in the original graph. 
Then, the result of the intersection between the vertex's neighbor set and the superset will be appended at the end of $edges$.

We index the neighbor sets to quickly find the starting point of a given vertex's neighbor set in the $edges$.
To do so, we use an array $pos$ that is of the same size of the domain set $D$. 
The $i^{th}$ element in $pos$ index the neighbor set of the $i^{th}$ vertex in the domain set. 
To retrieve a vertex's neighbor set in the mini-graph, we can use binary search to find its index in the domain set.
The neighbor set's starting point is $pos[i]$ and its length is $pos[i+1] - pos[i]$.
However, we can retrieve all indexes in the subsequent computations using linear scan as well. 
In the case of Q2, we can intersect $V_5$ with the domain set of $G_{min}$ to get all indexes of $v_5$ in the subsequent computation.

We allocate small amount of memory for $pos$ and $edges$ using "malloc" at the start of execution. 
When the $edges$ or $pos$ is full, we enlarge the size of the memory using "realloc". 
In this case, we can simply overwrite the $edges$ and $pos$ to reuse the memory.

% To build a mini-graph for function $F_k^{j+1}$, \optimizer{} needs to find a superset $S_{v_k}^i$ contain all possible vertices in $V_k^{j}$.
% This observation encourages us to use the most selective set that includes all possible $v_k$ in $V_{k}^j$. 
% At the $i^{th})$ loop, this set is $V_k^i$. 

% \subsection{Domain Set}
% $D_{v_j}^i$ should have as many input vertices as possible while excluding the vertices that definitely won't be used as input for $F_{k}^{j+1}$.

% It encourages us to use the most selective set that includes all possible input vertex $v_i$ for the optimized function $F_{k}^i$. 
% At the $i^{th}$ loop, this set is $V_j^i$. 

% The reason is simlar for determing the superset. $F_j^i$ defines the relation between $v_j$ and $[v_1, \ldots, v_i]$.
% Without obtaining the value of $v_{i+1}$ at the $i^{th}$ loop, we have no more information to obtain a more selective domain set.
% Thus, we use $D_{v_j}^i$ as the domain set to build the mini-graph for $F_{k}^{j+1}$ in the $i^{th}$ loop. 


% \subsection{Building mini-graph}
% We first discuss what information the optimizer needs to build a mini-graph.
% Recall that in 4-clique counting, \ao{maybe use a different example? I think we decided in NOTI to avoid cliques as they're extensively studied and this is more general} we choose to cache the result of $N(v_1) \cap N(v_3)$ at loop level one because we have the following information from the pattern and schedule:
% \begin{enumerate}
%     \item $V_4$ is a subset of $N(v_1)$. 
%     \item The search space of $v_3$ is a subset of $N(v_1)$. 
% \end{enumerate}
% We denote $S_{V_4}^1$ as a superset of $V_4$ at the $1^{st}$ loop.
% We denote $D_{v_3}^1$ as the domain set of $v_3$ at the $1^{st}$ loop.
% A mini-graph is based defined by a $D$, a $S$ and a set of neighbor sets $N(u)$. 
% $D$ include all the vertices in the mini-graph.
% Each neighbor set in the mini-graph is a subset of $S$, since it is computed by intersecting $S$ and one of the $N(u)$.
% In this case, both $D_{v_3}^1$ and $S_{V_4}^1$ can be set to $N(v_1)$ for building the mini-graph that optimize $F_4$.


% \subsection{Cost Model}
% Simply analyzing domain set and superset would encourage us to build the mini-graph in all scenarios.
% But building the mini-graph can introduce overhead. It is only worth to do when its benefits outweight its cost.

% A shortcut for solving this problem is manually set the mini-graph to be at least two levels above the function being optimized.
% This idea is based on the assumption that the expected number of times each neighbor set in the mini-graph being computed and reused is super-linear to the loop level.
% In addition, the domain set and the super set must be a subset of some neighbor sets. 
% If the domain set can include all vertexes in the graph, the overhead of building the mini-graph is too large and it might consume too much memory.
% If the superset can include all vertexes in the graph, using the neighbor set in it is the equivalent compared to using the orginal neighbor set.

% However, this method does not evaluate the overhead of building the mini-graph. It might cause the new algorithm as a whole to be slower. 
% To solve this problem, we use a cost model to analysis this overhead and the potential speedup it brings. 

% \jl{Todo: finalizing cost model}
% We use a simplified model to estimate the cost of building a mini-graph $G_{min}(D, S)^i$ with domain set $D$ and superset $S$ at the $i^{th}$ loop.
% Building one mini-graph needs to compute the set intersection between $S$ and all the neighbor sets of the vertices in $D$.
% We can estimate it using:
% $$ Cost(D, S) = \sum_{\forall u \in D} (|N(u)| + |S|) $$

% We also assume the graph is random so the expected degree is $\frac{2|E|}{|V|}$.
% % So this cost formular can be also written as:
% % $$ Cost(D, S) = |D| \times (\frac{2|E|}{|V|} + |S|) $$
% % $$ Cost(D, S, i) = \prod_{1 \leq t \leq i}|V_t| \times Cost(D, S)$$
% Note that to optimize function $F_k^{j+1}$, we will set $D = V_j^i$ and $S = V_k^i$ at the $i^{th}$ loop.
% Also, the mini-graph is built at the $i^{th}$ loop, we should consider the number of times it will be built.
% So the cost of building the mini-graph would be:
% $$ Cost(D_{v_j}, S_{v_k}, i) = \prod_{1 \leq t \leq i}|V_t| \times |V_j^i| \times (\frac{2|E|}{|V|} + |V_k^i|) $$
% We can estimate the orginal cost of function $F_k^{j+1}$ using:
% $$ Cost(F_k^{j+1}) = \prod_{1 \leq  t \leq j} |V_t| \times (|V_k^j| + N(v_{j+1}))$$
% and its optimized version:
% $$ Cost(opt\_F_k^{j+1} ) = \prod_{1 \leq  t \leq j} |V_t| \times (|V_k^j| + N_{new}(v_{j+1}))$$

% Before comparing the cost before and after using mini-graph, it remains to estimate the cardinality of the prefix sets and the new neighbor sets in the mini-graph.
% To do this, we modified the cost model in GraphPi.
% In our cost model, $p_1$ is the probability that two random vertices in the graph form an edge:
% $$p_1 = \frac{2|E|}{|V|^2}$$
% and $p_2$ is the probability that any two vertices in a common neighbor set form an edge:
% $$p_2 = \frac{tri\_cnt \times |V|}{(2 \times |E|)^2}$$
% which is derived from the idea that: 
% $$E(tri\_cnt) = |V| \times (\frac{2 \times |E|}{|V|})^2 \times p_2$$
% We assume the number of triangles is given like GraphPi does.

% Recall that prefix sets and new neighbor sets are formed by set intersection and set subtraction of some neighbor sets.
% Both can be abstracted into a function that defines the relationship among some neighbor sets using set intersection and set subtraction.

% We name the function $F$, its result $R$, the set of vertices $Q$ that defines the neighbor sets to compute the function.
% We define the first vertex in $Q$ that has a neighbor set corresponds to set intersection $v_{base}$, and $R$ is a subset of $N(v_{base})$.
% If the function has only subtraction then the cardinality of its result is set to $|V|$.
% In real graphs, $|V| >> |N(v_{base})|$. 
% We should avoid computing the functions with zero neighbor set to intersect with.
% It won't prevent getting the results. Because the input pattern is connected and every non-prefix function should at least have one neighbor set to intersect with.
% It will prevent us from computing the prefix functions that brings overhead.

% We partition the vertices in $Q$ except for $v_{base}$ into two sets $U, T$ such that $\forall u \in U: E(u, v_{base}) \in E, \forall t \in T: E(t, v_{base}) \notin E$.
% We then count the number of vertices in $U$ and $T$ that correspond to set intersection $i_u$ and $i_t$ respectively.
% The cardinality of $R$ is estimated using the following formular:
% $$ |R| = \frac{2\times|E|}{|V|} \times (p_1)^{i_t} \times (1-p_1)^{|T| - i_t} \times (p_2)^{i_u} \times (1-p_2)^{|U| - i_u}  $$
% \jl{will update this part after test it out}


% % \cache{} works better when:
% % \begin{enumerate}
% %     \item It's often the case that $ | C \cap B | << |B| $.
% %     \item The result of $C \cap B$ can be used for multiple times.
% %     \item $ Deg(v) << |V| $ for most $v$ in the graph.
% % \end{enumerate} 
% % \cache heavily relies on the first assumption to bring a speed-up. 
% % Also, some reasoning for \cache{} relies on the third assumption and we will explain them in the following sections.

% % In a nutshell, \cache{} computes the intersections between a superset with some neighbor sets. The superset acts like the set C and the neighbor sets are set B in the above formular. 

% % The \cache{} optimization is complementary to the prefix optimization. It filters the neighbor sets that the prefix optimization does not. It can also work in orthogonal with offline indexing which convert input sets from sorted integers into a more efficient layout. 

% % We now discuss how the \optimizer{} works in two phases.

% \subsection{Prerequisite}
% \optimizer{} needs to be built on top of AutoMine. Recall that AutoMine uses the function $F_k$ to compute $V_k$ and $F_k^{p}$ to compute the prefix sets for $V_k$. Note that $F_k$ is essential $F_k(k)$. We can relax the constraint so the function $F_k^{p}$ defines all $F_k$’s operation on $v_1, v_2, \ldots,v_{p} (p<=k)$. A schedule for a pattern of size n is equivalent to a list of functions: 
% $$F_1(1), F_2(1), \ldots, F_n(1), \ldots, F_n(n)$$ 

% These functions will generate a list of results:
% $$V_1^1, V_2^1, \ldots, V_n^1, \ldots, V_n^n$$

% The precomputation optimization tries to optimize each of the function in the schedule by replacing the neighbor sets with the precomputed sets. Prefix sets cannot be further optimized so they are kept the same. 

% This optimization takes place in two phases. In the first phase, \optimizer{} identifies the functions in the list to optimize and the \cache{} required. 
% In the second phase, \optimizer{} generates efficient code by inserting the \cache{} at the corresponding loop and rewrites any of $F_k$ or $F_k^{p}$ that can use the pre-computed results.

% \subsection{ Phase I }
% In the first phase the \optimizer{} identifites the optimization opportunities for each function in the schedule. The functions can be categorized into two main categories:
% \begin{enumerate}
%     \item The cmoputation of the function is simply an assignment. For example, $F_1$ always return all vertices in the graph. 
%     \item The computation of the function envolves set operations. The input sets can be a prefix set and one or many neighbor sets.
% \end{enumerate}
% \optimizer{} iterates through all the functions in the schedule. If the function belongs to the first category than there is no need for optimization. 

% For each function $F_k^{p}$ that falls in the second category, \optimizer{} iterate through its inputs $N(v_m)$ and tries to find a set of values $\alpha, \delta, \beta$ that satisfy the following requirements:
% \begin{enumerate}
%     \item $v_{p-\beta}$ connects to $v_k$ and $(p \geq \beta \geq \alpha)$
%     \item $v_{p-\delta}$ connects to $v_{m}$ and $(p \geq \delta \geq \alpha)$
%     \item $ \alpha >= 2 $
% \end{enumerate}
% If there is no valid result, \optimizer{} will analyze the next function in the list. If there exists one or multiple results, \optimizer{} will store $(k, p, m, \max(\alpha))$ in memory. We call it the metadata for a \cache.
% \optimizer{} keeps doing so until it iterates through all the functions in the list.

% We now explain the intuition of this algorithm.

% Recall that the \cache{} computes the intersections between a superset with some neighbor sets. 

% To optimize $N(v_m)$, \optimizer{} needs to first find a set $C$ for computing the intersections with $N(v_m)$ the in an upper loop where $C$ is a superset for $V_k^{p}$. 

% The selection of $C$ can greatly influence the efficiency of the pre-computed result. For example, an extreme case is using the set that contains all vertices in the graph. It always provides the correct result but the \cache{} here is purely redundant.

% We observe that the prefix sets of $V_k^{p - \alpha} \space (p \geq \alpha \geq 0)$ can be used as the superset $C$. By definition $ V_k^{p} \subseteq V_k^{p - \alpha} $. Moreover, $V_k^{p - \alpha}$ is computed based on the relationship between $v_k$ and $v_1, v_2, \ldots, v_{p - \alpha}$. When \optimizer{} insert pre-computaion at level $p - \alpha$, it cannot determine the value of $v_{p - \alpha + 1}$ or increase the prefix set's selectivity. $V_k^{p - \alpha}$ turns out to be the most selective superset for $V_k^{p}$ at $(p - \alpha)^{th}$ loop. 

% However, $V_k^{p - \alpha}$ can contain all the vertexes in the graph. This occurs all the vertices determined $v_1, v_2, v_{p - \alpha} $ do not connect to $v_k$). 
% \optimizer{} needs to check if there exists $\beta \space (\beta \geq \alpha)$ such that $v_{p-\beta}$ is connected to $v_k$. 
% The existance of such $v_{p-\beta}$ indicates that $ V_k^{p - \alpha}$ is a subset of $v_{p-\delta}$'s neighbor set: $ V_k^{p - \alpha} \subseteq N(v_{p - \beta)} $.
% This generates the first requirement.

% On the other hand, \optimizer{} also need to have enough information to determine the domain of $v_{m}$ when insert the \cache. We observe that for a fixed $v_{p-\alpha}$, the domain of $v_{m}$ is a subset of $V_{m}^{p-\alpha}$. Using the same analysis, we can conclude that using $V_{m}^{p-\alpha}$ as the domain for $v_{m}$ is the best \optimizer{} can do. It also implies that there must exist $\delta \space (\delta > \alpha)$ such that $v_{p-1}$ is connected to some $v_{p-\delta}$. The presence of the $v_{p-\delta}$ implies that $V_{m}^{p-\alpha} \subseteq N(v_{p - \delta})$. This generates the second requirement.

% The third requirement is a herustic value for $\alpha$. It is used to ensure the pre-computed results will be used for multiple times. However, for sparse graphs that have less $\alpha$-clique compared to $(\alpha - 1)$-clique, this value needs to be changed.

% [Fig algorithm I, identify precomputation opportunity, insert results]
% \jl{ this section might have too many variables, difficult to understand}

% \subsection{ Phase II }
% In the second phase, \optimizer{} iterates through the set of $(k, p, m, \alpha)$ computed in the previous phase and insert the \cache. 

% The \cache{} operation can be described as the following:
% $$P(C, D) = \forall v \in D: N(v) \cap C $$
% $P$ defines the \cache{} operation. It takes two inputs: $C$ is the superset and $D$ is the domain set, where $C$ is a superset for $V_k^{p}$ and $D$ is contains all possible $v_m$ in the subsequent computation.

% Given a tuple $(k, p, m, \alpha)$, \optimizer{} inserts the intersection inserts $P(V_k^{p - \alpha}, V_m^{p - \alpha})$ at the end of the $(p - \alpha)^{th}$ loop. 
% It stores the result in $T_i$ for each \cache. We will discuss the implementation detail of function $T_i$ in the next section.

% It then iterates the functions and generates code that replace the neighbor set with the pre-computed set. 
% Note that \optimizer{} will use the metadata to determine which neighbor sets can be replaced. 
% Given a function $F_k^{p}$, for each input neighbor set $N(m)$, \optimizer{} scans all the metadata for the \cache{}. 
% It tries to find a \cache{} with $C$ that is a superset of $V_k^{p}$ and $D$ that contains all $v_m$. 
% \optimizer{} can use the same method in the identification phase to check these requirements.
% When a pre-computation is found, \optimizer{} replace the input set $N(m)$ with function $Pre(v_m, T_i)$ which returns a filtered $N(v_m)$ stored in $T_i$.

% [Fig Algorithm II, aggressively replace neighbor sets with pre-computed results]


 


==> sections-old/5-evaluation.tex <==
\section{Evaluation}
\begin{figure}
    \caption{Tested Patterns}
    \includegraphics[width=0.45\textwidth]{figures/patterns_bold.png}
\end{figure}% \jl{Working on the plots, current patterns are same to GraphPi except P1 (4-clique in our case), considering change P1 from 4-clique to 5-clique }

We evaluate the performance of the algorithm generated by the \optimizer{} in this section.

\subsection{Methodology}
\textbf{Platforms} We perform our evaluation on a server with dual Intel(R) Xeon(R) Silver 4216 CPUs and 128 GB of RAM.
All the programs are compiled with gcc 11.1 (-O3). We use OpenMP to achieve hyper-threading at the outer most loop.

\textbf{Datasets}
\input{tables/graph_info.tex}
We use 3 real-world graphs for evaluations as shown in Table \ref{graph_info}.


\subsection{Baseline}
For the baseline, we use the methodology from the state-of-the-arts to build the system.
The baseline system mainly has two components: the scheduler and the code generator.

The input to the scheduler is an abstract graph pattern with many possible traversing orders.
The scheduler needs to decide which order to follow in the subsequent computation.
It also needs to determine the restrictions apply to the vertexes for pruning all the automorphisms for.

GraphPi is the state-of-the-art in terms of schedule and restrictions generation.
Its has reported to achieve over an order of magnitude's speed up in terms of execution time compared to the other systems like GraphZero.

AutoMine is the state-of-the-art methodology for generating low level C++ code.
It is highly optimized for memory consumption and data locality.

To build the baseline system we use GraphPi as the default scheduler and AutoMine to generate efficient low level code.

For the data graphs, we assume the graphs fit in the main memory for our experiments.
We store the entire graph in CSR format and is read-only / immutable.
% In the low level, we use $edges$ to point to the sorted start of sorted neighbor sets.
% We use $pos$ array to store the starting point of each vertex's the neighbor sets.
% For example, the starting point of vertex $u$'s neighbor set can be retrieved by returning the pointer $edges + pos[u]$.
% The degree of $u$ can be computed by $pos[u+1] - pos[u]$.
We re-index the vertex ids to ensure that they are contiguous.
We also keep the relative magnitude of the vertexes for fair comparison.

For set operation, we implement both the set intersection and the set subtraction using a linear scan approach.
We also let the set operation terminates when a given upper bound is reached, which reduce the data access overhead caused by automorphisms.

The baseline method aggressively apply prefix optimization to generate the computation code.
However, it will skip the materialization of functions that take the all the vertexes in the graph as input.
These functions are the prefix functions for vertexes that do not have any connection with explored vertexes in the partial match.

\subsection{LOVE}
For comparison, \optimizer{} also aggressively apply prefix optimization. 
In addition, it greedily find opportunities of using mini-graphs to accelerate the materialization.
In our implementation. if there are more than one valid mini-graphs for a given function, \optimizer{} always build the mini-graph with the most selective superset.
Similarly, if there are more than one mini-graphs can be used to accelerate the computation of a given function, \optimizer{} would use the one with the most selective superset.
The rational is the more selective the superset, the shorter the input might be.

\subsection{Experiment Results}
\begin{figure*}[ht]
    \includegraphics[width=\textwidth]{figures/exec_time_1.pdf}
\end{figure*}
\jl{Working on the plots, current patterns are same to GraphPi except P1 (4-clique in our case), considering change P1 from 4-clique to 5-clique }
\jl{Working on the plots + experiments of multi-threads + top 5\% degree}


==> sections/0-abstract.tex <==
\begin{abstract}
    Finding all instances of a graph pattern in a larger data graph is a fundamental problem that underlies many common graph mining tasks. 
    The main bottleneck in graph pattern mining is performing set operations involving adjacency lists. 
    This paper explores a new direction to alleviate this bottleneck: \emph{proactively} pruning the adjacency lists \emph{online} during query execution.
    We show how to build \emph{minigraphs}-compact pruned versions of the input graph-and use them instead of the original input graph.
    We propose GraphMini, a graph pattern matching system that automatically generates pattern matching code leveraging minigraphs.
    Our evaluation shows that GraphMini can be combined with state-of-the-art graph pattern mining techniques to speed up query execution by up to one order of magnitude on commonly used benchmarks while using only minimal memory.
    
    % The study of structural patterns in graphs is fundamental to graph mining. Existing work has proposed a compilation-based system for handling graph mining problems. 
    
    % Here, the system uses a backtracking algorithm to match the subgraphs. It optimizes the backtracking algorithm based on the query pattern and the structural information of the data graph. 

    % In this paper, we revisit the methodology of current state-of-the-art computation plan. We observe that the approach suffers as the generated code from the existed system does not prune the adjacency lists to reduce redundant computation. Thus, we propose an online graph pruning technique to optimize the computation plan. It proactively prune the adjacency lists to speed up the computation. 
    
    % % In our experiments, this new technique contributes to at most 5x speedup.
\end{abstract}

==> sections/1-introduction.tex <==
\section{Introduction} \label{section:introduction}
Graphs represent and integrate large amounts of data in domains such as knowledge bases, finance, recommender systems, social networks, and biology. 
Several systems have been proposed and used to analyze graph data.
Graph computation algorithms such as PageRank~\cite{PageRank} or some shortest path algorithms can be expressed using message-passing between stateful vertices in a graph, a programming abstraction that is supported by Pregel~\cite{Pregel} and subsequent work.
Graph mining algorithms enumerate and process subgraphs in a graph, for example, motif counting or frequent subgraph mining. 
They are used in biology, chemistry, knowledge graphs, and social network analysis, and are supported by graph mining systems like Arabesque~\cite{Arabesque}.
Graph mining is very challenging since the number of possible patterns and subgraphs in a graph can be exponential in the size of the graph.
This is why we have seen a great interest in research on graph mining system that can support general graph mining applications at high performance~\cite{Arabesque, Graphflow, Fractal, RStream, GraphX, EmptyHeaded, AutoMine,GraphZero,GraphPi}.

This paper focuses on optimizing  \emph{graph pattern matching}, a step that represents the fundamental building block in state-of-the-art graph mining systems such as AutoMine, Peregrine, and GraphPi~\cite{AutoMine, Peregrine, GraphPi} and is also supported by systems like EmptyHeaded and Graphflow~\cite{EmptyHeaded, Graphflow}.
The problem of graph pattern matching consists of finding all subgraphs in an input graph, or \emph{data} graph, that match a given graph pattern, or \emph{query} graph. 
It involves performing repeated set operations (intersections and subtractions) among the adjacency lists of the vertices in the input graph to find the data vertices that match the query vertices.
Existing work has shown that set operations represent the computational bottleneck in graph pattern matching.
State-of-the-art graph mining systems alleviate this bottleneck with several optimizations that target \emph{query scheduling} or \emph{query execution}.

Query scheduling occurs before the actual execution of a pattern matching query. 
Given a query, a scheduling algorithm optimizes the order in which query vertices and edges are matched.
The goal is to \emph{minimize the number of set operations} executing during the matching process.
GraphZero and GraphPi are two recent examples of scheduling algorithms.
A related problem to query scheduling is finding symmetries in the query graph.
Given a query and a schedule, it is possible to identify canonicality checks that filter out automorphic matches, that is, redundant copies of the same matching subgraph where vertices appear in a different order.
This reduces the number of matches and partial matches that need to be considered during the matching process.
For example, work on GraphPi \cite{GraphPi} particularly focuses on finding efficient canonicality checks.

Query execution occurs after obtaining a query schedule and its canonicality checks.
Typical pattern matching algorithms are backtracking algorithms implemented as a sequence of nested loops.
State-of-the-art systems first generate query-specific pattern matching code given a query graph and then run it.
Each nested loop performs set operations on adjacency lists, and these operations represent the fundamental computational bottleneck of pattern matching.
Prior work has observed that some set operations are \emph{loop-invariant}: they are executed repeatedly in a loop but they could be moved outside of the loop body without changing the semantic of the program~\cite{AutoMine}.
An effective optimization to minimize the number of set operations during query execution is thus to \emph{move up loop-invariant set operations} to the shallowest possible loop so that they can be executed only once.
This can be seen as a type of loop-invariant code motion, a technique used in compilers. 

This paper explores a new class of query execution optimizations: \emph{proactively pruning the data graph online during query execution}.
More specifically, we show how to \emph{prune} the adjacency lists of a graph, store them in compact data structures called \emph{minigraphs}, and use them as input for \emph{future} set operations during query execution.
Reducing the size of the adjacency lists decreases the running time of set operations since the time complexity of the commonly used set operations is linear or super-linear to the size of their inputs.
Pruning is proactive because it prunes the adjacency list of vertices that have not yet been added to the current partial match. 

Proactive online pruning of the data graph requires solving several complex technical challenges to make sure that the cost of pruning can be amortized.
We need to identify which adjacency lists need to be pruned.
We must find pruning criteria that guarantee the correctness of the matching process while effectively reducing the size of the adjacency lists.
Finally, we need to manage multiple minigraphs efficiently with limited memory overhead.

We implement these techniques in GraphMini, a graph pattern matching system that generates query execution code.
Proactive online pruning complements existing optimizations: it can work with arbitrary scheduler and it leverages loop-invariant code motion.
Our evaluation using standard benchmarks shows that GraphMini can outperform the state-of-the-art graph pattern matching system by up to an order of magnitude.


==> sections/2-background.tex <==
\section{Background and Motivation}
\label{section:background}

We now formalize the problem of graph pattern matching and describe the workflow of state-of-the-art graph pattern matching systems.
Our work focuses on the code generation step of the workflow.
To describe our contribution, we must discuss query execution more in detail and show the limitations of existing optimizations.

% \jl{Move this example to later section}
% \begin{minipage}{\columnwidth}
%     \centering
%     \includegraphics[width=0.5 \linewidth]{figures/MiniGraph-P0.png}
%     \captionof{figure}{Subgraph for Matching $P_0$ with $b = M(v_1)$}
%     \label{figure:MiniGraph-P0}
% \end{minipage}

% The current state-of-the-art graph pattern mining algorithms are back-tracking algorithms that incrementally extend partial matches. 
% To determine the set of vertices to be matched to the query pattern, these algorithms perform set intersections and set subtractions on adjacency lists. 


% As we will explain in \ref{section:nested-loops}, these system rely on the fact that the edge and non-edge relationship between different query vertices can be converted into set intersections and set subtractions among the matched vertices' adjacency lists. 
% The central theme of many optimizations is reducing the number of set operations and the average time for each set operation. 

% Our approach aims at reducing the average time spend on set operation. However, we use a different approach compared to the previous efforts, which changes the low-level representation of the graph and re-ordering the data graph. Instead, we prune the input adjacency lists for set operations on the fly to speed up the set operation.
% Here is an example of we can prune adjacency lists while preserving the results. The figure \ref{figure:MiniGraph-P0} shows a data graph with 6 vertices and a query pattern $P_0$ consists of 4 vertices. When match vertex $b$ in the data graph to the vertex $v_1$ in the pattern graph, we know that $e$ and $f$ won't be part of the partial matching because they are not connected to $b$. Thus, we can safely ignore $e$ and $f$ after matching $b$ to $v_1$ and remove these vertices from the adjacency lists of $a$, $d$ and $c$.
% In figure \ref{figure:MiniGraph-P0}, the dashed lines highlight the removed edges and dashed circles highlight the removed vertices, and these vertices and edges are not relevant to the current partial match. The pruned graph contains all the vertices and edges required to match the subsequent query vertices. 
% As we will explain, the technique in this example can be derived from a more generalized framework. We will come back to this example soon.
% Since we build the technique on top of the existing optimizations, we will first discuss the optimizations that builds the foundations of our technique and explain how we generalize the pruning technique in section \ref{section:adj_pruning}. 

\input{tables/terms}
% \begin{itemize}
%     \item $G(V, E)$: the data graph.
%     \item $G_q(V_q,E_q)$: the query graph.
%     \item $v_i$: the $i^{th}$ query vertex ($v_i \in V_q$).
%     \item $u_i$: the vertex that matches to $v_i$ ($u_i \in V$ ).
%     \item $N(u_i)$: the adjacency list of $u_i$.
%     \item $S_i$: the set of candidate vertices matched to $v_i$.
%     % \item $S_i^j$: the $j^{th}$ prefix set for $S_i$ (more details in section \ref{section:prefix-optimization}). 
% \end{itemize}

\subsection{Problem Definition}
We now define the graph pattern matching problem described in~\cite{AutoMine,GraphZero}.
We refer to Table~\ref{table:terminologies} for a summary of the notation.

A subgraph $ G_s(V_s, E_s) $ of $G$ is \emph{isomorphic} to $G_q$ if there exists a bijection $M$ between the sets $V_q$ and $V_s$ such that:
\begin{equation}
    \forall v_i, v_j \in V_q:\: (v_i, v_j) \in E_q \iff (u_i, u_j) \in E_s
\end{equation}
where $u_i = M(v_i)$ and $u_j = M(v_j)$. 

The \emph{graph pattern matching} problem takes an input data graph $G$ and a query graph $G_q$ as input and outputs all subgraphs $G_s$ that are isomorphic to $G_q$ and guarantee that:
\begin{equation}
    \forall u_i, u_j \in V_s:\: (u_i, u_j) \in E_s \iff (u_i, u_j) \in E
    \label{eqn:vertex-centric}
\end{equation}

In this case, we say $G_s$ \emph{matches} $G_q$. 
Typically, we want to output a result set $R$ consisting of \emph{unique} subgraphs, that is, subgraphs that are not \emph{automorphic} to any other subgraph in $R$. 
Two subgraphs $G_s = (V_s,E_s)$ and $G'_s =(V'_s, E'_s)$ of $G$ are automorphic if and only if $V_s = V'_s$ and $(u,v) \in E_s \iff (u,v) \in E'_s$.


% We acknowledge there are two variants of the problem.
% In the \emph{vertex-induced} variant, given a subgraph $G_s$ of the data graph, we require $E_s$ to contain all the edges in $G$ where the end points are in $V_s$, that is:
% $$ \forall v_i, v_j \in V_s:\: (v_i, v_j) \in E_s \iff (v_i, v_j) \in E$$


\subsection{The Workflow of Graph Pattern Matching Systems}
\label{sec:workflow}
State-of-the-art graph pattern mining systems like AutoMine and GraphPi adopt the workload depicted in Figure~\ref{figure:workflow}.
It goes through two main phases, query scheduling and query execution, which we describe in the following.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/pipeline.pdf}
    \captionof{figure}{General Workflow of Graph Pattern Matching Systems}
    \label{figure:workflow}
\end{figure}

\subsubsection{Query scheduling}
The input to the process includes an arbitrary query graph $G_q$.
The query graph only provides the query vertices and the edge relationship between vertices but does not specify in which order to match the query vertices. 
The system runs a scheduling algorithm to find a matching order for the query. 
The scheduler can also use statistics collected from the data graph and is somewhat analogous to a query optimizer in relational databases.
We use the notation $v_i$ to denote the query vertex in $V_q$ that has the $i^{th}$ position in the matching order.
We call the ordering of query vertices the \emph{query schedule}.

If the graph query is symmetrical there could be automorphic (i.e., duplicate) matches.
For example, suppose that the query graph of Figure~\ref{figure:workflow} has a match $G_s$ with vertices $[u_1, u_2, u_3, u_4]$ ordered according to the query vertex they match (i.e., $u_i$ matches $v_i$).
Because of the symmetry of the graph, the subgraph $[u_1, u_2, u_4, u_3]$ is also a match to $G_q$, as is $[u_2, u_1, u_4, u_3]$.
However, we only want to output one canonical match among all these automorphic matches.
One option would be to materialize these matches and then filter them out.
Better yet, we could filter \emph{partial} symmetrical matches during the query execution to save the cost of materializing full matches only to discard them later.

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{figures/automorphism-P0.png}
%     \captionof{figure}{Automorphic Matchings For $P_0$}
%     \label{figure:Automorphism-P0}
% \end{figure}

To perform this pruning, the scheduler generates a set of \emph{canonicality checks}, which are rules to prune symmetrical matches.
In the example of Figure~\ref{figure:workflow}, the scheduler can require the id of a vertex matching $v_1$ to be smaller than the id of a vertex matching $v_2$.
Similarly, it can require that $v_3 < v_4$.
In the previous example if the id of $u_1$ is smaller than the one of $u_2$ and $u_3$ is smaller than $u_4$, then only the match $[u_1, u_2, u_3, u_4]$ will be canonical among its automorphisms.

Applying canonicality checks helps to reduce the number of set operations. 
A scheduler needs to determine the optimal combination of the matching order and canonicality checks for a given query graph based on the data graph. 
The resulting canonicality checks are specific to the order used to match the query vertices. 

\subsubsection{Query execution}
With a query schedule, it is possible to start executing the query on the data graph.
Rather than running the query plan using a pre-compiled query execution runtime, state-of-the-art graph pattern matching systems \emph{generate query execution code} that is specific to a query, its schedule, and its canonicality checks.
Then the query execution code is compiled and executed on the data graph to produce matches.
Code generation and compilation are very fast and the extra overhead is offset by the speedups of running query-specific code.

The final output of the query executor is a set of matches.
General graph mining systems like Arabesque offer programming APIs that enable users to perform arbitrary user-defined functions on the subgraphs of a graph. 
Arabesque, however, mines subgraphs in a pattern-agnostic manner.
More recent work such as Automine and Peregrine has shown that a more efficient approach to support general graph mining applications is to first run graph pattern matching and then execute user-defined functions of the matching subgraphs.
In this paper, we simply consider the problem of finding matches and passing them to an \emph{emit} procedure, which we see as a black box.

\subsection{Query Execution: Basic Backtracking Algorithm} \label{section:nested-loops}
The contributions of this paper focus on code generation.
We now describe the current approaches to code generation and then discuss the limitations of existing work.

Existing systems generate code that matches patterns using a back-tracking algorithm implemented as a sequence of nested loops. 
In this approach, the body of the nested loop at depth $i$ executes on a partial match $I_i=[u_1, \ldots, u_i]$ consisting of vertices of the data graph.
It then performs set intersections and subtractions on the adjacency lists of the vertices in the partial match to compute the set $S_{i+1}$ of candidate vertices that match $v_{i+1}$. 
The next loop then iterates over each $u_{i+1} \in S_{i+1}$ to build the partial match $I_{i+1}=[u_1, \ldots, u_{i+1}]$. 

An example of query execution code for the query graph of Figure~\ref{figure:workflow} is shown in Algorithm~\ref{algorithms:Q1}.
The query graph has four vertices, which correspond to four nested loops.
The first query vertex $v_1$ can be matched to any vertex in $V$.
Therefore the set of candidates $S_1$ is $V$, and the first loop iterates over all candidates $u_1 \in S_1$.
The body of the first loop executes on a partial match $I_1 = [u_1]$ and accesses the adjacency list $N(u_1)$ to build the set of candidates $S_2$ that match $v_2$.
The second loop then iterates over all $u_2 \in S_2$ and computes set operations on $N(u_1)$ and $N(u_2)$ to find the candidate set $S_3$ that match $v_3$, and so on.

\input{algorithms/Q1}

The code generator needs to determine which specific set operations are required to compute the candidate set at each loop.
Based on the order, the generator checks the connections between the next vertex to be matched and all the previously matched vertices to generate the corresponding set operations.

More precisely, consider computing the candidate set $S_i$ at the nested loop at depth $i-1$.
The algorithm has already found an instance of partial matching $I_{i-1}= [u_1, \ldots, u_{i-1}]$. 
% To into set intersections and set subtractions among adjacency lists. 
The set of the candidate vertices $S_i$ contains the data vertices matching the query vertex $v_i$.
It is computed by performing set operations on the adjacency lists of the vertices in $I_{i-1}$ that have already been matched.
To determine these set operations, the code generator analyzes the connections between $v_i$ and the vertices in the query graph that have already been matched, $[v_1, \ldots v_{i-1}]$.
The generator partitions the vertices of $I_{i-1}$ into two sets $I_T$ and $I_F$ such that:
\begin{gather}
    \forall u \in I_T: u = M(v_j) \text{ and } (v_j, v_i) \in E_q \notag\\
    \forall u \in I_F: u = M(v_j) \text{ and } (v_j, v_i) \notin E_q  \label{equation:partition-partial-matching-candidate}
\end{gather}

Then, $S_i$ is then computed as:
\begin{equation}
    \label{equation:func_1}
    S_i = V \cap \big( \bigcap_{u \in I_T} N(u) \big) - \big( \bigcup_{u \in I_F} N(u) \big) 
\end{equation}
The above formula generalizes the computation for computing the candidate vertices in terms of set operations among the adjacency lists of the matched vertices.
In other words, if $v_i$ is connected with some previously matched vertices $v_j$, we can use set intersections to filter out the vertices in the candidate set $S_i$ that are not connected to $v_j$. Similarly, we use set subtraction to filter vertices in $S_i$ that are connected to $v_j$ if $v_i$ and $v_j$ are not connected in the query graph. 

In real graphs, the vertex set $V$ is usually many orders of magnitude larger than the largest adjacency list in the graph. 
To avoid using $V$ as input in the set operation, schedulers put a constraint on the ordering.
Each matched vertex $v_i$ must be a neighbor of some matched $v_j$ with $j<i$ unless it is the root vertex, that is, $i=1$. 
This constraint ensures that $I_T$ contains at least one vertex so the computation for $S_i$ becomes: 
\begin{equation}
    S_i =  \bigcap_{u \in I_T} N(u) - \bigcup_{u \in I_F} N(u) \label{eqn:naive_candidate_computation}
\end{equation}

Algorithm~\ref{algorithms:Q1} shows an example of using Eqn.~\ref{eqn:naive_candidate_computation} to find candidate sets.
For example, when finding the candidate set $S_4$, we must look at the vertex set $v_4$ in the query graph.
The set operations must involve the adjacency lists of the vertices that have already been matched, which are in $I_3 = [u_1, u_2, u_3]$.
The query vertex $v_4$ is a neighbor of $v_1$ and $v_2$, so we intersect the adjacency lists $N(u_1)$ and $N(u_2)$.
Since $v_4$ is not a neighbor of $v_3$, we subtract the vertices in $N(v_3)$.
Once the algorithm finds a full match, it invokes the \emph{emit} procedure described previously.

% \subsubsection{Prioritizing Set Intersection}
% Rather than using set union, we can compute the result of the set intersections first, then subtract the adjacency lists of the vertices in $I_F$ one after another.
% By doing so, we only use set intersection and set subtraction to compute the new results, both computation can only produce results no larger then the biggest input. This optimization effectively reduces memory consumption. It also allows the system to pre-allocate the buffer required to store the results of the set operations based on the maximum degree of the vertices in the graph.

\subsection{Optimizing Query Execution} \label{section:prefix-optimization}
We now illustrate optimizations to the basic backtracking algorithm that have been proposed by existing work.
Next, we discuss further potential optimizations that are not exploited by existing work and that motivate our work.

\subsubsection{Prefix Sets}
Prefix sets are an effective optimization to the backtracking algorithm introduced by AutoMine~\cite{AutoMine}.
The fundamental insight is that some set operations executed in a loop are loop-invariant, that is, they can be brought outside the loop without changing the semantics of the program.

To see an example, consider again Algorithm~\ref{algorithms:Q1}.
Computing the candidate set $S_4$ requires computing, among others, the set intersection $N(u_1) \cap N(u_2)$.
This computation is performed in the loop at depth $3$, which iterates over $u_3$, but $u_3$ is not involved in the computation.
The set intersection $N(u_1) \cap N(u_2)$ is loop invariant because it can be computed outside of the third loop.
Moving the set intersection outside the third loop avoids executing it redundantly.
The result of the set intersection is called a \emph{prefix set} of $S_4$.

The prefix sets of the candidate sets can be, in principle, computed at each nested loop.
We use $S_i^{j}$ to denote the prefix set for the candidate set $S_i$ computed at the nested loop with depth $j < i$.
The set operations at loop $j$ can only consider the adjacency lists of the vertices in $I_j = [u_1, \ldots, u_j]$.
We partition $I_j$ into two sets $I_{j,T}$ and $I_{j,F}$ such that:
\begin{gather}
    \forall u \in I_{j,T}: u = M(v_k) \text{ and } (v_i, v_k) \in E_q \notag\\
    \forall u \in I_{j, F}: u = M(v_k) \text{ and } (v_i, v_k) \notin E_q  \label{equation:partition-partial-matching-prefix}
\end{gather}

Then, when $I_{j, T}$ is not empty, the prefix set $S_i^{j}$ can be defined by:
\begin{equation}\label{eqn:naive_prefix_computation}
    S_i^j = \bigcap_{u \in I_{j,T}} N(u) - \bigcup_{u \in I_{j,F}} N(u) 
\end{equation}

It follows from the previous equation and Eqn.~\ref{eqn:naive_candidate_computation} that the candidate set is equal to the last prefix set, so:
\begin{equation}
    S_i = S^{i-1}_i
\end{equation}

In a nested loop algorithm, we can compute prefix sets incrementally and use a prefix set computed in one loop to compute a prefix set in the next loop.
Therefore, we actually compute $S_i^{j}$ as:
\begin{gather}
      S_i^{j} = S_i^{j-1} \cap N(u_j) \quad \text{if} \quad (v_i, v_j) \in E_q \label{eqn:prefix_prefix_computation-1} \\ 
      S_i^{j} = S_i^{j-1} - N(u_{j}) \quad \text{if} \quad (v_i, v_j) \notin E_q 
\label{eqn:prefix_prefix_computation-2}
\end{gather}

%The current systems start to materialize the prefix set when $I_{j,T}$ is not empty, for same reason discussed in \ref{section:connected-ordering}. Then, it can use the materialized prefix sets to compute the prefix sets in the next loop.


Algorithm \ref{algorithms:Q1-Prefix} shows how to generate code leveraging prefix sets to optimize Algorithm \ref{algorithms:Q1}. 
Both algorithms use the same schedule shown in Figure \ref{figure:workflow} to generate the algorithm, but the latter is faster because it avoids executing set operations redundantly.
\input{algorithms/Q1-Prefix}

Prefix sets are \emph{materialized} only when they effectively restrict the scope of candidates for a query vertex.
Formally, we materialize a prefix set $S_i^j$ at loop level $j$ when the partial match $I_j$ contains at least one vertex $u_i$ such that $(v_j, v_i) \in E_q$. Since $u_i$ is matched to $v_i$, $S_i^j$ is a subset of $N(u_i)$ by Eqn.~\ref{eqn:naive_prefix_computation}. Doing so, we restrict the prefix set $S_i^j$ to be a subset of the adjacency list $N(u_i)$.

\subsubsection{Applying Canonicality Checks}
The canonicality checks identified by the scheduler can be used to stop set operations earlier.
For example, in Algorithm~\ref{algorithms:Q1}, when computing $S_2$ for a partial match $I_1 = [u_1]$, we can skip all elements of $N(u_1)$ with a vertex id larger than $u_1$.
This constraint is easy to enforce by simply sorting the adjacency lists by vertex id.
Similarly, when computing $S_4$ given a partial match $I_3 = [u_1, u_2, u_3]$, we can skip all candidates with a vertex id larger than $u_3$.

\subsection{Limitations of Existing Optimizations}
Existing optimizations have different purposes.
Prefix sets avoid executing the same set operations redundantly at deeper loops by bringing them up to higher loops. 
They reduce the \emph{number} of set operations executed during query execution.
An orthogonal direction is to reduce the \emph{running time} of the set operations.
Canonicality checks enable \emph{early stopping} of set operations in some cases, but they only help when a query vertex is symmetrical to others.

A potential online optimization that has not been explored by existing work is \emph{pruning} the graph, or more precisely its adjacency lists, \emph{before} set operations are executed.
The complexity of set operations is linear or superlinear to the size of the adjacency lists they take as input, so pruning the adjacency lists can substantially speed up execution.
Once pruned and stored, an adjacency list can be used in multiple set operations.
This approach is complementary to early stopping and does not require symmetry.

Our work explores the opportunities presented by online proactive graph pruning.
In the following sections, we discuss the technical challenges entailed in proactive online pruning and show how we address them.

==> sections/3-new-methodology.tex <==
\section{Criteria for Proactive Online Pruning} \label{section:graphmini}

In this paper, we present \cache{}, a graph pattern matching system.
The fundamental idea of GraphMini is to keep multiple compressed versions of the graph consisting of pruned adjacency lists, besides the input graph.
We call this data structure a \emph{minigraph}.
In this section, we discuss the criteria we use to build minigraphs.
Section~\ref{section:methodology} then discusses how GraphMini applies these criteria for code generation.

Minigraphs are built online during the execution of the backtracking algorithm which consists of a sequence of nested loops.
The fundamental purpose of minigraphs is that \emph{a minigraph built in a nested loop contains pruned adjacency lists that will be used as input for set operations in deeper nested loops.}
At each level of the nested loop, we use the information the algorithm has collected so far about partial matches to proactively build minigraphs.

Using a minigraph requires answering two fundamental questions, which we address in the following:
\begin{enumerate}
    \item Which adjacency lists should be pruned and added to the minigraph?
    \item How to prune these adjacency lists?
    %\item When and how to use minigraphs to speed up query execution?
\end{enumerate}

\subsection{Properties of Prefix Sets}
Before introducing minigraphs, we discuss some insights and useful properties of prefix sets, which were introduced in Section~\ref{section:prefix-optimization}.
We will leverage these properties to build minigraphs.
% Prefix sets represent a form of loop-invariant code motion that ``pulls up'' invariant set operations from lower to higher loops.

First, we argue that \emph{each prefix set for a query vertex is a superset of the candidate set of that vertex}.
The purpose of prefix sets is to restrict the set of vertices that could be potentially matched to a query vertex.
Consider two prefix sets $S_i^{h}$ and $S_i^{h+1}$ computed at loop $h$ and loop $h+1$ respectively.
We know that $S_i^{h+1}$ can be computed by subtracting $N(u_{h+1})$ from $S_i^h$ or intersecting $S_i^h$ with $N(u_{h+1})$ as shown in Eqns.~\ref{eqn:prefix_prefix_computation-1} and~\ref{eqn:prefix_prefix_computation-2}. 
In either case, the set operation only removes vertices from $S_i^h$. 
Therefore, we have that the following holds:
\begin{equation} \label{lemma-1}
    S_i^{h+1} \subseteq S_i^{h} \qquad \forall h,i:\: h + 1 < i
\end{equation}
which implies that:
\begin{equation}
    S_i^{f} \subseteq S_i^{h} \qquad \forall h,i,f:\: h < f < i
    \label{lemma-2}
\end{equation} 

The candidate set $S_i$ is equivalent to the prefix set $S_i^{i-1}$ as shown by Eqns.~\ref{eqn:naive_candidate_computation} and~\ref{eqn:naive_prefix_computation}. 
Therefore, we have that:
\begin{equation}
    S_i = S_i^{i-1} \subseteq S_i^h \qquad \forall h,i:\: h < i \label{eqn:superset_candidate}
\end{equation}
which amounts to say that each prefix set $S^h_i$ for a query vertex $v_i$ is a superset of the candidate set $S_i$ of that vertex.

% Consider the prefix set $S^h_i$ computed at loop depth $h$ in the previous example.
% the prefix set $S_i^{h}$ represents a \emph{superset} of the data vertices that will match future query vertices $v_i$ with $i > h$.
% In other words, for every partial match $[u_1, \ldots, u_i]$ obtained in the nested loops at depth greater than $h$, we know that $u_i \in S^h_i$. Formally,
% This because $S_i$ can be derived from $S_i^h$ by intersecting and subtracting the adjacency lists of $[u_{h+1}, u_{h+2}, \ldots, u_{i-1}]$ according to equation \ref{eqn:naive_candidate_computation} and \ref{eqn:naive_prefix_computation}. Since both set intersection and set subtraction only remove vertices from $S_i^h$ , the final result must be a subset of $S_i^h$.
% For the same reason, a query vertex $v_i$'s prefix set computed at a deeper loop is a subset of its prefix set computed at an upper loop. Formally,
% \begin{equation}
%     S_i^f \subseteq S_i^h \:\: (i > f > h) \label{eqn:superset_prefix}
% \end{equation}

The prefix set $S^h_i$ is actually the \emph{minimal superset of $S_i$ that can be computed based on the partial match available at loop $h$}. 
% Formally, we have that:
% \begin{gather}
%     \not\exists S \subseteq S^h_i: \: S = f(I_n) \text{ and } S_i \subseteq S
%     \label{eqn:minimal}
% \end{gather}
% where $f$ is a combination 
The loop at depth $h$ operates on the partial match $I_h = [u_1, \ldots, u_h]$.
The prefix set $S^h_i$ is the result of executing \emph{all} the set operations involving the adjacency lists $N(u_i)$ for all the vertices in $I_h$, that is, with $i \in[1,h]$.
Any prefix set $S^j_i$ with $j > h$ is obtained by performing set operations between $S^{j-1}_i$ and $N(v_j)$ (see Eqn.~\ref{eqn:prefix_prefix_computation-1} and~\ref{eqn:prefix_prefix_computation-2}). 
Therefore, $S^h_i$ is minimal at loop $h$ because to further remove any vertex from the prefix sets, we need to consider the adjacency lists of other vertices which will only be matched in deeper loops. 

\subsection{Selecting Adjacency Lists for the Minigraph}
As discussed previously, the purpose of a minigraph built at loop depth $h$ is to prune the adjacency lists used as input for set operations at loop depths greater than $h$.
Let $v_k$ be a query vertex matched in a deeper loop than $h$, with $k > h$.
Suppose that we want to build a minigraph to speed up the construction of the candidate set $S_k$ in deeper nested loops.
We want to prune and add adjacency lists which will be used in later set operations to compute $S_k$.
How can we identify these adjacency lists?

To answer this question we need to consider operations executed at three different depths of the nested loop indexed as shown in Table~\ref{table:depths}.
We call $h$ the depth of the loop where we want to build a pruned adjacency list to be added to the minigraph, and $k$ the deeper loop where we iterate over the candidate set $S_k$.
The other indices are related to the way we perform pruning and will be described in the following. 
Otherwise, we will use the same notation as in Section~\ref{section:background} (see Table~\ref{table:terminologies}).

To obtain $S_k$, we need to compute the set operations among the adjacency lists of vertices in the partial match $I_{k-1}=[u_1, \ldots, u_{k-1}]$, as shown in Eqn.~\ref{eqn:prefix_prefix_computation-1} and~\ref{eqn:prefix_prefix_computation-2}.
To speed up those set operations, we could prune the adjacency lists of the vertices in $I_{k-1}$.
Remember that we are considering building a minigraph at loop depth $h$ to speed up set operations of the nested loops with a depth greater than $h$.
At loop depth $h$, we have only matched the vertices in $I_h=[u_1, \ldots, u_h]$.
%We can only prune the adjacency lists of vertices in $I_h$ because the remaining vertices $[u_{h+1}, \ldots, u_k]$ are still unknown.

Unfortunately, pruning the adjacency lists of the vertices in $I_h$ at loop $h$ would not speed up the computation of $S_k$ in deeper nested loops.
At loop $h$ we can compute the prefix set $S^h_k$, which is a superset of $S_k$ as shown in Eqn.~\ref{eqn:superset_candidate}.
Because of the minimality property of prefix sets following from Eqn.~\ref{eqn:naive_prefix_computation}, we know that $S^h_k$ already incorporates the results of all set operations involving the adjacency lists of the vertices $[u_1, \ldots, u_h]$.
Pruning the adjacency lists of those vertices would not help to compute the candidate set $S_k$.

Pruning can speed up set operations at loop depth greater than $h$ only if applied to the adjacency lists $N(u_i)$ with $u_i \in [u_{h+1}, \ldots, u_{k-1}]$.
Before we discuss how to prune $N(u_i)$ we need to find $u_i$ in the first place.
The vertex $u_i$ is a match to a query vertex $v_i$, but the matching only occurs at a deeper loop level than $h$, the current level. 
The candidate set $S_i$ contains all vertices $u_i$ to be matched to $v_i$, but we don't have that set available at loop $h$. 
However, we know that the prefix set $S^h_i$ is a superset of $S_i^{i-1}$ because of Eqn.~\ref{eqn:superset_candidate}.
Therefore, the GraphMini adopts the following criterion to build minigraphs:
\begin{criterion}
At nested loop depth $h$, GraphMini prunes the adjacency lists $N(u)$ for each $u \in S^h_i$.
\label{crit-1}
\end{criterion}

\input{tables/loops}


\subsection{Our method of pruning the adjacency lists}
Now that we have established which adjacency lists to prune at loop depth $h$, we can discuss how to prune these lists.
As we will argue, we prune adjacency lists differently for different query vertices $v_k$ that we will match next.
Given an adjacency list $N(u_i)$, we call $N^h_k(u_i)$ the version of the adjacency list pruned at loop depth $h$ in order to find matches of $v_k$ more efficiently.

When using prefix sets, the set operations on the adjacency list $N(u_i)$ are computed at loop depth $i$.
The prefix set $S^i_k$ for $v_k$ is computed using either a set intersection (see Eqn.~\ref{eqn:prefix_prefix_computation-1}) or a set subtraction (see Eqn.~\ref{eqn:prefix_prefix_computation-2}), depending on whether $v_k$ is a neighbor of $v_i$ or not.

Consider first the case where $(v_i, v_j) \in E_q$ and we must compute $S^i_k = S^{i-1}_k \cap N(u_i)$ according to Eqn.~\ref{eqn:prefix_prefix_computation-1}.
How can we prune $N(u_i)$ to speed up this set operation while still preserving correctness?

By Eqn.~\ref{eqn:naive_prefix_computation}, each prefix set $S^j_k$ with $j < i$ is a superset of $S^{i-1}_k$.
In particular, since we are currently at loop depth $h$, we have $S^h_k$ and we know that $S^{i-1}_k \subseteq S^h_k$.

Let $N^h_{k,i}(u_i)$ be a set of data vertices computed as follows:
\begin{equation}
    N^h_{k,i}(u_i) = S^h_k \cap N(u_i)
    \label{eq:intersect}    
\end{equation}
We call the set $N^h_{k,i}(u_i)$ a \emph{pruned adjacency list} of $N(u_i)$ since $N^h_{k,i}(u_i) \subseteq N(u_i)$.
We can use this pruned adjacency to compute $S^i_k$ as follows:
\begin{equation}
    S^i_k = S^{i-1}_k \cap N^h_{k,i}(u_i) \quad \text{if} \quad (v_i, v_j) \in E_q
    \label{eqn:pruned-intersect}
\end{equation}

We now argue that replacing Eqn.~\ref{eqn:prefix_prefix_computation-1} with Eqn.~\ref{eqn:pruned-intersect} leads to the same value of $S^i_k$.

\begin{lemma}
    It holds that $S^{i-1}_k \cap N(u_i) = S^{i-1}_k \cap N^h_{k,i}(u_i)$ for each $h<i<k$.
    \label{lemma-3}
\end{lemma}
\begin{proof}
\noindent
The pruned adjacency list $N^h_{k,i}(u_i)$ is defined as $S^h_k \cap N(u_i)$ in Eqn.~\ref{eq:intersect}.
Therefore, we need to prove that $S^{i-1}_k \cap N(u_i) = S^{i-1}_k \cap S^h_k \cap N(u_i)$.
Since $h < i < k$, it follows from Eqn.~\ref{lemma-2} that $S^{i-1}_k \subseteq S^h_k$, so $S^{i-1}_k=S^{i-1}_k \cap S^h_k$.
\end{proof}

%This equation is correct since $S^{i-1}_k \subseteq S^h_k$ (see Figure \ref{figure:A_B}).

The GraphMini code generator can thus add the pruned adjacency list $N^h_{k,i}(u_i)$ to the minigraph and use it later to reduce the cost of computing set operations at loop depth $i > h$.
Instead of using Eqn.~\ref{eqn:prefix_prefix_computation-1}, we can replace $N(u_i)$ with a smaller pruned adjacency list $N^h_{k,i}(u_i)$.

A similar argument holds for the case where $(v_i, v_j) \notin E_q$ and we must compute $S^i_k = S^{i-1}_k - N(u_i)$ according to Eqn.~\ref{eqn:prefix_prefix_computation-2}.
In this case, we can compute $N^h_{k,i}(u_i)$ as:
\begin{equation}
    N^h_{k,i}(u_i) = S^h_k \cap N(u_i)
    \label{eq:subtract}    
\end{equation}
and $S^i_k$ as:
\begin{equation}
    S^i_k = S^{i-1}_k - N^h_{k,i}(u_i) \quad \text{if} \quad (v_i, v_j) \notin E_q
    \label{eqn:pruned-subtract}
\end{equation}

We can now replace Eqn.~\ref{eqn:prefix_prefix_computation-2} with Eqn.~\ref{eqn:pruned-subtract} and obtain the same value of $S^i_k$.
The correctness argument is analogous to Lemma~\ref{lemma-3} and can be proved similarly.

\begin{lemma}
    It holds that $S^{i-1}_k - N(u_i) = S^{i-1}_k - N^h_{k,i}(u_i)$ for each $h<i<k$.
    \label{lemma-4}
\end{lemma}

As discussed previously, at loop depth $h$ we don't know the exact set of vertices $u_i$ for which we need to prune $N(u_i)$.
However, we know that these vertices are included in the prefix set $S^h_i$.
According to Criterion~\ref{crit-1}, GraphMini computes a pruned adjacency list $N^h_{k,i}(u)$ of $N(u)$ for each $u \in S^h_i$ at loop depth $h$.
We now have two more criteria for using minigraphs:
\begin{criterion}
GraphMini computes the pruned adjacency list $N^h_{k,i}(u)$ at loop depth level $h$ for each $i,k$ such that $h<i<k$ using Eqn.~\ref{eq:intersect} or~\ref{eq:subtract}. \label{crit-2}
\end{criterion}
\begin{criterion}
GraphMini replaces Eqn.~\ref{eqn:prefix_prefix_computation-1} with Eqn.~\ref{eqn:pruned-intersect} and Eqn.~\ref{eqn:prefix_prefix_computation-2} with Eqn.~\ref{eqn:pruned-subtract} when computing prefix sets $S^j_k$ at all loop levels with depth $j \in [i,k)$. \label{crit-3}
\end{criterion}

% \subsection{Pruning Adjacency Lists With Set Intersection} \label{section:set-property}
% We use a property of sets to prune the adjacency lists. 
% \begin{lemma}
%     \label{eqn:set_property}
%     If $A \subseteq A^*$ and  $T = A^* \cap B$ then:  
%     \begin{gather}
%         A \cap B = A \cap T  \notag \\
%         A - B = A - T 
%     \end{gather}
% \end{lemma}

% \begin{minipage}{\columnwidth}
%     \includegraphics[width=0.9\linewidth]{figures/A_B.pdf}
%     \captionof{figure}{Set Intersection \& Set Subtraction}
%     \label{figure:A_B}
% \end{minipage}

% %\begin{minipage}{\columnwidth}
% %    \includegraphics[width=0.9\linewidth]{figures/A_subtract_B.pdf}
% %    \captionof{figure}{Set Subtraction}
% %    \label{figure:A_minus_B}
% %\end{minipage}

% Here, $T$ is a subset of $B$ as any element in $T$ must also in $B$. Since $T$ is a subset of $B$, computing set operations between $A$ with $T$ can be less expensive compared to computing set operation between $A$ and $B$.

% In the context of adjacency lists pruning:
% \begin{itemize}
%     \item $A$ corresponds the prefix set of $S_k^{i-1}$
%     \item $A^*$ corresponds to $S_k^h$
%     \item $B$ corresponds the original adjacency list $N(u_i)$
%     \item $T$ corresponds the pruned adjacency list $N_{k, i}^h(u_i)$
% \end{itemize}


% \spara{How to store minigraphs?}
% We have discussed how GraphMini prunes at loop depth $h$ the adjacency lists of vertices matched at lower loop depths.
% When GraphMini builds a minigraph at loop depth $h$, it uses it for all deeper nested loops.
% It then discards that minigraph at the next iteration at depth $h$ and rebuilds a new minigraph.

% A minigraph is the union of the adjacency lists computed at that depth. 
% More specifically, a minigraph $M^h$ computed at loop depth $h$ is the union of all pruned adjacency lists $N^h_{k,i}(u)$ for each $k,i$ such that $h < i < k$ and for each $u \in S^h_i$.

% Minigraphs are built incrementally based on the minigraph of the current outer loop.
% For example, the minigraphs at loop depth $h$ are built based on the minigraph at loop depth $h-1$.
% Specifically, suppose that we need to compute $N^h_{k,i}(u)$ using Eqn.~\ref{eq:intersect}.
% The minigraph in the outer loop contains a pruned adjacency list $N^{h-1}_{k,i}(u)$ for $N(u)$.
% Therefore, we can now compute $N^h_{k,i}(u)$ as:
% $$
% N^h_{k,i}(u) = S^h_k \cap N^{h-1}_{k,i}(u)
% $$

% The minigraph for the outer loop must have an entry $N^{h-1}_{k,i}(u)$ for vertex $v$.
% In fact, a minigraph at depth $h$ has pruned adjacency lists for each $u \in S^h_k$ and we know that $S^h_k \in S^{h-1}_k$.

==> sections/3-overview.tex <==
\section{Overview Of GraphMini}
In this paper, we present \cache{}, a query compiler that generate optimized algorithms based on query schedule. It proactively prunes the input adjacency lists by analyzing the query schedule. We used a set of rules to determine which adjacency lists can be pruned at compile time. 

% The complexity of the algorithm is in order of $O(|V_q|^3)$. Since the pattern graphs are usually small, identifying the pruning opportunities introduce almost no extra cost in practice. 
GraphMini takes two steps to generate an algorithm. In the first step, it greedily searches for opportunities of pruning adjacency lists for the set operations in each loop level. In the second step, it uses the pruned adjacency lists to accelerate set operations when possible. Since the analysis is static and straight forward, using our technique adds very small overhead to the existing systems for code generation.
% Our technique can achieve significant speedup for complex queries running on large graphs. It only requires consume very small extra memory, which is less than 20MB per thread in our experiments. Our experiments also show that with proactive pruning, the algorithm runs at most \speedup{} faster than the current state-of-the-arts.

% In section \ref{section:motivation} we gave an example of using a pruned graph to help humans find all matchings of query $Q_1$ with $b=M(v_1)$. We now discuss how we can use this idea in the context of nested loop algorithm to speed up query execution. 
% The main idea of our technique is we can use a subgraph containing edges and vertices that is relevant to the current partial match for matching the subgraph. We avoid unnecessary data access by pruning the data graph. In the following section, we will discuss:

% \begin{enumerate}
%     \item How we can prune the data while preserving the results.
%     \item In what scenario we can prune the data graph to speed up the query execution.
%     \item Low level tricks to speed up set operations.
% \end{enumerate} 

% \ms{you will argue that most of the time is spent running set intersections in the lowest loop. before you propose your solution, you could present numbers to validate your argument. run regular automine and see how much time it spends there.} 
% One approach to speed up the algorithm is caching. It is based on the observation that the number of vertices explored in the deeper loops grows exponentially, indicating the cached results can be hit for multiple times in the inner loops. In fact, the prefix optimization can be considered as one such example. In stores the partial edge relations between the matched vertex and some to be matched vertices in the prefix set. It is effective because each prefix set is going to be used for multiple times in the next inner loop if the next loop iterates through multiple vertices. 

% Since the main computations in the generated algorithm are set intersections and set subtractions between the adjacency lists, another caching strategy is pre-computing the set operations between the adjacency lists. For example, assume the all the pattern graphs are connected and we have pre-computed the set intersections and set-subtractions between two adjacency lists. We can then use the cached results in the second layer of the nested loop without further computation (ex, algorithm \ref{algorithms:prefix-pattern-2}, line 7-8). We can also use them as partial results to speed up computations in the deeper layers. This pre-computation certainly adds overhead to the algorithm but it can be amortized over many queries.

% The problem of this strategy is two folds. First it wants to build a cache for subgraph matching on any root vertex. Therefore, it needs to store large amount of cached results that is irrelevant to the partial matching it is working on. This significantly increase the memory consumption of the algorithm as a whole. In addition, it is also limited to pre-compute the set operations between two adjacency lists due to the high memory cost. Storing set operations between three or more adjacency lists in memory is impractical as the size of the results grows exponentially. With prefix optimization already cached some of the set operations, it can only marginally speed up the computations in the deeper nested loops.

% We propose a query based caching approach called \newalgo{}. Instead of building the cache before query execution, it builds the cache on the fly and only cache those results that are relevant to the current partial matching. It can cache the set operations between three or more adjacency lists using little memory consumption. By analyzing the query graph, the \newalgo{} focus on caching the set operations of a small range of adjacency lists such that the computation has low overhead and the cached results can be easily stored in memory. These property allows the \newalgo{} to significantly speed up the computation in the inner loops and thus the algorithm as a whole. We now discuss our algorithm and its methodology. 


==> sections/4-methodology.tex <==
\section{GraphMini: A Graph Pattern Matching System} \label{section:methodology}
We now discuss GraphMini, a new graph pattern matching system that uses proactive online graph pruning to obtain minigraphs and speed up query execution.
In Section \ref{section:graphmini}, we discussed the criteria used by GraphMini to prune the adjacency lists and build minigraphs. 
Building minigraphs represents an additional cost that should be minimized.
In this Section, we discuss additional techniques  and optimizations used by GraphMini to build minigraphs efficiently. 
We then show an example of query execution code using minigraphs.

\subsection{Optimizing the Use of Minigraphs}
GraphMini uses several optimizations to avoid computing the same minigraphs repeatedly, reuse the minigraphs whenever possible, and only compute the pruned adjacency lists that might be used multiple times.
To do so, it takes three steps when generating query execution code. 

In the first step, it greedily searches for the opportunities to prune adjacency lists based on the criteria discussed in the previous section.
At each loop in the query execution code, it groups the pruned adjacency lists into minigraphs.
The grouping is based on which set operations the pruned adjacency lists can be used to accelerate. 
It then adds all the possible minigraphs to a list for further analysis. 
In the second step, GraphMini removes the duplicated minigraphs in the list and merges multiple minigraphs when certain conditions are satisfied. 

In the final step, it uses the minigraphs that remained in the list to accelerate set operations and generates code accordingly. 

We will discuss each step and the optimizations we applied in detail in this section.
We will also show that the analysis of minigraphs is static and straightforward. 
Using our technique adds a very small overhead to the existing systems which are discussed in Section \ref{section:evaluation}.

\subsubsection{Materializing Minigraphs}
GraphMini organizes the pruned adjacency lists into multiple minigraphs.
At each loop, it groups the pruned adjacency lists that will be used for the same future set operation into the same minigraph. 

In Section \ref{section:graphmini} we discussed how to find the adjacency lists to prune and how to prune them.
Doing this requires two specific prefix sets:
\begin{itemize}
    \item The \emph{selecting-set} is the prefix set used to select which adjacency lists to prune ($S^h_i$ in Criterion \ref{crit-1}).
    \item The \emph{filtering-set} is the prefix set used to compute the pruned adjacency lists by intersecting it with the adjacency lists of the vertices in the selecting-set ($S^h_k$ in Eqns.~\ref{eq:intersect} and \ref{eq:subtract}).
\end{itemize}

The system \emph{materializes} a minigraph when both the selecting-set and the filtering-set it uses have been materialized.
These prefix sets are materialized when they effectively restrict the scope of candidates for a query vertex, as discussed in Section~\ref{section:prefix-optimization}.
% \ms{define filtering and selecting set beforehand then talk about materialization}
% The system \emph{materializes} a minigraph when two requirements are satisfied: 
% \begin{enumerate}
%     \item Its filtering-set has been materialized in the loop that we build the minigraph. \ms{add references to Eqns or Table II}
%     \item Its selecting-set has been materialized in the loop that we build the minigraph.
% \end{enumerate}
More specifically, to build a minigraph for computing $S_k^i$ at loop depth $h$, $S_k^h$ (the filtering-set) and $S_i^h$ (the selecting-set) need to be both materialized at loop $h$. 
For each vertex in $S_i^h$ we compute the intersection of its adjacency list with $S_k^h$ and the result is $N_{k, i}^h(u_i)$, the pruned adjacency list of $u_i$ at loop $h$ for the set operation to compute $S_k^i$. 

We store these pruned adjacency lists in compressed sparse row format in the same minigraph.
We denote this minigraph as \emph{MiniG}$(S_{k}^h, S_{i}^h)$, where:
$$ N_{k, i}^h(u) = S_k^h \cap N(u) \quad (\forall u \in S_i^h) $$
In it, $N_{k, i}^h(u_i)$ can replace $N(u_i)$ as input for computing $S_k^i$.

\subsubsection{Merging Minigraphs}
It is possible to have minigraphs that are identical because they are computed using the same set operations on the same adjacency lists.
To avoid building such minigraphs repeatedly, we can compare the filtering-set and the selecting-set of different minigraphs in the same loop. 
If both sets are equal then the minigraphs must also be equal. 
In this case, we only need to materialize one instance of the minigraph in that loop.
% Analyzing of the relationship between different minigraphs is straight forward. 
% Two minigraphs can be either inclusive or exclusive. One minigraph can include the other minigraph when its selecting-set and filtering-set are both superset of those of the other minigraph. Two minigraphs are are exclusive otherwise, as they either have mutually exclusive selecting-set or filtering-set. Two minigraphs can also be identical, if they have exactly the same selecting-set and filtering-set, a special case where the two graphs include each other simultaneously.
% If there are multiple minigraphs that can be materialized in the same loop, we only need to materialize the ones that include the others. If they are materialized in different loops, we can use the larger minigraph to build the minigraphs it includes. 

\subsubsection{Reusing the Minigraphs}
In addition to using the pruned adjacency lists to speed up set operations for computing prefix sets and candidate sets, we can also use the minigraph to speed up the construction of another minigraph.

For example, assume we can build two minigraphs at loop level $h$ and $h+1$ respectively, both minigraphs intend to accelerate the computation for $S_k^i$. We can denote them as \emph{MiniG}$(S_k^h, S_i^h)$ and \emph{MiniG}$(S_k^{h+1}, S_i^{h+1})$ respectively. 

% Notice that the larger minigraph must be materialized in previous loops before materializing the smaller one because of the property of prefix sets discussed in section \ref{section:property_of_prefix}. We call the larger minigraph the parent minigraph and its subset the child minigraph. 
Consider the computation for building the minigraph \emph{MiniG}$(S_k^{h+1}, S_i^{h+1})$, for each vertex $u$ in its selecting-set $S_i^{h+1}$ we compute the pruned adjacency lists by intersecting $N(u)$ with $S_k^{h+1}$. 
Assume the minigraph \emph{MiniG}$(S_k^h, S_i^h)$ has been materialized. 
We know its filtering-set $S_k^h$ is a superset of $S_k^{h+1}$ because of Eqn.~\ref{lemma-1}. 
We can therefore use $N_{k, i}^h(u_i)$ to replace $N(u_i)$ in the set intersection. 
This is correct as shown in Lemma~\ref{lemma-3} and~\ref{lemma-4}. 
In addition, the $S_i^{h}$ is superset of $S_i^{h+1}$, which means \emph{MiniG}$(S_k^h, S_i^h)$ contains all the pruned adjacency lists required in the set intersections that build the pruned adjacency lists in \emph{MiniG}$(S_k^{h+1}, S_i^{h+1})$. 

In summary, if both the selecting-set and the filtering-set of a minigraph are supersets of those of another minigraph, we can use the former to build the latter. 

\subsubsection{Amortizing the Overhead of Pruning Adjacency Lists}
%It is essential that each pruned adjacency list can be used for multiple times such that the overhead of computing it can be amortized. 
At loop level $h$, GraphMini prunes only the adjacency lists of the vertices that will be matched at least two loop levels deeper than $h$.
That is because the cost of pruning adjacency lists $N(u_i)$ with $i=h+1$ is unlikely to be amortized later.
We now argue why.

In Section \ref{section:graphmini}, we have argued that building the minigraph at loop $h \geq i$ cannot accelerate the set operation for computing $S_k^i$. 
Here we show that building minigraph at loop $h = i - 1$ does not help to speed up the computation for $S_k^i$ either. 
At loop level $i-1$, we have matched $u_{i-1}$ and we can compute $S_i$ in the same loop. 
This allows us to know exactly which vertices $u_i$ will be visited by the next loop. Then we simply need to iterate through $S_i$ to compute $S_k^i$ in the next loop.
Therefore, the computation required to compute $S_k^i$ is going to be less expensive than building a minigraph at loop $h=i-1$.
In fact, building the minigraph entails pruning the adjacency lists of each vertex in $S^h_i = S_i$, and each pruned adjacency list is used exactly once in the next loop.

% The same logic applies to the case where $h < i - 2$. 
% The higher the loop we build the pruned adjacency lists, the more likely it will be reused multiple times in the deeper loops. 

We choose $h = i - 2$ so the cost can be amortized to some extent. This strategy still does not guarantee that the pruned adjacency lists will be used multiple times, especially in small graphs. However, it can effectively reduce the size of large adjacency lists which are often accessed many times in the future set operations, which are slow to compute. Reducing the size of these adjacency lists can significantly speed up the query. 

%We leave more sophisticated strategies to the future work.
% The set of vertices in the child pruned graph ($S_j^{k-1}$) is a subset of the set of vertices in the parent pruned graph ($S_j^{k}$). This is because the parent pruned graph contains all the vertices and edges in the child pruned graph so it can be used to build the child pruned graph.

% Consider the computation for building the child pruned graph, for each vertex in $S_j^k$, we need to compute the set intersection between its adjacency list $N(u_j)$ in the original graph with an the prefix set $S_i^k$. Now, if its parent pruned graph $G_{p}(S_i^{k-1}, S_j^{k-1})$ has been built, we can instead use the adjacency list of $u_j$ in the parent pruned graph instead of its adjacency list in the original graph to compute the set intersection. The results will be the same due to the set property discussed in section \ref{section:set-property}. 

% \subsection{ Algorithm Complexity }
% To identify the opportunities for adjacency lists pruning, we can analysis the computation for each prefix set $S_i^j$ and check if any pairs of $S_i^k \text{ and } S_j^k $ have been materialized and $k \leq j - 2$. 

% The entire algorithm is in $O(|V_p|^3)$, because checking if a prefix set can be materialized is constant time operation, the total number of prefix set to be checked is bounded by $O(|V_p|^2)$, and for each prefix set we need to check $O(|V_p|)$ different values of $k$. Multiplying them together gives $O(|V_p|^3)$.

% In reality, the size of the pattern graph $|V_p|$ tends to be small and this marking process can be done in almost no time.

% We greedily mark the opportunities of materializing its pruned graphs for all valid values of $k$. If there are multiple valid $k$, we materialize all of them and use the parent pruned graph to build the child pruned graph as described above.

\subsubsection{Pruning Automorphisms}
To prune the automorphisms, the previous systems enforce a set of canonicality checks at run time as discussed in Section \ref{section:background}. 

GraphZero and GraphPi apply these canonicality checks by performing bounded set operations. 
Assuming the inputs are sorted, the bounded set operations use a given vertex id as the upper bound and terminate the operation immediately when the bound is reached. 
The result of the bounded set operation only contains the vertices within the given bound. 
We implement this pruning technique in our experiments to remove automorphisms.

GraphMini also applies this optimization when it builds the minigraphs. 
Given a minigraph, if all the future set operations using the minigraph are bounded operations for the same vertex id, we can apply the bounded set operation in advance when we build the minigraph. 
For example, we can apply canonicality checks for clique patterns when building the minigraphs.

\subsection{Example of Generated Code Using Minigraphs}
\input{algorithms/Q1-GraphMini}
Algorithm \ref{algorithms:Q1-GraphMini} gives an example of applying proactive adjacency lists pruning to generate algorithms for the pattern $P0$. In this query, we can accelerate the computation for $S_4$ by pruning the adjacency lists $N(u_3)$. We materialize the pruned adjacency lists inside the second loop from lines~\ref{ln:mini-start}-\ref{ln:mini-end} and store them in a minigraph.

Notice that instead of computing $S_3$ and $S_4^2$ at line~\ref{ln:mini-compute}, we can simply read from the minigraph because it contains results. This is because $S_4^1$, the filtering-set of the minigraph is $N(u_1)$. The pruned adjacency lists in the \emph{MiniG}$(S_4^1, S_3^1)$ are the set intersection between $N(u_1)$ and $N(w)$. When we retrieve the pruned adjacency list at line~\ref{ln:mini-retrieve}, we set $w = u_2$. Since the selecting-set $S_3^1$ is equal to $S_2$, which includes all possible $u_2$ that will be used in the intersection. Thus, we can simply query for the minigraph for the result of the set intersection.

Finally, we use the pruned adjacency lists to speed up the computation for the candidate set $S_4$ at line~\ref{ln:mini-s4}. 
Notice that we only need to read from the minigraph to match the vertices other than $v_1$. This property can be helpful for out-of-core systems which store the data graph on disks.
% In fact, we can use the minigraph in figure \ref{figure:MiniGraph-P0} to match the remaining vertices is not a coincidence. The solid part of the graph is equivalent to the minigraph we would get with b matched to $v_1$. This is why it contains all the information required to match the remaining subgraphs. 

% \section{Old Methodology} \label{section:old-methodology}
% Previous work \cite{AutoMine, GraphZero, GraphPi} use the prefix optimization to speed up the nested loop, which prunes the candidate set as more new vertex is added to the partial match. \cache{} utilizes the prefix sets to proactively prune the input adjacency lists. We now discuss how we prune the adjacency lists using the prefix sets. 

% \subsection{Properties of The Prefix Sets }\label{section:property_of_prefix}
% Our approach rely on two properties of the prefix sets to achieve correctness and efficiency.

% We say that $S_i^{j-1}$ is the parent prefix set of $S_i^j$ and $S_i^j$ is the child prefix set of $S_i^{j-1}$. The first property we use is that if we derive a child prefix set from a parent prefix set, then the child prefix set is a subset of the parent prefix set.

% By definition, $S_i^{j-1}$ denotes the prefix set for $S_i$ after handling the edge and non-edge relations between $u_i$ and all the vertex in $I_j = [u_1, \ldots, u_{j-1}]$. The difference between $S_i^{j-1}$ and $S_i^{j}$ is the later also take into account the connection between $u_i$ and $u_j$.

% If $S_i^{j-1}$ has been materialized by the time materializing $S_i^j$, we can simplify the computation for $S_i^j$ as:
% \begin{equation}
%     S_i^{j} = \begin{cases}
%          S_i^{j-1} \cap N(u_j) \:if \: (v_i, v_j) \in E_q \\ 
%          S_i^{j-1} - N(u_j) \:if \: (v_i, v_j) \notin E_q 
%     \end{cases}
% \end{equation}
% % Note that a parent prefix set is always a superset of its child prefix sets. We will use this property to decide what vertices and edges shall be contained in a minigraph. We greedily materialize the prefix set and use the parent prefix set to accelerate the computation when possible. 
% % In the nested loop based implementation, each loop only matches one vertex. 
% The second property we use is the materialized prefix sets in each loop are the most selective sets of vertices for the corresponding candidate sets in that loop. They are most selective because any additional pruning on them does not guarantee the correctness of the final results. To further remove any vertex in the prefix set $S_i^{j}$, we need to know if the removed vertex exists in any of $N(u_{j+1}), N(u_{j+2}), \ldots, N(u_{i-1})$. However, $[u_{j+1}, \ldots, u_{i-1}]$ are not matched until next loops, so we cannot compute this at the current loop. As a result, the prefix sets are most selective. Here, we assume the canonicality constraints are applied to the prefix sets during materialization, we will discuss how the detail in section \ref{section:automorphisms}.

% \subsection{Adjacency Lists Pruning} \label{section:adj_pruning}
% We now discuss the connection between graph pruning optimization with the prefix sets. For simplicity, we will focus on a hypothetical computation for a prefix set $S_i^j$ and assume the parent prefix set for $S_i^j$ has been materialized, so the computation for $S^i_j$ is the set operation between $S_i^{j-1}$ and the adjacency list $N(u_j)$. In the current state-of-the-art approach, the adjacency list is not filtered regardless how many vertices have been added to the partial match. In our approach, we want to prune the adjacency list to speed up this computation. The challenge we face is twofold: 
% \begin{enumerate}
%     \item How to filter $N(u_j)$ while preserve the correctness of $S_i^j$?
%     \item How to filter $N(u_j)$ efficiently such that doing so can bring a speedup?
% \end{enumerate}
% To solve those challenges:
% \begin{enumerate}
%     \item We use set intersection to filter the adjacency list. 
%     \item We compute the set intersection proactively to amortize the overhead of filtering.
% \end{enumerate}

% \subsubsection{Pruning Adjacency Lists With Set Intersection} \label{section:set-property}
% A special property of set inspired us to use set intersection for filtering the adjacency list. 
% \begin{lemma}
%     If $A \subseteq A^*$ and  $T = A^* \cap B$ then:  
%     \begin{gather}
%         A \cap B = A \cap T  \notag \\
%         A - B = A - T 
%     \end{gather}
% \end{lemma}

% \begin{minipage}{\columnwidth}
%     % \centering
%     \includegraphics[width=0.9\linewidth]{figures/A_intersect_B.png}
%     \captionof{figure}{Set Intersection}
%     \label{figure:A_and_B}
% \end{minipage}

% \begin{minipage}{\columnwidth}
%     % \centering
%     \includegraphics[width=0.9\linewidth]{figures/A_minus_B.png}
%     \captionof{figure}{Set Subtraction}
%     \label{figure:A_and_B}
% \end{minipage}
% % \begin{minipage}{\columnwidth}
% %     \begin{minipage}{0.45 \linewidth}
% %         % \vspace*{-0.5cm}
% %         \centering
% %         \includegraphics[width= \linewidth]{figures/A_intersect_B.png}
% %         % \captionof{figure}{\\data graph}
% %         \label{figure:A_and_B}
% %     \end{minipage}
% %     \hfill
% %     \begin{minipage}{0.45 \linewidth}
% %         % \vspace*{0.5cm}
% %         \centering
% %         \includegraphics[width= \linewidth]{figures/A_minus_B.png}
% %         \label{figure:A_minus_B}
% %     \end{minipage}
% % \end{minipage}
% We first observe that $T$ is a subset of $B$ because any element in $T$ must also in $B$, but the reverse is not true. Since $T$ is a subset of $B$, computing set operations between $A$ with $T$ can be less expensive compared to computing set operation between $A$ and $B$.

% In the context of adjacency lists pruning, $A$ represents the prefix set of $S_i^j$, $A^*$ is any ancestral prefix set of $S_i^j$, $B$ represents the adjacency list $N(u_j)$, and $T$ is the filtered adjacency list. We can filter $N(u_j)$ by intersecting it with any ancestral prefix set of $S_i^j$. For instance, to compute the prefix set $S_i^j$, we can first compute $T = S_i^k \cap N(u_j) (k < j)$, then we can use $T$ instead of $N(u_j)$ as the input in the computation of $S_i^j$. 

% \subsection{Amortize The Overhead}
% It is essential that $T$, the filtered adjacency list, can be used for multiple times such that the overhead of computing it can be amortized. 

% To amortize the cost of pruning, we set $k$ to be at most $j-2$. 

% This constraint is based on the hope that when iterate through the vertices in $S_{j-1}$, there might exist multiple paths that lead to the same $u_j$ when computing $S_i^j$. 

% To explain this constraint from a different perspective, suppose we have matched $u_{j-1}$, we can first compute the candidate set of $S_j$, then we simply need to iterate through $S_j$ to compute $S_i^j$ directly. Pruning the adjacency list of $u_j$ does not speed up the computation because each pruned adjacency list will be used for exact once. 

% \subsubsection{The Challenge of Proactive Pruning}
% The biggest challenge of this approach is we need to prune the adjacency list of $u_j$ before we match $u_j$. We don't know which particular $u_j$ will be matched for computing $S_i^j$ by the time we prune its adjacency list. To guarantee the computation for $S_i^j$ can use the pruned adjacency list for all different $u_j$, we filter all adjacency lists that might be used. We do so by pruning all the adjacency lists of all the vertices in $S_j^k$, the ancestral prefix set of $S_j$. \jl{add visual} 

% \subsubsection{The Trade-Off of Proactive Pruning}
% The proactive pruning approach does not assume the pruned adjacency lists will definitely be used. In fact, there might exist no path that lead to the use of any of the pruned adjacency list. 

% We argue that mistakenly pruning the adjacency lists that won't be used only introduce small overhead because these adjacency lists are likely to be small in size. On the other hand, adjacency lists that are expensive to prune are large in size. They are likely to be used for multiple times and the cost of pruning them can be amortized. 

% We do acknowledge that on small graphs where adjacency lists are short, this approach can introduce an overhead, we will discuss this in \ref{section:evaluation}.

% \subsection{Minigraph}
% In each loop, we group the pruned adjacency lists used for the same set operation into a minigraph and materialize a pruned graph when two require are satisfied: 
% \begin{enumerate}
%     \item The ancestral prefix set used to filter the pruned adjacency lists has been materialized. We call it the filtering-set. 
%     \item The ancestral prefix set used to select the adjacency lists to be pruned have been materialized. We call it the selecting-set. 
% \end{enumerate}

% To build a pruned graph for computing $S_i$ at the $k^{th}$ loop, $S_i^k$ (the filtering-set) and $S_j^k$ (the selecting-set) need to be both materialized. For each vertex in $S_j^k$ we compute the intersection of its adjacency list with $S_i^k$ and the result is $N_p(u_j)$, the pruned adjacency list of $u_j$. It can be used to replace $N(u_j)$, the original adjacency list of $u_j$, when computing $S_i^j$. We group the pruned adjacency lists together and analysis and them as a graph. We denote the pruned graph we just described as $G_{p}(S_i^k, S_j^k)$. 

% In it, $V_{p} = S_j^k$ and $N_{p}(u_j) = N(u_j) \cap S_i^k$. 

% \subsection{Analyzing Pruned Graph}
% Analyzing of the relationship between different pruned graphs is straight forward. 

% Two pruned graphs can be either inclusive or exclusive. One pruned graph can include the other pruned graph when its selecting-set and filtering-set are both superset of those of the other pruned graph. Two pruned graphs are are exclusive otherwise, as they either have mutually exclusive selecting-set or filtering-set. Two pruned graphs can also be identical, if they have exactly the same selecting-set and filtering-set, a special case where the two graphs include each other simultaneously.

% If there are multiple pruned graphs that can be materialized in the same loop, we only need to materialize the ones that include the others. If they are materialized in different loops, we can use the larger pruned graph to build the pruned graphs it includes. 

% Notice that the larger pruned graph must be materialized in previous loops before materializing the smaller one because of the property of prefix sets discussed in section \ref{section:property_of_prefix}. We call the larger pruned graph the parent pruned graph and its subset the child pruned graph. 

% Consider the computation for building the child pruned graph, for each vertex $u_j$ in its selecting-set, we need to compute the set intersection between its adjacency list $N(u_j)$ with the filtering-set of the child pruned graph. 

% Now, the parent pruned graph has been materialized and its filtering-set is a superset of that of the child pruned graph. As a result, the pruned adjacency lists in the parent pruned graph are superset of the corresponding pruned adjacency lists in the child pruned graph. We can therefore use the $N_p(u_j)$ from the parent pruned graph to compute the set intersection instead of using $N(u_j$ from the original data graph. The results will be the same because of the set property discussed in section \ref{section:set-property}. 

% In addition, the selecting-set of the child pruned graph is subset of the selecting-set of the parent pruned graph. It means the parent pruned graph contains all the pruned adjacency lists needed to build the child pruned graph. So we don't need to read from the original data graph when build the child pruned graph, as long as the parent pruned graph is a superset of the child pruned graph.

% % The set of vertices in the child pruned graph ($S_j^{k-1}$) is a subset of the set of vertices in the parent pruned graph ($S_j^{k}$). This is because the parent pruned graph contains all the vertices and edges in the child pruned graph so it can be used to build the child pruned graph.

% % Consider the computation for building the child pruned graph, for each vertex in $S_j^k$, we need to compute the set intersection between its adjacency list $N(u_j)$ in the original graph with an the prefix set $S_i^k$. Now, if its parent pruned graph $G_{p}(S_i^{k-1}, S_j^{k-1})$ has been built, we can instead use the adjacency list of $u_j$ in the parent pruned graph instead of its adjacency list in the original graph to compute the set intersection. The results will be the same due to the set property discussed in section \ref{section:set-property}. 

% \subsection{ Algorithm Complexity }
% To identify the opportunities for adjacency lists pruning, we can analysis the computation for each prefix set $S_i^j$ and check if any pairs of $S_i^k \text{ and } S_j^k $ have been materialized and $k \leq j - 2$. 

% The entire algorithm is in $O(|V_p|^3)$, because checking if a prefix set can be materialized is constant time operation, the total number of prefix set to be checked is bounded by $O(|V_p|^2)$, and for each prefix set we need to check $O(|V_p|)$ different values of $k$. Multiplying them together gives $O(|V_p|^3)$.

% In reality, the size of the pattern graph $|V_p|$ tends to be small and this marking process can be done in almost no time.

% We greedily mark the opportunities of materializing its pruned graphs for all valid values of $k$. If there are multiple valid $k$, we materialize all of them and use the parent pruned graph to build the child pruned graph as described above.

% \subsection{Example}
% \input{algorithms/Q1-GraphMini}
% Algorithm \ref{algorithms:Q1-GraphMini} gives an example of applying proactive adjacency lists pruning to generate algorithms for the pattern $P_0$. In this query, we can accelerate the computation for $S_4$ by pruning the adjacency lists $N(u_3)$. We materialize the pruned adjacency lists inside the second loop from line 6-9 and store them in a pruned graph.

% Notice that instead of computing $S_3^2$ and $S_4^2$ at line 12, we can simply read from the pruned graph because it already contained results. This is because $S_4^1$, the filtering-set of the pruned graph, is just $N(u_1)$. The pruned adjacency lists in the \emph{MiniG}$(S_4^1, S_3^1)$ are the set intersection between $N(u_1)$ and $N(w)$. When we retrieve the pruned adjacency list at line 11, we set $w = u_2$. Since the selecting-set $S_3^1$ is equivalent to $S_2$, all possible $u_2$ is included.

% Finally, we use the pruned adjacency lists to speed up the computation for the candidate set $S_4$ at line 15. 


% Notice that we only need to read from the pruned graph to match the vertices other than $v_1$. 

% In fact, we can use the pruned graph in figure \ref{figure:MiniGraph-P0} to match the remaining vertices is not a coincidence. The solid part of the graph is equivalent to the pruned graph we would get with b matched to $v_1$. This is why it contains all the information required to match the remaining subgraphs. 

==> sections/5-engineering.tex <==
% % Two subgraphs are automorphic if they have the same vertices and edges. Automorphic matches to the same query graph are typically considered redundant and are filtered out. Figure \ref{figure:Automorphism-P0} gives an example of automorphic matchings for query pattern $P_0$. All the 4 matchings have the same vertices and edges.



% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[width=0.9\linewidth]{figures/automorphism-P0.png}
% %     \captionof{figure}{Automorphic Matchings For $P_0$}
% %     \label{figure:Automorphism-P0}
% % \end{figure}

% GraphPi \cite{GraphPi} and GraphZero \cite{GraphZero} identify all the pairs of vertices that are symmetrical. We can switch the matched vertices for the two vertices in a symmetrical pair and still get a valid matching. As in figure \ref{figure:Automorphism-P0}, the blue node and the red node are symmetrical as well as the yellow node and the green node are symmetrical as well. If we switch two vertex matched to the blue and the red node in the matched subgraph, the resulting match is still valid. The same is true if we switch the two vertices matched to the green and the yellow node respectively. Without any restrictions, the nested loop algorithm will identify the same subgraph for multiple times.

% This method can prune all the automorphisms, but it makes the set operation more complex as it needs to constantly check if the bound has been reached. 

% To avoid this additional complexity, we pre-compute the bounded length of each vertex's adjacency list with respect to the vertex id. This additional information allow us to perform normal set intersection on the bounded adjacency lists instead of bounded set intersection. Since the vertices in the bounded adjacency lists are all in within the bound (smaller than the vertex's id), the result of set intersection must also be within the bound. 

% For set subtraction, we first perform a normal set subtraction on the bounded adjacency list. However, the result might still contain some vertices outside the bound. We need to perform an additional linear scan to completely remove the vertices outside the bound. We compare the performance of the two approaches in section \ref{section:evaluation}. \jl{add example / visual here}
\section{GraphMini Implementation} \label{section:automorphisms}
We implemented the GraphMini code generator in C++ in about 1000 lines of code. It can produce efficient C++ code for graph queries based on the input schedules (see Figure~\ref{figure:workflow}).
The code generator implements all the optimizations discussed in Section~\ref{section:prefix-optimization} as well as the techniques related to minigraphs discussed in Section~\ref{section:methodology}.
We implement the set operations as linear scans of two sorted sets. 

The generated code stores both the original graph and the pruned graphs in memory. 
The original graph is loaded and its adjacency lists are sorted before query execution. 
The code stores the data graph in compressed sparse row format. 
Each minigraph includes a managed buffer space to store the pruned adjacency lists. 
The code initializes the buffer with a small memory size and it dynamically expands it at run time if necessary. 

The GraphMini code generator is designed to take an arbitrary schedule as an input. 
In our implementation, we integrate the state-of-the-art scheduler from GraphPi \cite{GraphPi} to generate a schedule and the canonicality checks given a graph query.
The schedule and the checks are enforced by the query execution code generated by GraphMini.
We directly run the scheduling code of GraphPi, which is publicly available.
%Since we use an empty \emph{emit} function, the innermost loop which calls \emph{emit} is skipped.

We use OpenMP (v4.5) to automatically parallelize the generated algorithms.
Our parallelization strategy is aimed at avoiding the overheads associated with inter-thread synchronization.
In GraphMini's generated algorithms, a minigraph built at one loop is used only in the lower-level nested loops.
Having threads share minigraphs would require inter-thread synchronization.
To avoid these synchronization overheads, we choose to parallelize only the top-level loop, using multiple threads and OpenMP's dynamic scheduler with chunk size of 1. 
We use a similar criterion on a distributed setup. 
In our generated algorithms, each iteration at the top-level loop starts the matching process from a different vertex in the data graph.
We statically partition the starting vertices among servers, assuming that the cost of each vertex is proportional to its degree, and assign the corresponding top-level loop iterations to servers accordingly.
Each server then uses OpenMP to further parallelize its assigned top-level loop iterations across cores as described previously.

%We remove vertices that have been matched during the set operations \ms{What does this mean?}. 

==> sections/6-evaluation.tex <==
\section{Experimental Evaluation} \label{section:evaluation}

\subsection{Evaluation Setup}
\subsubsection{Data and query graphs}
We use 8 real-world graphs from SNAP \cite{SNAP_datasets} in our evaluation and they are shown in Table \ref{graph_info}. The Twitter graph is only used for memory test.
% \add{We further use graph500 to generate a large graph with billions edges. We use scale 28 and edge factor 16, which generate a graph with $2^{28}$ vertices and $2^{32}$ edges. This graph is only used for scalability test.}
All the graphs are stored in memory during query execution. We consider all the graphs as undirected graphs. That is, if there is an edge $(v_i, v_j)$ in the data set, we assume $v_j \in N(v_i) \text{ and } v_i \in N(v_j)$. 
Figure \ref{figure:patterns} shows the pattern graphs we use in the evaluation. 

These are the same standard benchmarks used in the evaluation of previous work~\cite{GraphZero,GraphPi}. 
These complex patterns are meant to stress test the pattern matching algorithms.

\input{tables/graph_info}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/queries.pdf}
    \captionof{figure}{Query Graph Patterns}
    \label{figure:patterns}
\end{figure}

\subsubsection{Hardware and Software Setup}
We run all \add{single-server} experiments on a server-class machine running Ubuntu 18 with 32 cores (64 threads) and 128 GB of RAM. The machine has two Intel(R) Xeon(R) Silver 4216 CPUs (with Intel Turbo Boosting disabled). 
All tests use one CPU thread unless otherwise stated. 
\add{For distributed experiments, we use a cluster of 15 servers.
Each server has two Intel(R) Xeon(R) CPU X5650 CPUs, each with 6 cores (12 threads) and 64 GB RAM.}
All programs are written in C++ and compiled with gcc 7.5 with -O3 optimization. 
In all cases, the input graph is loaded entirely in memory.

\subsubsection{Baseline}
The current state-of-the-art graph pattern mining system is GraphPi.
GraphPi considers a different variant of the graph pattern mining problem compared Automine, GraphZero, and GraphMini.
In that variant, the ``if and only if" logical operator of Eqn.~\ref{eqn:vertex-centric} is replaced with an ``if".
This makes it impossible to conduct a meaningful general comparison between the performance of GraphPi and GraphMini: GraphMini is much faster but this is also because it returns a smaller result set for most patterns.
% For example, on the LiveJournal (Lj) graph, GraphMini can run query P2 in about $10^4$ seconds using $1$ thread, whereas the GraphPi paper reports a running time close to $10^5$ seconds with $24$ threads.
% This, however, is just an artifact of incompatible problem definitions.

\input{tables/experiments-graphpi.tex}

To have a homogeneous and fair ground for comparison, we use the same codebase for all experiments.
We integrate all graph pattern matching optimizations of GraphPi, including its state-of-the-art scheduler and canonicality checks, into both GraphMini and the baseline.
We also used GraphZero's scheduler open sourced by GraphPi, but our evaluation confirmed the published results showing that GraphPi produces much better schedules~\cite{GraphPi}.
Both GraphMini and the baseline also include the state-of-the-art code generation optimizations introduced by Automine and GraphZero and discussed in Section~\ref{section:prefix-optimization}.
We reimplemented those optimizations since neither the code nor the executable of Automine and GraphZero are publicly available.
The only difference between the baseline and GraphMini is that GraphMini uses minigraphs.

\add{
To validate the quality of our baseline implementation in absolute terms, we compared it with the original GraphPi implementation, which is the current state of the art, in the special case of clique query patterns, for which both systems return the same results.
We considered cliques of size 3 to 5 and the wiki, patents, lj, and orkut graphs.
Our baseline implementation outperforms GraphPi by a factor of at least 2.1$\times$ and at most 5.2$\times$, depending on the graph and the query.

In this evaluation section, all query execution times exclude the time required to load the input graph in memory. 
For GraphMini, the query execution times always include the construction time of minigraphs, which takes place online during query execution.}

\subsection{Query Execution Time}
% \input{sections/experiments/exp_run_time}
% \input{tables/experiments-graphzero.tex}
We now compare the performance of \cache{} and the baseline method using GraphPi's schedules. 
We focus on the performance comparison with a single thread since the optimizations enabled by minigraphs are not specifically related to parallelism.
The performance comparison between GraphMini and the baseline is shown in Table \ref{table:graphpi}. \add{The `Base` column shows the running time of the baseline and the `Gm` column shows the results from GraphMini.}
We denote with `OT' experiments that took more than \add{24} hours to complete.

Using minigraphs results in significant speedups in almost all cases, reaching one order of magnitude for query $P3$ running on YouTube.
As expected, with a given graph, the speedups tend to grow with \add{query graphs that are larger and take longer to process.}
Executing a query with many vertices requires many nested loops.
The cost of executing minigraphs is paid at top-level loops and amortized when executing deeper loops.
Executing a large number of loops, as expected, offers more opportunities to leverage existing minigraphs and amortize the minigraph construction cost.

For example, query $P0$ only has four vertices, which correspond to four loops in the query execution code.
In this case, GraphMini only builds minigraphs in the first loop, and these minigraphs are only used in the last loop where set operations occur.
For these reasons, the cost of building minigraphs cannot be amortized on all graphs.
However, we obtain speedups on all graphs for all other queries, with the only exception of Youtube and $P1$ where the running time slightly decreases.
Overall, we observe that GraphMini always offers relative speedups for the slowest queries which are the most critical to optimize in terms of absolute running time.
\add{For P6, we use the best schedule we found for both the baseline and GraphMini.}
% In the second experiment, we use the GraphZero's model to generate the schedules and restrictions for each pattern query. We observe that both GraphPi and GraphZero generate the same schedules and restrictions for $P0$ and $P1$ for all the tested graphs. We omit these results in the table \ref{table:graphzero}, which contains the running time for $P2$, $P3$, $P4$, and $P5$ only. 
% Here, we observe that both the Baseline and GraphMini take longer to run given the same query and graph. GraphMini still outperforms the baseline method in $P4$. It has a relatively worse performance in $P2, P3$. For query $P5$ running on the graph YouTube, GraphMini is significantly slower than the baseline due to the schedule it uses. This is because GraphMini amplifies the influence of the schedule. The schedule impact the size of the prefix sets used to build the pruned graphs. As discussed in GraphPi \cite{GraphPi}, a fast schedule usually has small candidate sets (and prefix sets) in the upper loops, which reduce the number of vertices traversed in the future loops and hence reduce the number of set operations. GraphMini use the prefix sets in upper loops to build the pruned graph, so their sizes have a significant influence on GraphMini's the performance.

\subsection{Code Generation Time}
The results of Table~\ref{table:graphpi} only report the running time of the query execution code, which takes a data graph as input and enumerates the matches.
This is the last step of the workflow of a graph pattern matching system (see  Figure~\ref{figure:workflow}).

% To obtain the query execution code it is necessary to run a scheduling algorithm to find a query schedule and then generate the code.
% These are one-time costs that can often be amortized, since the generated code can be rerun multiple times, but it still needs to be reasonably low.

% To evaluate the running time of the preliminary steps to query execution, we measured the code generation and scheduling time for different queries.
% Table \ref{table:code_generation_time} shows the results.
% Both the baseline and GraphMini use GraphPi's query scheduler, so the scheduling time is the same in both cases and is reported only once.
% The results show that scheduling takes much longer than code generation, both for the baseline and for GraphMini.

GraphMini does introduce extra overhead for code generation compared to the baseline.
This extra time is necessary to establish when introducing minigraphs in the generated code.
However, code generation takes less than 1 ms even in the case of GraphMini.
This overhead can be ignored when considering the entire workflow of the subgraph matching system. 
% or even just the time required to compute a schedule. 
% \input{tables/experiments-code-generation}

\subsection{Multithreaded Scalability}

To evaluate the performance of GraphMini on multiple threads and its scalability, we consider the largest graph and the most complex query GraphMini can run within 48 hours using a single thread, which is graph Lj and query $P2$ respectively. 
We scale the number of threads up to 64, which is the maximum number of hyperthreading supported by our server.
\add{We use OpenMP to determine the maximum number of allowed threads and CPU cores.
In configurations with up to 16 threads, OpenMP schedules all threads on the first CPU.
With more than 16 but less than 32 threads, OpenMP uses all cores of the first CPU and a subset of the cores of the second CPU.
With 32 threads or more, all cores are used.
}

Both GraphMini and the baseline achieve significant speedup when using multiple threads, showing similar performance trends.

The relative speedup of GraphMini is slightly lower than the baseline with 64 threads, but its absolute running time is still significantly better: GraphMini takes 266 seconds to complete, a 5$\times$ speedup compared to the 1375 seconds required by the baseline. 

\add{The reason for the lower speedups compared to the baseline is the additional data accesses required to proactively build the minigraph  (see for example Algorithm~\ref{algorithms:Q1-GraphMini}, ln~\ref{ln:mini-start}-\ref{ln:mini-end}).
Both the baseline and GraphMini scale similarly when using one CPU, that is, from 1 to 16 threads.
When switching to using the second CPU, i.e., with more than 16 threads, GraphMini does not scale well initially, but then scales linearly again, for example from 24 to 48 threads or from 32 to 64.

We observed that GraphMini has a higher last-level cache miss rates than the baseline and it takes less advantage from the additional cache space  available when moving to the second CPU.
When running query P2 on the Lj graph, for example, the last-level cache miss rates for GraphMini are 11.59\%, 6.45\%, and 7.98\% with 16, 32, and 64 threads respectively, compared to 8.97\%, 3.28\%, and 4.59\% for the baseline.
This is due to the additional proactive data accesses required to build minigraphs.
The additional main-memory accesses due to cache misses are more expensive with two CPUs because they can incur NUMA overheads.
Nonetheless, even if the relative speedups plateau between 16 and 32 threads, building minigraphs allows GraphMini to perform less work, making GraphMini much faster than the baseline in terms of absolute running time. 
}

% Overall, \cache{} is more beneficial for complex queries taking longer time to execute. Here, the size of the graph is not the main factor of the complexity of the query. 
% Take the experiments for $P_3$ as an example, it takes the baseline 1.4 hours to run on the graph YouTube, but less than 0.84h (2995.4s) to run on the graph Pokec. Pokec has ten times the edges and 50 percent more vertices than YouTube, but it still takes longer time to run this query on YouTube. 
% This is true even after we switch to using GraphPi's schedule and restrictions, which speed up the baseline for 2.6x on Pokec and 3x on YouTube respectively. The reason for this discrepancy is the two graphs have different structural properties and distributions of the edges. The query time spend on the dense regions in the graph is significantly larger than the rest. Using \cache{} reduce the querying time spend on the dense regions, where the pruned adjacency lists can be used for multiple times which reduce the computation time significantly. In YouTube, using \cache{} along speedup the baseline for 2x, whereas it using with GraphPi's schedule and restrictions speed up the baseline for 15x. 

\add{
    \subsection{Distributed Scalability}
\add{
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/multithread_scalability.pdf}
    \captionof{figure}{\add{Multithreaded scalability Test}}
    \label{figure:multithread_scalability}
\end{figure}
}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/multinode_scalability.pdf}
    \captionof{figure}{\add{Multinodes scalability Test}}
    \label{figure:multinode_scalability}
\end{figure}

In the distributed scalability test, we statically assign the top level vertex to each node.
We assume that the cost of each vertex is proportional to its
degree. We sort the top-level vertices by degree and and assign to servers accordingly. Each server then uses OpenMP to further parallelize its assigned top-level loop iterations across
cores. This scheduling has a fixed overhead for each node and is included in the figure. This overhead is pattern independent and only related to the data graph. The scheduling overhead is 0.6s for Lj and 12s for Friendster.

We observe that this scheduling strategy provides near linear speed up for P2, P3, and P4 on Friendster, P2 and P3 on Lj. It has a worse scalability for P4 on Lj due to unbalanced workload distribution. We also test the baseline using the same strategy on P2 for Lj, it has a less speedup when increasing the nodes from 8 to 15. We plan to solve this problem by implementing dynamic scheduling strategy. }

\input{tables/experiments-memory}

\subsection{Memory Consumption}
We now measure the memory overhead of materializing minigraphs in GraphMini.
Table \ref{table:memory} shows the memory requirement for storing each data graph and the peak memory requirement used by each thread for storing all its minigraphs.
We measure peak memory requirement because GraphMini dynamically scales the memory usage based on the size and number of the minigraphs, starting from a small memory footprint.

Table \ref{table:memory} shows that the \add{per thread} size of the minigraphs is usually only a small fraction of the data graph. 
The size of minigraphs is not directly related to the size of the data graph itself but rather to the density of connections in the graph or part of the graph with the exception of the graph Twitter.  
Some graphs, like Patents or Pokec, only induce minigraphs that are orders of magnitude smaller than the input graph, independent of the query graph. Other graphs show a larger variance. The memory consumption is per-thread because in the current implementation of our system we have each thread build minigraphs independently. 

\add{It is difficult to predict the size of the minigraphs as it is correlated to many factors, including the connection density of the data graph, the pattern graph and the schedule. We empirically observe that the memory consumption might be correlated to the max degree of the graph for the graph we tested. Figure \ref{figure:memory} shows the peak memory consumption per thread for minigraph on P0 with different data graphs. 

Notably, the peak memory consumption for minigraph is more than 4GB on twitter, which is in the same order of magnitude compared with the original graph. This is because there is a large densely connected region in the data graph. The worst case is when the entire data graph is strongly connected, where the minigraph will cache the entire data graph. However, using a bit matrix to store the minigraph/original graph is preferred in this situation. We plan to investigate the techniques to reduce the memory consumption of minigraphs for dense data graph by using binary or hybrid representation instead of simply integer vertex ids. }

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/memory_p0.pdf}
    \captionof{figure}{\add{Minigraph Memory vs.Max Degree on P0}}
    \label{figure:memory}
\end{figure}

%The highest memory consumption is less than 14 MB and occurs with querying $P0$ on Orkut. 


% This is not a problem in general, given that the size of the minigraphs is so small.
% Even in the worst case in terms of memory, where we run Orkut with $P0$ with all the 64 threads supported by our server, the size of the minigraphs is still smaller than the input graph.

==> sections/7-relwork.tex <==
\section{Related work}

Several frameworks \cite{Pregel, GraphX, Ligra} tackle general graph processing, which may be either vertex-centric or edge-centric. 
These frameworks provide an extensible high-level task API while abstracting several low-level components such as scheduling, graph access, and parallelism. However, they are not well suited for graph mining problems such as motif counting and frequent subgraph mining. 
This has motivated the development of dedicated subgraph-centric graph mining frameworks \cite{Arabesque, RStream, Pangolin, Fractal, Peregrine, AutoMine, GraphZero, GraphPi}. 
Recent graph mining systems work uses subgraph query matching as a subroutine \cite{AutoMine, Peregrine}. 
They select the optimal schedules at query time and generate an optimized algorithm or binary to handle query matching. 
They also introduced a code generation approach to further improve performance~\cite{ AutoMine, GraphZero}. 
GraphMini advances this line of work by proposing a novel direction for performance optimization.
Throughout the paper, we discuss the state of the art extensively to motivate our work and show that using minigraphs can lead to further performance reduction compared to it. 

This work considers unlabeled data graphs and queries, a problem that some work calls \emph{subgraph enumeration}.
Prior work developed a separate family of algorithms to deal with labeled graphs and queries, a problem that some work calls \emph{subgraph matching}.
For a recent survey and experimental evaluatation of these algorithms see~\cite{in-depth}.
RapidMatch is another more recent work in this area~\cite{rapidmatch}.
cuTS optimizes subgraph matching on GPUs~\cite{cuTS}.
A key challenge in subgraph matching is leveraging labels to filter candidate vertices and find a good query schedule, which is not an issue in subgraph enumeration.


This work considers main-memory graph pattern matching (or subgraph enumeration) algorithms.
Other work considered algorithms for out-of-core graphs~\cite{DUALSIM}, exploit symmetry to reuse computation~\cite{ParallelSingleMachine}, or explore output compression~\cite{cbf}. 
None of these algorithms considered proactive online graph pruning, where we prune the adjacency list of vertices that we have not yet matched online, during query execution.

Some work proposes accelerating set intersections by using a binary representation of the graph and using SIMD instructions in the CPUs \cite{EmptyHeaded, SIMD}. 
Our work also aims to speed up set operations, but it does so by reducing the size of the input sets, independent of how the inputs are represented.
These two approaches are complementary and combining them represents an interesting direction to further optimize running time.

Graph databases are increasingly used in many applications \cite{GraphProcess,Demystify,EmptyHeaded}. 
These systems enable users to run graph queries and optimize the order of joins~\cite{JoinProcessing}.
% Much work has focused on algorithms for subgraph isomorphism and subgraph enumeration, as for example \cite{Dualism, SubgraphMapReduce}. 

\section{Conclusion}
Proactive online pruning represents a novel direction to reduce the running time of graph pattern mining algorithms.
It entails building minigraphs, a pruned representation of the data graph that can be used instead of the original graph to speed up query execution.
Minigraphs represent a complementary technique that can be combined with other state-of-the-art algorithms for query scheduling and code generation.
The GraphMini system shows that minigraphs can speed up query execution time by up to $10\times$ with a low memory cost.
Introducing minigraphs in generated query execution code only adds a negligible slowdown to code generation.

Proactive online pruning is a novel approach that opens up several new avenues to optimize graph pattern matching.
One promising direction is to develop scheduling algorithms that can produce schedules and canonicality checks that can better leverage minigraphs. 
Another interesting direction is exploring the binary or compressed representation of the minigraphs.
Since minigraphs are generated online anyway, using a binary representation may be even more advantageous.
Finally, combining minigraphs with parallel query execution is also a promising direction.
When running queries using multiple parallel threads, it could be possible for the threads to share the computational and memory cost of building minigraphs.


==> sections/experiments/exp_run_time.tex <==
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/P0_figure.png}
        \caption{$P_0$}
        \label{table:q2}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/P1_figure.png}
        \caption{$P_1$}
        \label{table:q3}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/P2_figure.png}
        \caption{$P_2$}
        \label{table:q4}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/P3_figure.png}
        \caption{$P_3$}
        \label{table:q5}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/P4_figure.png}
        \caption{$P_4$}
        \label{table:q6}
    \end{subfigure}
    % \begin{subfigure}[b]{0.33\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/P5_figure.png}
    %     \caption{$Q_7$ and $Q_8$}
    %     \label{table:q7q8}
    % \end{subfigure}
    % \begin{subfigure}[b]{0.33\textwidth}
    %     \centering
    %     \includegraphics[width=\textwidth]{figures/q8_std_rtm.png}
    %     \caption{Q8}
    %     \label{table:q8}
    % \end{subfigure}
    % \subfloat[Q2]{\includegraphics[width=0.33\textwidth]{figures/q2_std_rtm_cano.png}\label{table:q2}}
    % \subfloat[Q3]{\includegraphics[width=0.33\textwidth]{figures/q3_std_rtm_cano.png}\label{table:q3}}
    % \subfloat[Q4]{\includegraphics[width=0.33\textwidth]{figures/q4_std_rtm_cano.png}\label{table:q4}}        \hfill
    % \subfloat[Q5]{\includegraphics[width=0.33\textwidth]{figures/q5_std_rtm_cano.png}\label{table:q5}}
    % \subfloat[Q6]{\includegraphics[width=0.33\textwidth]{figures/q6_std_rtm_cano.png}\label{table:q6}}
    % \subfloat[Q7 and Q8]{\includegraphics[width=0.33\textwidth]{figures/q7q8_std_rtm_cano.png}\label{table:q7q8}}
    % \subfloat[q8]{\includegraphics[width=0.33\textwidth]{figures/q8_std_rtm.png}\label{table:q8}}
    \caption{Subgraph Enumeration Performance of \cache{} vs. the Standard Algorithm}
    \label{fig:graphmini_vs_standard_cano}
\end{figure*}

==> sigmod-sections/0-Abstract.tex <==
\begin{abstract}
    Subgraph enumeration is a fundamental problem encountered by many common graph mining tasks. It aims to enumerate all subgraphs that match specific patterns on unlabeled graphs.
    This paper explores for the first time how to proactively prune graphs to speed up subgraph enumeration by leveraging solely the structure of the query pattern and the input graph. 
    We propose MiniGraph, a new subgraph enumeration algorithm that builds pruned auxiliary graphs to replace the original graph during query execution.
    This requires careful balancing between the upfront cost of pruning and the gains of faster set operations.
    Our evaluation shows that using Minigraph can achieve a speed up to one order of magnitude compared to the state-of-the-art subgraph enumeration system on commonly used benchmarks while using only minimal memory.
\end{abstract}

==> sigmod-sections/1-Introduction.tex <==
\section{Introduction} 
\label{section:introduction}
% In the recent years, the emerging large graphs from a wide range areas encouraged the development of efficient systems for solving the NP-hard graph problems \cite{Ubiquity}.

Subgraph enumeration aims to find all subgraphs in an unlabeled data graph that are isomorphic to a query graph. 
It is a fundamental problem encountered by many common graph mining tasks and real-world applications, such as analyzing social \cite{social1, social2} and protein-protein interaction network~\cite{ppt1}. 
It is a basic building block of graph pattern matching systems~\cite{Arabesque, Peregrine, Fractal, RStream, GraphX, GraphProcess}.
The problem is challenging because the search space and the size of intermediate data increase exponentially with the size of the data graph and query graph. 
This has motivated the development of state-of-the-art systems such as AutoMine~\cite{AutoMine}, GraphZero~\cite{GraphZero}, Dryadic~\cite{Dryadic}, and GraphPi~\cite{GraphPi}.

% This is why we have seen a great interest in research on graph mining systems that can support general graph mining applications at high-performance \cite{Arabesque, Fractal, G-miner, ASAP, GraphX, SubgraphMapReduce, RStream, BENU,yang2021huge} in the distributed context. 
% \ms{This could be integrated as the first paragraph.} \jl{done}

% Specialized systems for subgraph enumeration \cite{AutoMine, GraphZero, GraphPi} have been developed to handle large graphs and complex queries. These systems implement the subgraph enumeration algorithm as nested loops and generate a new algorithm for each query pattern instead of using one algorithm to solve all the queries. AutoMine \cite{AutoMine} has shown that a compilation-based system often outperforms a generalized algorithm by several orders of magnitude. It also demonstrates its compiled algorithm can handle data graphs with tens of billions of edges with minimal memory overhead, allowing a single machine to take large data graphs that overwhelm many distributed systems \cite{AutoMine}. GraphZero and GraphPi \cite{GraphPi, GraphZero} reveal that the performance for a compiled algorithm can vary significantly with different matching order and symmetry-breaking paradigms. That is why the state-of-the-art subgraph enumeration systems thoroughly discussed the compilation techniques, matching orders, and symmetry-breaking paradigms \cite{AutoMine, GraphZero, GraphPi, Dryadic}. 

% These systems find more efficient matching orders and symmetry-breaking paradigms to reduce search space and leverage compilation techniques to reduce query execution time. 
% Although they have achieved excellent performance improvements, they did not consider the key strategy of leveraging auxiliary data structures to accelerate query execution. 
% They use the labels and degrees of the query and data vertices to prune the adjacency lists, which reduces the algorithm's search space and leads to significant speed up \cite{in-depth, Versatile}. However, the state-of-the-art subgraph enumeration system like~\cite{AutoMine, GraphZero, GraphPi} overlooked the opportunity of using pruned graphs to accelerate the subgraph enumeration. They only prune adjacency lists for removing \emph{automorphisms}, which require the given query pattern to be symmetrical. 
% AutoMine \cite{AutoMine} has shown that a compilation-based system often outperforms a generalized algorithm by several orders of magnitude. It also demonstrates its compiled algorithm can handle data graphs with tens of billions of edges with minimal memory overhead, allowing a single machine to take large data graphs that overwhelm many distributed systems \cite{AutoMine}. GraphZero and GraphPi \cite{GraphPi, GraphZero} reveal that the performance for a compiled algorithm can vary significantly with different matching order and symmetry-breaking paradigms. That is why the state-of-the-art subgraph enumeration systems thoroughly discussed the compilation techniques, matching orders, and symmetry-breaking paradigms \cite{AutoMine, GraphZero, GraphPi, Dryadic}. 
% Prior work has proposed using auxiliary data structures (\emph{pruned} graphs) to accelerate graph mining in the context of subgraph matching \cite{GraphQL, BI, Han, in-depth, CECI, Turboiso, Versatile}. They use the labels and degrees of the query and data vertices to prune the adjacency lists, which reduces the algorithm's search space and leads to significant speed up \cite{in-depth, Versatile}. However, the state-of-the-art subgraph enumeration system like~\cite{AutoMine, GraphZero, GraphPi} overlooked the opportunity of using pruned graphs to accelerate the subgraph enumeration. They only prune adjacency lists for removing \emph{automorphisms}, which require the given query pattern to be symmetrical. 
This paper improves over this line of work and explores for the first time how to use \emph{proactive graph pruning} to accelerate subgraph enumeration. 
Subgraph enumeration algorithms iteratively generate a set of candidate vertices that can potentially match each target vertex in the query graph~\cite{Ullmann}. 
They are usually implemented as \emph{nested loops}, where each loop tries to match a query vertex with a data vertex and generates a set of candidate vertices from the data graph to match the next query vertex in the deeper loop. 
%A data graph consists of a set of \textit{adjacency lists}; each adjacency list corresponds to a data vertex and records the data vertex's neighbors. 
The computation of the candidate vertices usually involves computation-intensive \textit{set operations} on several adjacency lists.
Our basic idea is to construct \textit{auxiliary graphs} by pruning vertices in these adjacency lists and subsequently use them to accelerate the set operations without changing the graph enumeration results. 
We emphasize that this approach does not remove edges from the original graph, instead it builds mutiple versions of pruned graphs to accelerate the query execution. 
%An auxiliary graph is a collection of pruned adjacency list. 
%Proactively pruning vertices in adjacency lists for subgraph enumeration presents several technical challenges.
% since we can solely use structural information. 
% \hui{need to explicitly explain why ``solely'' is necessary. Why cannot use other information}\ms{clearer now?}

It is not trivial to effectively prune the adjacency lists in unlabeled graphs and several challenges exists.

First, we would like to prune adjacency lists at the upper loop levels and reuse them multiple times in deeper loop levels.
Our insight is that even though at an upper loop level we may not know exactly which vertices match a given query vertex, we can often already identify some vertices that \emph{definitely do not match it}.
We can thus build a separate version of an adjacency list to find matches for that query vertex and proactively prune those vertices.
We then add this pruned adjacency list to the auxiliary graph for that query vertex.
To prune the adjacency list, we propose a novel way to leverage \emph{prefix sets}, an optimization used by state-of-the-art approaches to execute loop-invariant set operations at upper loop levels.
Our work shows that prefix sets can also be useful for a different purpose: proactively pruning the input graph.

Second, determining which adjacency lists to prune can be challenging.
To find matches of a query vertex, we perform set operations using the adjacency lists of vertices in a partial match.
Some of these vertices may not yet be matched at upper loop levels, so we don't know which adjacency lists we should prune.
If we prune too many adjacency lists proactively, we pay an upfront cost at upper loop levels that may not be amortized at deeper loop levels.
However, if we prune too few adjacency lists, we might not gain much.
To solve this problem, we propose a cost model to select which adjacency lists to prune at query execution time.
To evaluate the effectivness of the cost model, we compare it with three variants. 
First, the \emph{eager} variant prunes all adjacency lists that might be used to match the query vertex. 
Second, the \emph{static} variant only prunes adjacency lists using set operations that are executed anyway.
Third, the \emph{static} variant delays the pruning until the adjacency list is used for set operations. 
The evaluation shows that using the cost model out perform the three variants in most cases. \jl{TODO: add some number}

\begin{comment}
First, we introduce a simple \emph{eager} strategy which prunes all adjacency lists that might be used to match the query vertex. This leads to large speedups in some cases, but it is not always beneficial since it may also prune several other adjacency lists that are not used, resulting in wasted work. 
% \hui{Seems that it is not necessary to mention eager strategy here. The best place to mention eager is in the evaluation section baselines for comparison. Instead, should directly mention the cost model and then use the cost model to help decide whether to prune or not}\ms{Edited the previous sentence to say that eager has its benefits. There's no single approach that always dominates.} 
%We then perform a cost-benefit analysis of pruning adjacency lists that shows that the eager strategy cannot always guarantee that proactive pruning is advantageous.
We then perform an analysis of the cost and benefit of proactively pruning adjacency lists.
The analysis shows that proactively pruning using the eager strategy is not always guaranteed to be advantageous.
Furthermore, the analysis shows that deciding at runtime which adjacency lists should be pruned is in itself more expensive than eager pruning.
Therefore, we further propose a \emph{lazy} strategy that only prunes adjacency lists using set operations that are executed anyway.
This lazy strategy guarantees that pruning introduces no extra cost, even though it sometimes achieves less significant gains than the eager strategy.
\end{comment}

\begin{comment}
\spara{Prior text}
Pruning vertices in adjacency lists suffer from several technical challenges.
% 
The first challenge is determining which adjacency lists to prune.
Pruning all adjacency lists once and for all and using them for all kinds of computations is impossible in subgraph enumeration.
We would like to prune adjacency lists at the upper loop levels and reuse them multiple times in deeper loop levels.
However, at the upper loop levels, we don't yet know the specific data vertices that will be matched at deeper levels, so it is challenging to prune the right adjacency lists.

The second challenge is how to prune the adjacency lists. It is unclear how to find the vertices that are irrelevant to the computation. We need to use information obtained at query execution time to prune the adjacency lists. This requires us to perform pruning on the fly, ensuring the correctness of the subgraph enumeration results while minimizing the pruning overhead.

\ms{Mention cost-benefit}

To tackle these challenges, we propose Minigraph, a subgraph enumeration system that leverages a novel auxiliary data structure \textit{auxiliary graphs} to accelerate the computation of candidate vertices and thus query execution. 
Minigraph focuses on accelerating set operations in the query execution and prunes adjacency lists only to be used in those computations.
Minigraph relies on the structural information of the query pattern to determine which adjacency lists to prune. 
It then prunes these adjacency lists at query execution time.  
Besides, Minigraph uses several compile-time optimization techniques to reduce the computation and space overhead of online pruning adjacency lists. 
\end{comment}

Minigraph uses a new code generation approach tailored to minimize the computational cost of building and retrieving auxiliary graphs.
%The system consists of an auxiliary graph-aware code generator that takes as input a query schedule and generates an optimal algorithm that maximizes the benefits of the auxiliary graphs. 
Whenever possible, Minigraph determines at compile time which auxiliary graph should be used when.
This saves the runtime overhead of looking up the right auxiliary graph at query execution time. 
This paper describes several compile-time optimization techniques to reduce the computation and space overhead of pruning adjacency lists. 


Our evaluation shows that using auxiliary graphs can speed up the query execution time by up to an order of magnitude compared to the state-of-the-art while using less than 1GB of additional memory.
In addition, by using only structural information of the input query, the code generation algorithm adds minimal overhead compared to the current approach. 

To summarize, we make the following contributions: 
\begin{itemize}
    \item We propose proactive graph pruning and a new auxiliary data structure called auxiliary graph to substantially speed up subgraph enumeration.
    \item We show that proactive pruning can leverage prefix sets, a complementary optimization originally introduced for a different purpose.
    \item We propose different pruning strategies based on a cost-benefit analysis of proactive pruning.
    \item We implement a novel subgraph enumeration system called Minigraph, which generates query execution code tailored to maximizing the benefit of proactive pruning using several compile-time optimizations.
    \item We experimentally show that Minigraph is substantially faster than state-of-the-art approaches.  
\end{itemize}

% The paper is organized as follows. Section 2 discusses our terminologies, problem statements, and previous techniques we incorporated into our system. Section 3 gives an overview of our online pruning technique. Section 4 introduces how Minigraph uses the pruning technique. Section 5 discusses the engineering details and other optimizations. Section 6 conducts a comprehensive experimental evaluation of our method and the state-of-the-art. Section 7 concludes the paper.
% More specifically, we show how to \emph{prune} the adjacency lists \emph{online} during query execution to build auxiliary graphs and use them to replace the original data graph to speed up the computation. 

% Pruning the data graph \emph{online} requires solving several complex technical challenges to ensure that the new algorithm can amortize the cost of pruning. 
% We need to identify which adjacency lists need to be pruned.
% We must find pruning criteria that guarantee the correctness of the matching process while effectively reducing the size of the adjacency lists.
% We need to manage potentially multiple auxiliary graphs efficiently with limited memory and computation overhead. Meanwhile, we must incorporate the state-of-the-art compilation technique and the symmetry-breaking paradigm to reduce runtime overhead. 

% We implement these techniques in Minigraph, a subgraph enumeration system that uses pruned graphs to speed up query execution. Our online pruning technique complements existing optimizations and leverages current compilation techniques. Our evaluation using standard benchmarks shows that Minigraph can outperform the state-of-the-art graph pattern matching system by up to an order of magnitude. \ms{this statement is a bit confusing since we propose our scheduler} \jl{modified}


==> sigmod-sections/2-Preliminaries.tex <==

\section{Preliminaries} \label{section:background}

{\color{red} This becomes a Background and Motivations section. The formalism of 2.3 and 2.4 and Table 1 are moved to section 3.

Structure of the new section.
\begin{itemize}
    \item Background: related work
    \begin{itemize}
        \item Introduce problem at high level. Consider the example of a 4-clique query. Add a diagram for the query.
        \item State-of-the-art algorithms use nested loops and match one query vertex at each loop, incrementally building a partial match. Use a diagram similar to Figure 2 as a running example so that we can use the same diagram to explain what we do.
        \item Existing work also introduce prefix sets to pull up loop invariant set operations. When we find matches for $v_3$ at loop depth 2, we need to compute $N(u_1) \cap N(u_2)$. Then for $v_4$ we need to compute $N(u_1) \cap N(u_2) \cap N(u_3)$ at loop depth 3. But instead of computing $N(u_1) \cap N(u_2)$ again at loop 3, we do it only once at loop 2 and reuse the results. Let's call the prefix set $C$.
    \end{itemize}
    \item Limitations of existing work
    \begin{itemize}
        \item The prefix set optimization, we still need to run $C \cap N(u_3)$. This is the major bottleneck, see Table 2.
    \end{itemize}
    \item Proposed approach: Minigraph. We describe the high-level idea. Based on the example above.
    \item Why is it hard? Research challenges. Making this idea work in practice is not obvious. Take the points in the intro and make them more concrete using the example.
    \begin{itemize}
        \item we don't know which adjacency lists to prune
        \item we don't know how much we can prune before we actually prune
        \item trade-off between the upfront cost of building the minigraph and the payoff        
        \item We will show that static approaches (eager and lazy) do not always bring speedups.
        \item Motivate the need for a cost model. We need to estimate the potential gain of building a minigraph. We show that we manage to outperform not only the state of the art but also eager and lazy.
    \end{itemize}
\end{itemize}
}

% This section introduces the necessary background on subgraph enumeration.  Subsection~\ref{} defines subgraph enumeration problem and subsection~\ref{} XX. 

% Subgraph enumeration comes in two variants. The non-induced (edge-induced) variant requires a match containing all the edges in the query graph, which might have extra edges. 
% The induced (vertex-induced) variant further requires a match that does not contain extra 
% edges. This work focuses on the induced (vertex-induced) variant. We refer to Table~\ref{notations} for a summary of the notations. \ms{Move the discussion on induced vs. non-induced after the definition because these terms have not been introduced yet. Also, if we say that the technique can be extended, we should at least add a discussion on how to do it.} \jl{addressed}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}


\begin{table}[t]
\centering
\caption{Notations}
\tabcolsep=0.05cm
\label{notations}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|}
\hline
\textbf{Notation}                       & \textbf{Description}                                            \\ \hline
$g(V(g), E(g))$                          & a subgraph, its vertices and its edges                               \\ \hline
$q(V(q), E(q))$                          & a query graph, its vertices and its edges                            \\ \hline
$G(V(G), E(G))$                          & data graph, its vertices and its edges                       \\ \hline
$M(v)$                                   & data vertex matching the query vertex $v$                          \\ \hline
$A_h(v_k, v_i)$                          & auxiliary graph with selecting set $C_h(v_k)$ and filtering set $C_h(v_i)$           \\ \hline
$h, k, i$                                  & three indices such that $h < k < i$                              \\ \hline
$v_i$                                    & $i^{th}$ query vertex to be matched, $v_i \in V(q)$             \\ \hline
$u_i$                                    & a vertex matched to $v_i$ and $u_i \in V(G)$                       \\ \hline
$I_i$                                    & a partial match consists $[u_1, u_2, \ldots, u_i]$               \\ \hline
$C(v_i)$                                 & candidate set of $v_i$                                           \\ \hline
$C_h(v_i)$                               & the $h^{th}$ prefix-candidate-set for $v_i$                      \\ \hline
% $u_{i}^{(h)}$                               & a vertex in $C_h(v_i)$                                           \\ \hline
$N(u_i)$                                 & neighbors of the vertex $u_i$                                    \\ \hline
$P_h(u_k|v_i)$                             & pruned neighbors of $u_k$ at depth h for constructing $C_k(v_i)$ \\ \hline
% $\phi$                                   & matching order                                                   \\ \hline
% $N^{\phi}_{+}(v_i)$, $N^{\phi}_{-}(v_i)$ & forward (backward) neighbors of $v_i$ given $\phi$               \\ \hline
\end{tabular}%
}
\end{table}

% \begin{figure*}[h!]
%     \centering
%     \includegraphics[width= \linewidth]{figures/dfs-tree.png}
%     \captionof{figure}{A running example of subgraph query execution. From left to right: (a) A query schedule with canonicality checks. (b) An unlabeled data graph. (c) A generated algorithm based on the query schedule. (d) Part of the DFS tree of running the generated algorithm on the data graph. The computation for the highlighted sub-tree is further expanded in Figure~\ref{figure:compare}}
%     \label{fig:runningexample}
% \end{figure*}

\subsection{Problem Definition}
\label{sec:problem-def}
We now define the subgraph enumeration problem.
We refer to Table~\ref{notations} for a summary of the notations.
The subgraph enumeration problem takes a data graph $G$ and a query graph $q$ as input and outputs the set of subgraphs $\{g\}$ that are \emph{isomorphic} to $q$. 
In the \emph{edge-induced} variant, a subgraph $ g(V(g), E(g)) $ of $G$ is \emph{isomorphic} to $q$ if there exists a bijection $M$ between the sets $V(q)$ and $V(g)$ such that:
\begin{equation}
    \forall v_i, v_j \in V(q): (v_i, v_j) \in E(q) \iff (u_i, u_j) \in E(g),
\end{equation}
where $u_i = M(v_i)$ and $u_j = M(v_j)$. 

The \emph{vertex-induced} subgraph enumeration problem has the additional requirements that:
\begin{equation}
    \forall u_i, u_j \in V(g): (u_i, u_j) \in E(g) \iff (u_i, u_j) \in E(G).
    \label{eqn:vertex-centric}
\end{equation}
In this case, we say the subgraph $g$ \emph{matches} $q$. 
Minigraph supports both variants, \jl{TODO: add some speedup numbers for either variant}

Typically, we want to output a result set $R$ consisting of \emph{unique} subgraphs -- that is, subgraphs that are not \emph{automorphic} to any other subgraph in $R$. We want to remove automorphic subgraphs because they are essentially the same subgraph obtained by matching the query vertices in different orders.
Two subgraphs $g(V(g),E(g))$ and $g'(V(g'), E(g'))$ of $G$ are automorphic if and only if $V(g) = V(g')$ and $(u_i,u_j) \in E(g) \iff (u_i,u_j) \in E(g')$.


\subsection{Workflow of Subgraph Enumeration} \label{sec:workflow}
State-of-the-art subgraph enumeration systems typically run in two stages, \textit{query scheduling} and \textit{query execution}~\cite{AutoMine, GraphZero, Dryadic, GraphPi}. Minigraph also follows these two stages with the additional step to build and use pruned graphs to accelerate computation.  

\subsubsection{Query scheduling} 
Given an arbitrary query graph $q$ as an input, query scheduling aims to find a \textit{matching order} for the query. 
% The query graph only provides query vertices and the edge relationship between vertices but does not specify how to match the query vertices. 
A matching order specifies which vertex in the query graph should be matched first to a vertex in the data graph.
Given a matching order $\phi$, we use the notation $v_i$ to denote the query vertex in $V(q)$ that has the $i^{th}$ position in the matching order.
If the query graph $q$ is symmetrical, there could be automorphic (i.e., duplicate) matches.
Query scheduling will generate a set of \emph{canonicality checks}, which are rules to prune symmetrical matches.
We call the ordering of query vertices and the canonicality checks a \emph{query schedule}. 
Figure~\ref{figure:workflow}(b) shows an example of a query schedule.

% With a query schedule, it is possible to start executing the query on the data graph.


\subsubsection{Query execution} 

Query execution first generates query execution code specific to a query schedule and then executes the generated code to produce matches. 
The state-of-the-art subgraph enumeration systems \cite{AutoMine, GraphZero, GraphPi} generate query execution code as a sequence of nested loops using Ullmann's backtracking algorithm \cite{Ullmann}. The code materializes a DFS algorithm that traverses vertices in the data graph and tries to identify a match between the vertices in the data graph and those in the query graph. 
Specifically, the body of the nested loop at depth $i$ executes on a \emph{partial match} $I_i=[u_1, \dots, u_i]$, where each $u_i \in V(G)$ and $u_i$ matches a vertex $v_{i} \in V(q)$.
It then computes a \emph{candidate set} $C(v_{i+1})$ so the next loop can iterate over each $u_{i+1} \in C(v_{i+1})$ to extend the partial match to $I_{i+1}=[u_1, \ldots, u_{i+1}]$.

% The search path of the algorithm is a DFS tree where each loop traverses a corresponding layer of the tree.
% We use Figure~\ref{fig:runningexample} to show a fig:runningexample of query execution on the schedule specified in Figure~\ref{figure:workflow}. \ms{right side}


% Rather than running the query plan using a pre-compiled query execution run time, state-of-the-art subgraph enumeration systems \emph{generate query execution code} that is specific to a query, its schedule, and its canonicality checks.
% Then, the query execution code is compiled and executed on the data graph to produce matches.
% Code generation and compilation are very fast, and the speedups of running query-specific code offset the extra overhead. The compiled programs can be reused across different graphs if the query schedule is the same, amortizing the compilation overhead over time.

% The final output of the query executor can be a set of matches or simply the number of matches. In this paper, we consider the problem of finding matches and passing them to an \emph{emit} procedure, which we see as a black box. 
% We implement the subgraph enumeration algorithm as a series of nested loops. 
% Each loop iteratively matches a data vertex to a query vertex and conducts some set operations between adjacency lists. We next describe the two stages in detail. 

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/pipeline.pdf}
%     \captionof{figure}{General Workflow of Subgraph Enumeration Systems}
%     \label{figure:workflow}
% \end{figure}


% \subsubsection{Query scheduling}
% Given an arbitrary query graph $q$ as an input, query scheduling aims to find a matching order for the query. The query graph only provides query vertices and the edge relationship between vertices but does not specify how to match the query vertices. A matching order specifies which depth in the nested loops we should match a query vertices to a data vertex.

% The system runs a scheduling algorithm to find a matching order for the query. 
% % Some algorithms also use statistics collected from the data graph.
% The scheduler is somewhat analogous to a query optimizer in relational databases.

% Given a matching order $\phi$, we use the notation $v_i$ to denote the query vertex in $V(q)$ that has the $i^{th}$ position in the matching order.
% We call the ordering of query vertices the \emph{query schedule}.


% For example, suppose that the query graph of Figure~\ref{figure:workflow} has a match $g$ with vertices $[u_1, u_2, u_3, u_4]$ ordered according to the query vertex they match (i.e., $u_i$ matches $v_i$).
% Because of the symmetry of the graph, the subgraph $[u_1, u_2, u_4, u_3]$ is also a match to $q$, as is $[u_2, u_1, u_4, u_3]$.
% However, we only want to output one canonical match among these automorphic matches.
% One option would be to materialize these matches and then filter them out \cite{AutoMine}.
% Better yet, we could filter \emph{partial} symmetrical matches during the query execution to save the cost of materializing full matches and discard them later \cite{GraphZero, GraphPi}.

% To perform this pruning, the scheduler generates a set of \emph{canonicality checks}, which are rules to prune symmetrical matches.
% In Figure~\ref{figure:workflow}, the scheduler can require the id of a vertex matching $v_1$ to be smaller than that of a vertex matching $v_2$.
% Similarly, it can require that $v_3 < v_4$.
% In the previous example, if the id of $u_1$ is smaller than that of $u_2$ and $u_3$ is smaller than $u_4$, then only the match $[u_1, u_2, u_3, u_4]$ will be canonical among its automorphisms.

% Applying canonicality checks help to reduce the number of set operations. 
% A scheduler needs to determine the optimal combination of the matching order and canonicality checks for a given query graph based on the data graph. 
% The resulting canonicality checks are specific to the order used to match the query vertices.

% \subsubsection{Query Execution}
% With a query schedule, it is possible to start executing the query on the data graph.
% Rather than running the query plan using a pre-compiled query execution run time, state-of-the-art subgraph enumeration systems \emph{generate query execution code} that is specific to a query, its schedule, and its canonicality checks.
% Then the query execution code is compiled and executed on the data graph to produce matches.
% Code generation and compilation are very fast, and the speedups of running query-specific code offset the extra overhead. The compiled programs can be reused across different graphs if the query schedule is the same, amortizing the compilation overhead over time.

% The final output of the query executor can be a set of matches or simply the number of matches. In this paper, we consider the problem of finding matches and passing them to an \emph{emit} procedure, which we see as a black box. 

% General graph mining systems like Arabesque offer programming APIs that enable users to perform arbitrary user-defined functions on the subgraphs of a graph. 
% Arabesque, however, mines subgraphs in a pattern-agnostic manner.
% More recent work, such as AutoMine and Peregrine, has shown that a more efficient approach to support general graph mining applications is first to run graph pattern matching and then execute user-defined functions of the matching subgraphs.

% \textbf{Subgraph Matching.} Subgraph matching is a closely related problem of subgraph enumeration. While subgraph enumeration targets unlabeled graphs, subgraph matching targets labeled graphs. As summarized in \cite{in-depth-2, in-depth}, the common approach for subgraph matching can be described as the following: 
% \begin{enumerate}
%     \item Construct a candidate set for each query vertex, where each candidate set contains all the data vertices that can be matched to a query vertex. (Vertices in a candidate set must have the same label of the query vertex that they match to). 
%     \item Filter the candidate sets to reduce the search space. (Using Label and Degree Filtering (LDF) and other algorithms to prune the candidate sets \cite{GraphQL, BI, Han, in-depth, CECI, Turboiso, Versatile}.)
%     \item Build an auxiliary data structure to maintain the edges between the vertices in different candidate sets. 
%     \item Generate a matching order.
%     \item Use the auxiliary data structure and candidate sets to find all the matches based on the matching order.
% \end{enumerate}

% A key observation is the label information plays an important role in the first two steps of subgraph matching. The pruning on the candidate sets aims to reduce false-positive candidate vertices to be matched, hence improving performance \cite{in-depth-2}. Even though subgraph enumeration and subgraph matching share many similarities, the state-of-the-art subgraph enumeration systems like \cite{AutoMine, GraphZero, GraphPi} do not follow this approach, as constructing and filtering the candidate sets before query execution is much more difficult without the label information. 

% \subsection{Query Execution: Backtracking Algorithm} \label{section:nested-loops}
% We now describe the current approaches to query execution. 

\subsection{Computing Candidate Set}
The performance bottleneck of the DFS algorithm lies in the computation of the candidate set at each loop. 
% Existing algorithms use \textit{set operations} to compute the candidates.  
Consider computing the candidate set $C(v_i)$ at the nested loop at depth $i-1$.
Assume the algorithm has already found a partial match $I_{i-1}= [u_1, \ldots, u_{i-1}]$.
The set $C(v_i)$ 
% must contain the data vertices matching the query vertex $v_i$.
% It 
is computed by performing set operations on the adjacency lists of the vertices in $I_{i-1}$.
The code generator analyzes the edges between $v_i$ and the vertices in the query graph that have already been matched, $[v_1, \ldots v_{i-1}]$.




% The algorithm, which is produced by a code generator in our workflow, must determine which specific set operations are required to compute the candidate set at each loop. 
% Based on the matching order $\phi$, the generator checks the connections between the next query vertex to be matched and all the previously matched vertices to generate the corresponding set operations.

% More precisely, consider computing the candidate set $C(v_i)$ at the nested loop at depth $i-1$.
% The algorithm has already found a partial match $I_{i-1}= [u_1, \ldots, u_{i-1}]$. 
% To into set intersections and set subtractions among adjacency lists. 
% The set $C(v_i)$ must contain the data vertices matching the query vertex $v_i$.
% It is computed by performing set operations on the adjacency lists of the vertices in $I_{i-1}$.
% To determine these set operations, the code generator analyzes the connections between $v_i$ and the vertices in the query graph that have already been matched, $[v_1, \ldots v_{i-1}]$.
% The algorithm partitions the vertices of $I_{i-1}$ into two sets $I_T$ and $I_F$ such that:
% \begin{gather}
%     \forall u \in I_T: u = M(v_h) \text{ and } (v_h, v_i) \in E(q) \notag\\
%     \forall u \in I_F: u = M(v_h) \text{ and } (v_h, v_i) \notin E(q)  \label{equation:partition-partial-matching-candidate}
% \end{gather}

Specifically, the algorithm partitions the vertices of $I_{i-1}$ into two sets $I_T$ and $I_F$ such that:
\begin{gather}
    \forall u \in I_T: u = M(v_h) \text{ and } (v_h, v_i) \in E(q) \notag\\
    \forall u \in I_F: u = M(v_h) \text{ and } (v_h, v_i) \notin E(q)  \label{equation:partition-partial-matching-candidate}
\end{gather}
A candidate set is defined as:
\begin{definition}[Candidate set]
In the \emph{vertex-induced} variant, the candidate set $C(v_i)$ contains the data vertices matching the query vertex $v_i$ and is defined as:
\begin{equation}
    \label{equation:func_1}
    C(v_i) = V(G) \cap \big( \bigcap_{u \in I_T} N(u) \big) - \big( \bigcup_{u \in I_F} N(u) \big). 
\end{equation}

In the \emph{edge-induced} variant, the candidate set $C(v_i)$ is defined as:
\begin{equation}
    \label{equation:func_1}
    C(v_i) = V(G) \cap \big( \bigcap_{u \in I_T} N(u) \big) \big). 
\end{equation}
\end{definition}


% Figure~\ref {fig:runningexample}(c) shows an example of generated nested loops.
% In this example, the query graph has four vertices corresponding to four nested loops.
% The first query vertex $v_1$ can be matched to any vertex in $V(G)$. We call it the top vertex.
% Therefore the set of candidates $C(v_1)$ is $V(G)$, and the first loop iterates over all candidates $u_1 \in V(G)$.

Naively calculating candidate sets based on Eqn. \ref{equation:func_1} is very slow. Existing works propose several optimizations to accelerate the calculation of candidate sets. Minigraph builds on these optimizations and further accelerates the candidate set calculation using auxiliary data structures. We next elaborate on the existing optimization techniques. For simplicity, we will focus on the \emph{vertex-induced} variant in the following discussion. Yet, the anaylsis also applies to the \emph{edge-induced} variant.

\subsection{Existing Optimizations on Query Execution}
\subsubsection{Connected Ordering} \label{connected_ordering}
In real graphs, the size of $V(G)$ is usually orders of magnitude larger than the largest adjacency list in the graph. 
To avoid using $V(G)$ as input in the set operation, schedulers put a constraint on the ordering.
Each matched vertex $v_i$ must be a neighbor of some matched $v_h$ where $h<i$ unless it is the top vertex, that is, $i=1$. 
This constraint ensures that $I_T$ contains at least one vertex, so the computation for $C(v_i)$ becomes: 

\begin{equation}
    C(v_i) =  \bigcap_{u \in I_T} N(u) - \bigcup_{u \in I_F} N(u). \label{eqn:naive_candidate_computation}
\end{equation}

 
% Figure~\ref{fig:runningexample}(c) shows an example of using Eqn.~\ref{eqn:naive_candidate_computation} to find candidate sets. Figure~\ref{fig:runningexample}(d) shows part of the resulting DFS tree using this algorithm to traverse the data graph.
\input{algorithms/Q1-Prefix}

\subsubsection{Prefix sets} 
% \label{section:prefix-optimization}
AutoMine~\cite{AutoMine} further introduces prefix sets to avoid the redundant execution of set operations. It pushes the set operations in computing candidate sets to the uppermost loop that the computation is feasible and reuses the intermiediate results in the inner loops.
The key insight is that some set operations executed in a loop are \emph{loop-invariant}, that is, we can bring them outside the loop without changing the semantics of the program. 
When we match a query vertex we immediately perform all the set operations that are associated with its adjacency list and that are needed to find candidate sets later.

% \hg{cut this section to the end of this page} \jl{done}
% \spara{Definition} \hg{the definition doesn't look consistent}
% The prefix sets of the candidate sets can be, in principle, computed at each nested loop.

We use $C_{h}(v_i)$ to denote the prefix set for the candidate set $C(v_i)$ that can be computed at the nested loop with depth $h$, with $h < i$. $C_{h}(v_i)$ is the superset of $C(v_i)$ that can be obtained based on the adjacency lists of the vertices that have been matched at loop depth $h$.  $I_h$ can be partitioned into two sets $I_{h, T}$ and $I_{h, F}$ such that: 
% These vertices constitute the partial match $I_h = [u_1,\ldots,u_h]$.
% We partition the data vertices in $I_h$ into two sets $I_{h,T}$ and $I_{h,F}$ based on the set operation that must be applied to their adjacency lists, which in turns depends on whether they are connected to the query vertex $v_i$.
\begin{gather}
    \forall u \in I_{h, T}: u = M(v_j) \text{ and } (v_i, v_j) \in E(q), \notag\\
    \forall u \in I_{h, F}: u = M(v_j) \text{ and } (v_i, v_j) \notin E(q).  \label{equation:partition-partial-matching-prefix}
\end{gather}

% A prefix set is defined as follows.
\begin{definition}[Prefix set]
\label{def:prefix-set}
The prefix set $C_h(v_i)$ is only materialized when $I_{h,T} \neq \emptyset$. It is defined as:
\begin{equation}\label{eqn:naive_prefix_computation}
    C_h(v_i) = \bigcap_{u \in I_{h,T}} N(u) - \bigcup_{u \in I_{h,F}} N(u). 
\end{equation}
\end{definition}
When $h = i - 1 $, the prefix set $C_h(v_i)$ is the candidate set $C(v_i)$.
The condition for materialization of a prefix set is that $I_{h,T} \neq \emptyset$.
This ensures that the prefix set can be used to actually prune the candidate set.

Instead of computing the prefix set $C_h(v_i)$ from scratch at each depth $h$, we can compute it incrementally based on the prefix set at the depth $h-1$ and the adjacency list of the data vertex $u_h$: 
\begin{equation}
C_h(v_i) = C_{h-1}(v_i) \circ_h N(u_h),
\label{eqn:prefix_prefix_computation}
\end{equation}
where the $\circ_h$ operator is the set intersection operator ($\cap$) if $(v_i, v_h) \in E(q)$ or the set subtraction operator ($\setminus$) otherwise.
Algorithm~\ref{algorithms:Q1-Prefix} shows an example of using prefix sets to optimize the generated algorithm for query schedule shown in Figure~\ref{figure:workflow}(b). 

\subsection{Motivation of Minigraph} 
We using Dryadic to profile the number of vertices scanned in the set operations. The set operations assume the input arrays are sorted and use a linear scan to compute the results. The profiling results~\ref{tab:motivation} show that the total number of vertices scanned in the adjacency lists dominate the total number of vertices scanned in relatively dense graphs like \emph{Wiki and Lj}. (See graph info in table~\ref{graph-info}.) 

\begin{table}[h]
\begin{tabular}{|c|c|c|c|}
\hline
Data Graph & \textit{Total Scanned} & \textit{From Adj List} & \textit{Percentage} \\ \hline
Wiki    & 99,708,781      & 90,958,752      & 91.2\%          \\ \hline
Patents & 214,095,975     & 96,672,500      & 45.1\%          \\ \hline
YouTube & 270,466,408     & 244,481,160     & 90.4\%          \\ \hline
Lj      & 440,972,948,513 & 422,943,654,151 & \textbf{95.9\%} \\ \hline
\end{tabular}
\caption{Number of Vertices Scanned (5-Clique)}
\label{tab:motivation}
\end{table}

% Computing prefix sets using Eqn~\ref{eqn:prefix_prefix_computation} still require $N(u_h)$, the full adjacency list of each candidate data vertex $u_h$. Since a data vertex can have many neighbors, the query execution's prefix set calculation remains the performance bottleneck.
Thus, one can further accelerate the set operations for subgraph matching on dense graphs by shortening the adjacency list of each candidate data vertex. We build Minigraph that captures this opportunity to accelerate set operations and query execution. 
% \jl{TODO: add a diagram showing the computation is dominated by scanning adjacency lists instead of intermediate prefix sets}


==> sigmod-sections/3-Minigraph.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{sigmod-figures/overview.png}
    \captionof{figure}{Workflow of Minigraph}
    \label{figure:workflow}
\end{figure}

\section{Minigraph}
Minigraph is an efficient subgraph enumeration system that leverages auxiliary data structures to accelerate query execution. 
The fundamental idea of Minigraph is to build auxiliary graphs consisting of pruned adjacency lists online and use the auxiliary graph in deeper nested loops to reduce execution time. 
We emphasize that Minigraph does not remove edges from the original data graph. Instead, it builds mutiple versions of pruned graphs to accelerate the computations for different prefix and candidate sets. 
% We emphasize that Minigraph does not change DFS tree of the generated algorithm. Instead, Minigraph accelerates the computation required to generate the DFS tree. 

The overview of Minigraph is shown in Figure~\ref{figure:workflow}. 
It takes as input a query pattern graph and an unlabeled data graph and produces a set of matched subgraphs. 
%Minigraph consists of two main components. 
The \textit{query scheduler} finds a matching order to generate the matching algorithm.
Minigraph allows using any algorithm to generate the schedule.
Our contribution focuses on the second component, the \textit{code generator}, which produces an efficient subgraph enumeration algorithm using auxiliary graphs. 


This section defines auxiliary graphs and discusses an eager approach to building and using them.
The next section will discuss the limitations of this eager approach and propose two other variants of the approach.
%and how we generate code based on auxiliary graphs in Section~\ref{sec:codegeneration}, and how \emph{dual-sort} schedule queries in Section~\ref{sec:dual-sort}.

\subsection{Auxiliary Graphs} 
\label{sec:auxiliarygraph}
The fundamental bottleneck of subgraph enumeration algorithms is executing the set operations to compute prefix sets and candidate sets (see Eqn.~\ref{eqn:prefix_prefix_computation}). 
An \emph{auxiliary graph} is a data structure designed to accelerate these set operations by reducing the size of the adjacency lists they take as input. 
Each auxiliary graph consists of multiple \emph{pruned adjacency lists}, each storing only a subset of the neighbors of a data vertex.
Whenever possible, Minigraph uses auxiliary graphs instead of the original graph to find the adjacency lists for the set operations.
Pruned adjacency lists are smaller than the original lists in the graph so set operations are faster.

Auxiliary graphs and prefix sets are fundamentally different and complementary optimizations.
Auxiliary graphs speed up set operations by pruning their inputs; prefix sets execute set operations as early as possible in the loop hierarchy using the same inputs.
Auxiliary graphs can speed up the calculation of prefix sets. 


Each auxiliary graph is relative to a \emph{pair} of query vertices, which we denote as $v_i$ and $v_k$ in the following.
The auxiliary graph $A(v_k, v_i)$ contains the pruned adjacency lists of the vertices matching $v_k$, which are then used instead of the original graph to compute prefix or candidate sets for $v_i$.
The way the pruning occurs depends on how $v_i$ and $v_k$ are connected in the query graph.

The auxiliary graph optimization has two main steps. 
%Note that since a candidate set is a special case of prefix sets (see for example Algorithm~\ref{algorithms:Q1-Prefix}), we focus our description on the computation of prefix sets.
At loop depth $h$, we compute pruned adjacency lists for the computation of a future prefix or candidate set. Then, at loop depth $k > h$, we use the pruned adjacency lists to speed up the computation of that set. The basic idea poses two core questions (1) which adjacency lists to prune and (2) how to prune the adjacency lists to make auxiliary graphs beneficial. We next answer these two questions and discuss our solutions. 

\subsection{Identifying the Adjacency Lists to Prune}
\label{sec:eager}
Consider building an auxiliary graph $A_h(v_k,v_i)$ at some loop depth $h$.
Our goal is to prune away some of the vertices in $N(u_k)$, which match $v_k$, in order to accelerate the computation of $C_k(v_i)$ at a deeper loop depth $k > h$. Specifically, we would like prefix set calculation to become: 
\begin{align}
    &\text{At loop h:} \quad \text{Compute } P_h(u_k) \subset N(u_k), \\ 
    &\text{At loop k:} \quad C_k(v_i) = C_{k-1}(v_i) \circ_k P_h(u_k).
    \label{eqn:target}
\end{align}
In other words, we want to replace the adjacency list $N(u_k)$ with a pruned version $P_h(u_k)$ in Eqn.~\ref{eqn:prefix_prefix_computation}.
This reduces the size of the input of the set operation $\circ_k$ and thus its running time.

To prune $N(u_k)$, we need to know the vertex $u_k$.
At loop $h$, however, we only have a partial match $I_h =[u_1 \ldots u_h]$ which is a prefix of $I_k$ and does not include $u_k$.
The question is, how can we identify $u_k$ so that we can prune its adjacency list?

Our proposed solution is to prune at loop $h$ the adjacency lists of the vertices in the prefix set $C_h(v_k)$.
%, which by definition is a superset of $C(u_k)$ and hence include all potential $u_k$.
The solution is based on the properties of prefix sets.
The data vertex $u_k$ is one of the vertices matching the query vertex $v_k$ by definition.
It holds that:
\begin{equation}
u_k \in C(v_k) = C_{k-1}(v_k) \subseteq C_h(v_k).
\label{eqn:identify-lists-to-prune}
\end{equation} 
% In fact, we know by definition that $u_k$ is in the candidate set $C(v_k)$.
When using the prefix optimization, the candidate set $C(v_k)$ is equal to the last of its prefix sets $C_{k-1}(v_k)$.
The prefix sets are built to incrementally remove candidate vertices using set operations, so $C(v_k) \subseteq C_h(v_k)$. 
Our strategy is thus to \emph{prune all adjacency lists} of the vertices in $C_h(v_k)$ as we would prune the adjacency list of $u_k$.
We refer to it as the \textit{eager} strategy. 

% We store these pruned adjacency lists in an auxiliary graph and reuse them later.
% Pruning adjacency lists for a superset of the candidate set $C(v_k)$ may result in some extra work, but this is outweighed by the benefits of speeding up later set operations.
% We refer to the strategy described in this subsection as 


\subsection{Pruning the Adjacency Lists}
After identifying the adjacency lists to prune, the next question is how to prune.
We want to produce a pruned version of the adjacency list $N(u_k)$ and use that instead of $N(u_k)$ to compute $C_k(v_i)$ at loop $k$ using Eqn.~\ref{eqn:prefix_prefix_computation}.
The idea is to prune the adjacency list at loop depth $h$ and then reuse it multiple times at loop depth $k$.
Even though at loop $h$ we do not know exactly which vertices match $v_i$, we can already tell that vertices that are not in $C_h(v_i)$ are definitely not matches, so we can remove them from $N(u_k)$.
The result will not change because of the following observation from the set theory. 


% We use Figure~\ref{figure:compare} as an example to show how we prune the adjacency lists. 
% We use the same color to highlight the adjacency lists or pruned adjacency lists of the same vertices. 
% For example, the adjacency lists of $\circled{6}$ consists of $\{1,2,3,4,5,7\}$. 
% The pruned adjacency lists of $\circled{6}$ consists of $\{1,2\}$. Both of them are in red color.

% To prune the adjacency list $N(u_k)$ we leverage the structure of the query graph.
% The prefix set $C_{k-1}(v_i)$ in Eqn.~\ref{eqn:target} contains the result of set operations among the adjacency lists of the vertices that have been matched at loop $k-1$ (in red in  Figure~\ref{fig:pruning-example}).
% These set operations depend on the query vertex $v_i$ and the structure of the graph.
% Even though we don't have $C_{k-1}(v_i)$ yet at loop $h$, we do have $C_h(v_i)$, which is a superset of  $C_{k-1}(v_i)$ (in blue in Fig.~\ref{fig:pruning-example}).

\begin{lemma}[Superset-based pruning rule]
\label{lem:pruning}
    Let $C$, $C'$, $P$, and $N$ be sets, and $\circ$ denote either the set intersection or the set subtraction operator.
    If $C \subseteq C'$ and $P = C' \cap N$ it holds that: 
    $$
        C \circ N = C \circ P
    $$
\end{lemma}

We use this rule to compute a pruned version of $N(u_k)$ for the auxiliary graph of $v_i$ at loop $h$.
We call this the \emph{pruned adjacency list} $P_{h,k}(u|v_i)$ and define it as follows:
\begin{equation}
    P_{h,k}(u|v_i) = C_h(v_i) \cap N(u), \quad u\in C_h(v_k).
    \label{eqn:prune-compute}
\end{equation}
Note that we use the notation $u$ instead of $u_k$ because $u$ is in the prefix set of $v_k$ at loop $h$ but it may not end up being a candidate for $v_k$.
Each pruned adjacency is specific to a query vertex $v_i$ because it is filtered using a prefix set of $C(v_i)$.

At loop $h$, we compute the pruned adjacency list.
Later, we use the pruning rule again at loop $k$ and replace Eqn.~\ref{eqn:prefix_prefix_computation} with the following expression:
\begin{equation}
    C_k(v_i) = C_{k-1}(v_i) \circ_k P_{h,k}(u_k|v_i)
    \label{eqn:prune-use}
\end{equation}
This expression is equivalent to Eqn.~\ref{eqn:prefix_prefix_computation} because of the superset pruning rule (Lemma~\ref{lem:pruning}) since $ C_k(v_i) \subseteq C_{k-1}(v_i)$.

In summary, we still compute  $ C_k(v_i)$ incrementally from $C_{k-1}(v_i)$ as in Eqn.~\ref{eqn:prefix_prefix_computation}, but we now do it using the pruned adjacency list $P_{h,k}(u_k|v_i)$ to speed up the execution of the set operation $\circ_k$.

\subsection{Putting It All Together}
The auxiliary graph $A_h(v_k,v_i)$ at loop depth $h$ includes all the pruned adjacency lists $P_{h,k}(u|v_i)$ for each $u\in C_h(k)$.
It optimizes the execution of the set operation $\circ_k$ in two steps:
\begin{enumerate}
    \item At loop $h$, we prune $N(u)$ by computing $P_{h,k}(u|v_i)$ as in Eqn.~\ref{eqn:prune-compute}, for each $u \in C_h(v_k)$. 
    \item At loop $k > h$, we compute $C_k(v_i)$ using $P_{h,k}(u|v_i)$ as in Eqn.~\ref{eqn:prune-use}.
\end{enumerate}

Building an auxiliary graph requires two prefix sets, which we call the \emph{selecting set} and the \emph{filtering set}.
The selecting set is the prefix set $C_h(v_k)$ in Eqn.~\ref{eqn:identify-lists-to-prune} used to select which adjacency lists to prune. 
The filtering set is the prefix set ($C_h(v_i)$ in Eqn.~\ref{eqn:prune-compute}) used to compute the pruned adjacency lists by intersecting it with the adjacency lists of the vertices in the selecting set. 
It determines how to prune the adjacency lists before adding them to the auxiliary graph.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{sigmod-figures/example.png}
    \captionof{figure}{Minigraph Pruning Example}
    \label{figure:example}
\end{figure}

\subsection{Example of Pruning} 
We use the example in Figure~\ref{figure:example} to illustrate how the proposed auxiliary graph works. Figures~\ref{figure:example}(a) and (b) shows the original data graph and its adjacent lists.

After $u_1$ is matched to node $1$, $C(v_3)$ and $C(v_4)$ will always be a subset of $N(1)$ in the inner loops, because the query schedule requires that $u_3$ and $u_4$ must be the neighbors of $u_1$. To accelerate the computation for $C(v_4)$, we can prune the adjacency lists of the vertices in $ \{2, 4, 5\} \: (N(1))$ by intersecting with them with $N(1)$. The resulting pruned adjacency lists $P_{1,3}(u|v_4)$ will be subsets of the original adjacency lists $N(u_3)$. 
Then, we can replace $N(u_3)$ in the computation for the candidate set $C(v_4)$ without affecting the results.
\begin{comment}
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/running-example.png}
    \caption{Building and using the auxiliary graph $A_1(v_3, v_4)$ in the example of Figure~\ref{fig:runningexample}. Colors match full adjacency lists on the left with the corresponding pruned lists on the right.
    }
    \label{figure:compare}
\end{figure*}
\subsection{Example} 
We use the example in Figure~\ref{figure:compare} to illustrate how the proposed auxiliary graph works. Figures~\ref{figure:compare}(a) and (b) show how prefix optimization and auxiliary graph accelerate the set operations, respectively. 

The prefix set optimization caches loop-invariant computation to reuse them in future set operations. Consider the DFS paths $\circled{7}\circled{6}\circled{2}$ and $\circled{7}\circled{6}\circled{1}$. The prefix optimization caches the results of $N(7) \cap N(6) $ after matching $\circled{7}\circled{6}$. It then reuses the results twice to compute the candidate set $C(v_4)$. This works because the cached set operation is loop-invariant, and the results can be used to compute $C(v_4)$ regardless of whether $\circled{1}$ or $\circled{2}$ will be matched to $v_3$. 

Auxiliary graphs accelerate the set operation by replacing the adjacency lists used in the computation that is not cached by prefix optimization. Consider the path $\circled{7}\circled{1}\circled{6}$ and $\circled{7}\circled{2}\circled{6}$.
We first prune the adjacency list of $\circled{6}$ after matching $\circled{7}$. We then use the pruned adjacency lists of $\circled{6}$ to compute $C(v_4)$. The pruned adjacency list of $\circled{6}$ ($\{1, 2\}$) is much shorter than the original adjacency list of $\circled{6}$ ($\{1,2, 3, 4, 5, 7\}$) so the set operation can be faster to compute.   

The data vertex \circled{6} is matched twice to $u_3$ at depth three. 
Thus, its adjacency list is used twice to find matches of the query vertex $u_4$.
Auxiliary graphs prune this adjacency list once after matching $\circled{7}$ at loop depth one and then use it twice at depth three.
\end{comment}

%We next discuss how our Minigraph system manages the complexity of the building, storing, and retrieving such a potentially large number of pruned adjacency lists using auxiliary data structures.

==> sigmod-sections/4-Analysis.tex <==
\section{Pruning Cost Analysis}
When pruning an adjacency list, we pay an upfront cost that we should amortize later.
The gain of pruning depends on how we select the vertices whose adjacency lists to prune, i.e., how we determine the selecting set of an auxiliary graph.
So far we discussed an \emph{eager} strategy, which selects all vertices $u \in C_h(v_k)$ and ensures that we prune the adjacency lists of every candidate of $v_k$ as early as possible.
In this section, we discuss two different strategies to remedy this problem. 

We first discuss a \emph{static} approach that only prunes vertices which guarantee no extra computation overhead. Next, we analyze the cost and benefits of pruning an adjacency list. We find that \emph{eager} pruning does not always guarantee computational gains, as also shown by our experimental evaluation. Based on the analysis, we propose an \emph{online} approach which uses the runtime information to decide which adjacency lists to prune.

\subsection{Static Approach}
% This analysis motivates a different approach than the eager one to select the vertices whose adjacency lists are pruned.
The eager approach tries to prune the adjacency lists of all the candidates $u_k \in C(v_k)$, which are unknown at loop $h$, without ascertaining that this cost will be amortized later.
% Calculating the gain requires knowing parameters that cannot be computed online in a cost-effective manner.

\paragraph{Static Strategy} Our \emph{static approach} only prunes the adjacency list of a vertex $u$ when this comes at \emph{no extra cost}.
Consider that we want to compute the pruned adjacency lists $P_{h,k}(u|v_i)$ at loop $h$ to find matches for query vertex $v_i$.
The static approach leverages that loop $h+1$ computes the prefix set:
\begin{equation}
    \label{eqn:static}
    C_{h+1}(v_i) = C_h(v_i) \circ_{h+1} N(u), \quad \forall u \in C(v_{h+1})
\end{equation}
If $\circ_{h+1}$ is a set intersection, the right hand side of Eqn.~\ref{eqn:static} can be seen as an instance of Eqn.~\ref{eqn:prune-compute}, where we compute $P_{h,k}(u|v_i)$ using the same filtering set $C_h(v_k)$ but a different selecting set $C(v_{h+1})$.
The static approach checks if $C(v_{h+1})$ is a subset of $C_h(v_k)$.
This check is done at compile time by examining the structure of the query graph and the set operations required to obtain the two prefix (candidate) sets.
If the check is positive, we compute Eqn.~\ref{eqn:static} and store the results as pruned adjacency list $P_{h,k}(u|v_i)$ at loop $h$.
Then, we reuse those results at loop $h+1$ as $C_{h+1}(v_i)$.

\subsection{Benefits and Cost of Pruning}
The \emph{eager} approach we describe previously computes the pruned adjacency list $P_{h,k}(u|v_i)$ at loop $h$ for each vertex $u \in C_h(k)$.
We now perform a cost-benefit analysis of computing the pruned adjacency list.
The purpose of $P_{h,k}(u|v_i)$ is to speed up the computation of $C_k(v_i)$ at loop $k$.
We express gains in terms of the reduction in the number of comparisons required to perform this computation. We assume the input adjacency lists are sorted and we estimate the number of comparison using sum of the set sizes.

Before starting the analysis, we give some definitions.
When our algorithm computes a pruned adjacency list at loop $h$, it reaches that loop depth after obtaining a partial match $I_h$.
The pruned adjacency list will be used in the nested loops at a higher depth than $h$, where all the partial and final matches will be extensions of $I_h$. 
We use $e(I_h, k, u)$ to denote the set of all partial matches of size $k$ that extend $I_h$ where the data vertex $u$ matches the query vertex $v_k$.
%The function $\hat{C}_k(u_k,I_h)$ returns $1$ if $u_k$ is in some candidate set $C(v_k)$ computed by extending the partial match $I_h$ and $0$ otherwise.
Note that each prefix set $C_j(v_i)$ is calculated after having obtained a partial match $s_j$, for any value of $j$.
We say in that case that $C_j(v_i)$ is relative to $s_j$. 
We still use the notation $C_j(v_i)$ instead of a more precise $C_{j,s_j}(v_i)$ for simplicity.

We start by counting the number of comparisons performed at loop depth $k$ without auxiliary graphs, using the expression of Eqn.~\ref{eqn:prefix_prefix_computation}.


\begin{equation*}
    o(I_h,k,u,i) = \sum_{I_k \in e(I_h,k,u)} |C_{k-1}(v_i)| + |N(u)|
\end{equation*}

%previous
% \begin{equation}
%     o(k,i,I_h) = \sum_{u_k \in \hat{C}(v_k,I_h)}\sum_{I_k \in e(I_h,k,u_k)} |C_{k-1}(v_i)| + |N(u_k)|
% \end{equation}

We assume that the sets $C_{k-1}(v_i)$ and $N(u)$ are sorted lists and that the set operation scans them.
The worst-case running time of the set operation is thus the sum of the cardinality of the two sets.

With auxiliary graphs, the cost becomes:
\begin{align*}
    a(I_h,k,u,i) =& \: |C_h(v_i)|+|N(u)| +\\
    & \sum_{I_k \in e(I_h,k,u)} |C_{k-1}(v_i)|+|C_h(v_i) \cap N(u)|
\end{align*}
% \begin{align}
%     a(k,i,I_h) =& \sum_{u_k \in \hat{C}(v_k,I_h)}\Big( |C_h(v_i)|+|N(u_k)| +\\
%     & \sum_{I_k \in e(I_h,k,u_k)} |C_{k-1}(v_i)|+|C_h(v_i) \cap N(u_k)| \Big) \\
%     & + \sum_{u_k \in C_h(v_k) \setminus \hat{C}(v_k,I_h)} |C_h(v_i)|+|N(u_k)|
% \end{align}
The first line of the equation is the cost of computing the pruned adjacency lists at loop $h$ using Eqn.~\ref{eqn:prune-compute}.
The second line is the cost of using the pruned adjacency list, which has size $|C_h(v_i) \cap N(u)|$.
For each vertex $u_k \in C(v_k)$, we compute $C_k(v_i)$ using Eqn.~\ref{eqn:prune-use}.

The gain of building a pruned adjacency list at loop $h$ can thus be expressed as follows.
% We use $pc(h,i,k) = |C_h(v_i)|+|N(u_k)|$ to express the cost of computing the pruned adjacency list $P_h(u_k|v_i)$.
\begin{align*}
    g(I_h,k,u,i)  =& \: o(I_h,k,u,i) - a(I_h,k,u,i)\\
                % =& \sum_{u_k \in \hat{C}(v_k,I_h)} \Big(\big(\sum_{I_k \in e(I_h, k, u_k)} |N(u_k)| - |C_h(v_i)\cap N(u_k)|\big)\\
                % &- pc(h,i,k)\Big)\\
                % -& \sum_{u_k \in C_h(v_k) \setminus \hat{C}(v_k,I_h)} pc(h,i,k)\\
                =& \: |e(I_h, k, u)| \cdot (|N(u)| - |C_h(v_i)\cap N(u)|)\\
                -& \: (|C_h(v_i)|+|N(u)|).
\end{align*}
% \begin{align}
%     g(k,i,I_h)  =& \: o(k,i,I_h) - a(k,i,I_h)\\
%                 % =& \sum_{u_k \in \hat{C}(v_k,I_h)} \Big(\big(\sum_{I_k \in e(I_h, k, u_k)} |N(u_k)| - |C_h(v_i)\cap N(u_k)|\big)\\
%                 % &- pc(h,i,k)\Big)\\
%                 % -& \sum_{u_k \in C_h(v_k) \setminus \hat{C}(v_k,I_h)} pc(h,i,k)\\
%                 =& \sum_{u_k \in \hat{C}(v_k,I_h)} |e(I_h, k, u_k)| \cdot (|N(u_k)| - |C_h(v_i)\cap N(u_k)|)\\
%                 -& \sum_{u_k \in C_h(v_k)} |C_h(v_i)|+|N(u_k)|
% \end{align}
% previous

% \begin{align}
%     \sum_{u_k \in C(v_k)}&\Big( |C_h(v_i)|+|N(u_k)| + \\
%     &\sum_{\langle u_1, \ldots, u_k \rangle \in ext(I_h)} |C_h(v_i) \cap N(u_k)| - |N(u_k)| \Big) + \\
%     \sum_{u_k \in C_h(v_k) \setminus C(v_k)}& |C_h(v_i)|+|N(u_k)|
% \end{align}
This expression shows that pruning is not always advantageous.
The eager strategy we have discussed previously prunes the adjacency lists of each $u \in C_h(v_k)$, but this does not guarantee that there is a gain.
Ideally, we would like to compute $P_{h,k}(u|v_i)$ if and only if the gain is positive for a given vertex $u$. 


\paragraph{Online Strategy} Based on the previous analysis, we propose an \emph{online} variant of the static approach. Besides pruning adjacency lists that will not bring extra cost like the \emph{static} approach does, the \emph{online} approach also uses runtime information to decide which other adjacency lists to prune.
% This variant uses the same compile-time strategy as the static approach to prune adjacency lists. 
% It also prunes additional adjacency lists using the cost model described above and runtime information. 

When deciding whether to prune an adjacency list, the two unknown factors in the analysis are $|e(I_h, k, u)|$ and $|C_h(v_i) \cap N(u)|$. 

To estimate the size of $|C_h(v_i) \cap N(u)|$ we assume that each vertex in $N(u)$ are equally likely to be inside $C_h(v_i)$ like all other vertices ($V$) in the graph. Then, we can express $|C_h(v_i) \cap N(u)|$ as:
\begin{equation*}
    |C_h(v_i) \cap N(u)|  = \frac{|C_h(v_i)| \times |N(u)|}{|V|}
\end{equation*}

To estimate $|e(I_h, k, u)|$, we assume all the vertices in $C_h(v_k)$ are equally likely to appear in $C(v_k)$ as we extend $I_h$ to $I_k$. Then, we can express $|e(I_h, k, u)|$ as:

\begin{align*}
    |e(I_h, k, u)|  =& \sum_{u_{h+1} \in C(u_{h+1})} \sum_{u_{h+2} \in C(u_{h+2})} \dots \sum_{u_{k} \in C(u_k)} \frac{1}{|C_h(v_k)|}
\end{align*}

Since the cardinality of $C(u_{h+1}), \dots C(u_k)$ are unknown at the time we just obtain $I_h$, we uniformly estimate their sizes. 

\begin{align*}
    |e(I_h, k, u)|  \approx \prod E(|C(u_{h+1})|) \dots \prod E(|C(u_{k})|) \frac{1}{|C_h(v_k)|}
\end{align*}

Similar to GraphPi~\cite{GraphPi}, we use topological information to further estimate the expected cardinality of the candidate sets based on the size of their parent prefix sets at loop $h$ (ex. $C_h(u_{h+1}), \dots C_h(u_k)$). 

\jl{TODO: write the remaining cost model. }
%The first term represents a positive gain, since we know that $|N(u)| \geq |C_h(v_i) \cap N(u)|$.
%To maximize this gain we want to prune large adjacency lists and achieve high pruning power, i.e., $|N(u)| \gg |C_h(v_i) \cap N(u)|$.
%\ms{A simple way to estimate the first parameter is to perform some matching (i.e., exploring a subset of the exploration tree) with pruning always on and measure it.} \jl{Using average degree/triangles to estimate this becomes inaccurate, sampling more statistics might be helpful.}
% Our approach is to estimate the gain at runtime every time we need to decide whether to compute $P_{h,k}(u|v_i)$ and then check it against a static threshold to see if pruning is beneficial. 
% We can express the requirement that $g(I_h,k,u,i) \geq 0$ in the following condition:
% \begin{align*}
%     |C_h(v_i)\cap N(u)| \leq & (1-1/|e(I_h, k, u)|)\cdot |N(u)|\\
%                           & - |C_h(v_i)|/|e(I_h, k, u)|.
% \end{align*}


\begin{comment}
Computing at runtime whether this predicate holds for a vertex $u$ is more expensive than pruning eagerly.
It is possible to calculate $|C_h(v_i) \cap N(u)|$ at loop $h$ by performing the set intersection, but this has the same cost as computing $P_{h,k}(u|v_i)$ eagerly.
The value of $|e(I_h, k, u)|$ counts how many times we reuse the pruned adjacency list.
Unfortunately, this parameter is also unknown at loop $h$, since it requires finding the partial matches that extend the current partial match.

If $|e(I_h, k, u)|$ is $0$ or $1$, pruning the adjacency list will not be beneficial independent of the value of $|C_h(v_i)\cap N(u)|$.
As $|e(I_h, k, u)|$ grows, it is more likely that we can amortize the cost of pruning since the pruned list will be reused many times.
\end{comment}

%\subsection{Estimating the Opportunities for Reuse}
%As expected, the right hand side of the inequality grows monotonically as that parameter grows.
% If we assume that $|e(I_h, k, u)| \geq \hat{e}$, for some constant $\hat{e}$, then we know that pruning the adjacency list will bring a gain if:
% \begin{align*}
%     |C_h(v_i)\cap N(u)| \leq & (1-1/\hat{e})\cdot |N(u)| \\
%                           & - |C_h(v_i)|/\hat{e}
% \end{align*}

\begin{comment}
We notice that there is a path between any vertex in $C_h(v_i)$ and $u$. 
This is because we materialize $C_h(v_i)$ if and only if $v_i$ is connected to at least one matched vertex $v_j (j < h)$. 
Consequently, all the vertices in $C_h(v_i)$ are neighbors of $u_j$. 
A similar argument holds for $C_h(v_k)$, the selecting set from which $u$ is drawn.
Since partial matches are connected (\ref{connected_ordering}), $u$ can form a path to $u_j$ and any $u$'s neighbor can form a path to any $u_j$'s neighbor. 
Therefore, a vertex in $|C_h(v_i) \cap N(u)|$ closes that paths and makes it a ring.

We assume that the path between the vertices in $C_h(v_i)$ and $u$ is a wedge that becomes a triangle if it is closed.
This simplification was also used to obtain GraphPi's cost model~\cite{GraphPi} and allows us to leverage the triangle count, a statistic that is commonly available, to perform our estimate.
Let $p$ be the probability of closing a random edge and form a triangle:
\begin{equation*}
    p = P(b \in N(a) | a, b, c \in V, a, b \in N(c))
\end{equation*}
In our case, we have that $a$ is $u$, $b$ is a vertex of $C_h(v_i)$, and $c$ is some matched vertex that connects $a$ and $b$. 
The size of the intersection is then $|C_h(v_i) \cap N(u)| = |C_h(v_i)| \cdot p$, where $p = \frac{tri\_cnt \cdot |V|}{(2 \cdot |E|)^2}$ and $tri\_cnt$ is the number of triangles in the input graph.

We can now obtain our final expression to evaluate whether to compute $P_{h,k}(u|v_i)$ as:

\begin{align}
    |C_h(v_i)| \cdot \frac{tri\_cnt \times |V|}{(2 \times |E|)^2} \leq & (1-1/\hat{e})\cdot |N(u)|  \\
                           & - |C_h(v_i)|/\hat{e}.
\end{align}
\end{comment}


==> sigmod-sections/5-Compilation.tex <==
% \section{Minigraph: A Subgraph Enumeration System} \label{section:methodology}


\section{Generating Query Execution Code}
\label{sec:reduceoverhead}
% We now discuss Minigraph, a new subgraph enumeration system that uses proactive online graph pruning to obtain auxiliary graphs and speed up query execution.
% In Section \ref{section:criteria}, we discussed the criteria used by Minigraph to prune the adjacency lists. 
We now discuss the Minigraph code generator, which minimizes the runtime overhead of handling auxiliary graphs.
% We then show an example of query execution code using auxiliary graphs.

\subsection{Code Generating Process}
Minigraph generates code in three steps. 
In the first step, Minigraph generates code for the standard algorithm using only prefix optimizations. 
It then searches for opportunities to prune adjacency lists based on the criteria discussed in the previous sections.
It groups these pruned lists into multiple auxiliary graphs and considers them as candidates to inject into the generated code.
In the second step, Minigraph visits all the candidate auxiliary graphs and removes duplicates. 
In the final step, it injects the logic of building and using auxiliary graphs into the generated code.
We now discuss some details of this process.
%\hui{since compilation process has the auxiliary graph based optimization. People would expect the evaluation to report how much time spend on compilation} \jl{changed and add experiment results}

\begin{comment}
\subsection{Materializing Auxiliary Graphs During Runtime}
\hui{I cannot get much info from this subsection. Might consider removing this subsection to save space.} \jl{I agree, it is removed}
Minigraph organizes the pruned adjacency lists into multiple auxiliary graphs, each stored in CSR format.
Minigraph keeps a separate version of the same auxiliary graph at each loop depth.
When the algorithm moves to a deeper loop depth, it builds a new version of the auxiliary graph by pruning the version of the parent loop.
When the algorithm backtracks to a parent loop depth, it adopts the parent's version.
\hui{This paragraph makes me feel that the auxiliary graph is computed during compile time because you mention "materialize auxiliary graphs". But I thought auxiliary graphs are computed during runtime given a search query, right? Should we say "Materializing auxiliary graph during runtime"?} 


Minigraph \emph{materializes} an auxiliary graph when both the selecting-set and the filtering-set it uses have been materialized (see Definition~\ref{def:prefix-set}).
% These prefix sets are materialized when they effectively restrict the scope of candidates for a query vertex, as discussed in Section~\ref{section:prefix-optimization}.
% 
More specifically, to build an auxiliary graph for computing $C_k(v_i)$ at loop depth $h$, $C_h(v_i)$ (the filtering-set) and $C_h(v_k)$ (the selecting-set) need to be both materialized at loop $h$. 
% We then build the version of the auxiliary graph of vertex $v_i$ at loop $h$ as:
% \begin{equation}
%     A_h(v_k, v_i) = P_{h,k}(u|v_i), \quad \forall u \in C_h(v_k)
% \end{equation}

% For each vertex in $C_h(v_k)$ we compute the intersection of its adjacency list with $C_h(v_i)$ and the result is $P_h(u_k|v_i)$, the pruned adjacency list of $u_k$ at loop $h$ for the set operation to compute $C_k(v_i)$. 
% We store these pruned adjacency lists in the same auxiliary graph.
% We denote this auxiliary graph as $A(C_h(v_k), C_h(v_i))$.
% where:
% \begin{equation}
%      P^h_i(u_k) = C_h(v_i) \cap N(u_k) \quad (\forall u_k \in C_h(v_k))
%      \label{eqn:auxiliary-compute}
% \end{equation}
% Where $N^k_h(u_i)$ can replace $N(u_i)$ as input for computing $C_i(v_k)$.
%It is essential that each pruned adjacency list can be used for multiple times such that the overhead of computing it can be amortized. 

At loop level $h$, Minigraph prunes only the adjacency lists of the query vertices $v_i$ that will be matched at least two loop levels deeper than $h$, i.e., when $i>h+1$.
That is because if $i=h+1$ then at loop depth $h$ we match the query vertex $v_{h+1}$ and obtain $C(v_{h+1})$.
The adjacency list $N(u_{h+1})$ of a vertex $u_{h+1} \in C(v_{h+1})$ is used at most once for the target computation at loop $h+1$.
\end{comment}
% The same logic applies to the case where $h < i - 2$. 
% The higher the loop we build the pruned adjacency lists, the more likely it will be reused multiple times in the deeper loops. 

%We choose $h \leq i - 2$ so the cost can be amortized to some extent. 
% There is no guarantee that the pruned adjacency lists in a materialized auxiliary graph will be used multiple times, especially in small data graphs. However, they can effectively reduce the size of large adjacency lists that are slow to compute and are often accessed many times in future set operations. Reducing the size of these large adjacency lists can significantly speed up the query. 

\subsection{Compile-Time Optimizations}

\subsubsection{Reusing Auxiliary Graphs}
\label{sec:reuse}
The standard algorithm code generated by systems like GraphPi reuses the content of prefix sets that have already been computed.
Every time the standard algorithm needs to perform a set operation, the compiler checks whether there exists some other prefix set or candidate set that has already computed the same result by applying the same set operations to the same inputs with the same canonicality checks.
For example, in Algorithm~\ref{algorithms:Q1-Prefix} the compiler can establish that $C(v_3) = C_2(v_4)$ at line~\ref{ln:reuse}  since they are both computed as $N(u_1) \cap N(u_2)$

The Minigraph compiler extends this mechanism to auxiliary graphs.
Every time the standard algorithm needs to compute a set operation $S \cap N(u)$, the compiler checks if there exists an auxiliary graph $A$ such that (i) $S$ is equivalent to the selecting set of $A$, and (ii) $u$ is included in the filtering set of $A$.
Like in the previous case, these checks are performed by examining at compile time the set operations used to compute the selecting and filtering sets of $A$ and their inputs.

\subsubsection{Removing Duplicated Auxiliary Graphs}
\label{sec:duplicated}
The compiler avoids generating duplicated auxiliary graphs at runtime.
Two auxiliary graphs are identical if both have the same filtering-set and selecting-set. 
To avoid building such auxiliary graphs repeatedly, the compiler compares the filtering set and the selecting set of different auxiliary graphs. 
% Two prefix sets are identical if both have the same set intersections and set subtractions that need be conducted at query execution. Eqn~\ref{eqn:naive_prefix_computation}. 
The filtering set and selecting set are prefix sets and the compiler checks if two prefix sets are identical as discussed previously.
% If two prefix sets are computed by intersecting the adjacency lists of the same set of vertices and subtracting the neighbors of the set of vertices, and the canonicality checks are the same, then the two prefix sets are equivalent. 
We use this rule to compare prefix sets and remove the duplicated auxiliary graphs at compile time. 
The code generator performs these checks and produces code that uses the right auxiliary graph, without performing further online checks.
% \ms{how is this check performed? it could be expensive} \jl{addressed} 

% Analyzing of the relationship between different auxiliary graphs is straight forward. 
% Two auxiliary graphs can be either inclusive or exclusive. One auxiliary graph can include the other auxiliary graph when its selecting-set and filtering-set are both superset of those of the other auxiliary graph. Two auxiliary graphs are are exclusive otherwise, as they either have mutually exclusive selecting-set or filtering-set. Two auxiliary graphs can also be identical, if they have exactly the same selecting-set and filtering-set, a special case where the two graphs include each other simultaneously.
% If there are multiple auxiliary graphs that can be materialized in the same loop, we only need to materialize the ones that include the others. If they are materialized in different loops, we can use the larger auxiliary graph to build the auxiliary graphs it includes. 

\subsubsection{Building An Auxiliary Graph From Another}
In addition to using the pruned adjacency lists to speed up set operations for computing prefix sets, we can also use the auxiliary graph to speed up the construction of another auxiliary graph.

For example, assume we can build two auxiliary graphs at loop level $h$ and $h+1$ respectively, both auxiliary graphs intend to accelerate the computation for $C_k(v_i)$. We refer to the auxiliary graphs as $A_h(v_k, v_i)$ and $A_{h+1}(v_k,v_i)$ respectively. The key idea is that we can use $A_h(v_k, v_i)$ to speed up the construction of $A_{h+1}(v_k,v_i)$. 

% Notice that the larger auxiliary graph must be materialized in previous loops before materializing the smaller one because of the property of prefix sets discussed in section \ref{section:property_of_prefix}. We call the larger auxiliary graph the parent auxiliary graph and its subset the child auxiliary graph. 
Consider the auxiliary graph $A_{h+1}(v_k,v_i)$. We can utilize the pruned adjacency list $P_{h, k}(u | v_i)$ to compute the pruned adjacency list $P_{h+1, k}(u | v_i)$ since:
\begin{align*}
P_{h+1,k}(u | v_i) &=  C_{h+1}(v_i) \cap N(u) \\
    &= C_{h+1}(v_i) \cap C_h(v_i) \cap N(u) \\
%    &= C_{h+1}(v_i) \cap (C_h(v_i) \cap N(u)) \\
    &= C_{h+1}(v_i) \cap P_{h,k}(u | v_i).
\end{align*}
Thus we can use the pruned adjacency lists in $P_{h,k}(u | v_i) \in A_h(v_k,v_i)$ to construct $A_{h+1}(v_k,v_i)$.

% We know $C_{h+1}(v_k) \subseteq C_h(v_k)$  
% We can therefore use $N^k_h(u_i)$ to replace $N(u_i)$ in the set intersection. 
% This is correct as shown in Lemma~\ref{lemma-3} and~\ref{lemma-4}. 
% In addition, the $C_h(v_i)$ is superset of $C_{h+1}(v_i)$, which means $A(C_h(v_k), C_h(v_i))$ contains all the pruned adjacency lists required in the set intersections that build the pruned adjacency lists in $A(C_{h+1}(v_k), C_{h+1}(v_i))$. 

In summary, if both the selecting-set and the filtering-set of an auxiliary graph $A$ are supersets of those of another auxiliary graph $A'$, Minigraph generates code that uses $A$ to build $A'$. 

% \subsubsection{Amortizing the Overhead of Pruning Adjacency Lists}


%We leave more sophisticated strategies to the future work.
% The set of vertices in the child pruned graph ($S_h^{k-1}$) is a subset of the set of vertices in the parent pruned graph ($S_h^{k}$). This is because the parent pruned graph contains all the vertices and edges in the child pruned graph so it can be used to build the child pruned graph.

% Consider the computation for building the child pruned graph, for each vertex in $S_h^k$, we need to compute the set intersection between its adjacency list $N(u_h)$ in the original graph with an the prefix set $S_i^k$. Now, if its parent pruned graph $G_{p}(S_i^{k-1}, S_h^{k-1})$ has been built, we can instead use the adjacency list of $u_h$ in the parent pruned graph instead of its adjacency list in the original graph to compute the set intersection. The results will be the same due to the set property discussed in section \ref{section:set-property}. 

% \subsection{ Algorithm Complexity }
% To identify the opportunities for adjacency lists pruning, we can analysis the computation for each prefix set $S_i^h$ and check if any pairs of $S_i^k \text{ and } S_h^k $ have been materialized and $k \leq j - 2$. 

% The entire algorithm is in $O(|V_p|^3)$, because checking if a prefix set can be materialized is constant time operation, the total number of prefix set to be checked is bounded by $O(|V_p|^2)$, and for each prefix set we need to check $O(|V_p|)$ different values of $k$. Multiplying them together gives $O(|V_p|^3)$.

% In reality, the size of the pattern graph $|V_p|$ tends to be small and this marking process can be done in almost no time.

% We greedily mark the opportunities of materializing its pruned graphs for all valid values of $k$. If there are multiple valid $k$, we materialize all of them and use the parent pruned graph to build the child pruned graph as described above.

\begin{comment}
\subsubsection{Pruning Automorphisms}
To prune the automorphisms, the previous systems enforce a set of canonicality checks at run time as discussed in Section~\ref{section:background}. 
Specifically, GraphZero~\cite{GraphZero} and GraphPi~\cite{GraphPi} apply these canonicality checks by performing bounded set operations. 
Assuming the inputs are sorted, the bounded set operations use a vertex id as the upper bound and terminate the operation immediately when the bound is reached. The result of the bounded set operation only contains the vertices within the given bound. 
% \ms{This is hard to follow. Example?}

Minigraph applies this technique also when it builds auxiliary graphs. 
Given an auxiliary graph, Minigraph checks at compile time if all the future set operations using the auxiliary graph are all bounded operations. If all future set operations are bounded and they all use the same matched vertex's id as the upper bound, Minigraph generates code that uses the bounded set intersection to prune the adjacency lists in advance. For example, we can use the bounded set intersection to build auxiliary graphs for clique patterns.
% \ms{This is hard to follow. Example?}
\end{comment}

\subsubsection{Code Generating Cost Analysis}
The number of prefix sets for a query graph q is in $O(|V(q)|^2)$. 
To determine if a prefix set can be accelerated using an auxiliary graph, we need to check at each loop if its parent prefix set and selecting set are both materialized. 

Since the number of loops is in $O(|V(q)|)$ and checking if a prefix set is materialized can be done in $O(1)$, the time complexity of finding all the auxiliary graphs is in $O(|V(q)|^3)$. In practice, this overhead is negligible as the number of vertices in the query graphs are usually small.

% \subsection{Example of Code Generation}
% \label{sec:codegeneration}
% \begin{comment}
% The previous steps decides which set of auxiliary graphs should be materialized by the generated code to speed up set operations. \hui{This sentence also confuse me. I thought auxiliary graph is computed at runtime. Why the final set of materialized auxiliary graph can be used in the generated code since you don't even have the auxiliary graphs yet?}
% \end{comment}
% Algorithm~\ref{algorithms:Q1-Minigraph} shows an example of code generated by Minigraph to further optimize Algorithm~\ref{algorithms:Q1-Prefix}.
% For simplicity, this example uses the eager approach and considers only the auxiliary graph $A_1(v_3,v_4)$.
% % The major difference is colored.
% The behavior of the algorithm is illustrated in Figure~\ref{algorithms:Q1-Minigraph}(b).

% The generated code materializes $A_1(v_3,v_4)$, which contains a pruned version of $N(u)$ with $u \in C(v_3)$, at loop depth 1 (lines~\ref{ln:mini-start}-\ref{ln:mini-end})
% . It then uses the auxiliary graph to speed up the computation of $C(v_4) = C_3(v_4)$ at lines \ref{ln:mini-s4-begin}-\ref{ln:mini-s4}.
% This example also shows how the generated code reuses auxiliary graphs as discussed in Section~\ref{sec:reuse}.
% Instead of computing $C(v_3)$ and $C_2(v_4)$ at line~\ref{ln:mini-compute}, the compiler determined that the code can reuse the auxiliary graph.

% %Minigraph does not build auxiliary graphs for the next two query vertices that are matched, so it builds only one auxiliary graph for $v_4$. 

% \begin{comment}
% Notice that instead of computing $C(v_3)$ and $C_2(v_4)$ at line~\ref{ln:mini-compute}, we can simply read them from the auxiliary graph of $v_4$.
% This is possible even for $C(v_3)$, which refers to a different query vertex than the auxiliary graph, thanks to our compile-time duplicate elimination (see Section~\ref{sec:duplicated}) 
% \ms{is that correct? If so, we need to highlight in the following discussion how what we do is an application of that optimization.}. \jl{commented}

% In fact $C_1(v_4)$, the filtering-set of the auxiliary graph is $N(u_1)$. The pruned adjacency lists in $A_1(v_3,v_4)$ are the results of the set intersection between $N(u_1)$ and $N(u)$. When we retrieve the pruned adjacency list at line~\ref{ln:mini-retrieve}, we set $u = u_2$. 
% This would work because the selecting-set $C_1(v_3)$ is equivalent to $C(v_2)$, which includes all possible $u_2$. Thus, we can simply query the auxiliary graph for the result of the set intersection instead of computing it again. Finally, we use the pruned adjacency lists to speed up the computation for the candidate set $C(v_4)$ at line~\ref{ln:mini-s4}. 
% \end{comment}
% % Notice that we only need to read from the auxiliary graph to match the vertices other than $v_1$. This property can be helpful for out-of-core systems which store the data graph on disks.
% \input{algorithms/Q1-Minigraph}


==> sigmod-sections/6-Implementation.tex <==
% % Two subgraphs are automorphic if they have the same vertices and edges. Automorphic matches to the same query graph are typically considered redundant and are filtered out. Figure \ref{figure:Automorphism-P0} gives an example of automorphic matchings for query pattern $P_0$. All the 4 matchings have the same vertices and edges.



% % \begin{figure}[t]
% %     \centering
% %     \includegraphics[width=0.9\linewidth]{figures/automorphism-P0.png}
% %     \captionof{figure}{Automorphic Matchings For $P_0$}
% %     \label{figure:Automorphism-P0}
% % \end{figure}

% GraphPi \cite{GraphPi} and GraphZero \cite{GraphZero} identify all the pairs of vertices that are symmetrical. We can switch the matched vertices for the two vertices in a symmetrical pair and still get a valid matching. As in figure \ref{figure:Automorphism-P0}, the blue node and the red node are symmetrical as well as the yellow node and the green node are symmetrical as well. If we switch two vertex matched to the blue and the red node in the matched subgraph, the resulting match is still valid. The same is true if we switch the two vertices matched to the green and the yellow node respectively. Without any restrictions, the nested loop algorithm will identify the same subgraph for multiple times.

% This method can prune all the automorphisms, but it makes the set operation more complex as it needs to constantly check if the bound has been reached. 

% To avoid this additional complexity, we pre-compute the bounded length of each vertex's adjacency list with respect to the vertex id. This additional information allow us to perform normal set intersection on the bounded adjacency lists instead of bounded set intersection. Since the vertices in the bounded adjacency lists are all in within the bound (smaller than the vertex's id), the result of set intersection must also be within the bound. 

% For set subtraction, we first perform a normal set subtraction on the bounded adjacency list. However, the result might still contain some vertices outside the bound. We need to perform an additional linear scan to completely remove the vertices outside the bound. We compare the performance of the two approaches in section \ref{section:evaluation}. \jl{add example / visual here}

% We now compare our the state-of-the-art scheduling method with our approach.

% \textbf{State-of-the-art.} GraphPi \cite{GraphPi} and GraphZero \cite{GraphZero} use a brute force approach to select the optimal schedule. The workflow can be described as following:
% \begin{enumerate}
%     \item Generate all possible matching orders for a given query. (There are $k!$ possible matching orders for a query $q$ with $V|q|=k$.)
%     \item Remove the schedules with matching orders that will not perform well based on empirical rules.
%     \item Use a cost model and the statistics of the data graph to select the optimal schedule from the remaining.
% \end{enumerate}
% Both GraphPi and GraphZero assume the cost of a set operations is linear to the size of its inputs. Thus, they use the (estimated) cardinality of its input prefix sets to estimate the cost of the computation. The number of times a set operation is executed can be estimated by multiplying the (estimated) cardinality of the candidate sets traversed in the outer loops. They can compute the cost of a schedule by summing up the (estimated) cost of all the set operations in the generated algorithm.

% GraphZero \cite{GraphZero} uses the total number of vertices ($|V(G)|$) and edges ($|E(G)|$) of the data graph to estimate the cardinality of the prefix sets and candidate sets. GraphPi \cite{GraphPi} additionally use the number of triangles in the data graph to make the estimation more accurate. 
% % This approach can generate a schedule that is or close to the best schedule in for the tested queries \cite{GraphPi}. However, the system needs to rerun the cost model when the data graph is modified.

% \textbf{Our Approach.} \label{scheduler}
% Similar to the state-of-the-art, our approach first generate all the possible schedules for a query $q$ like the state-of-the-art.
% \section{Implementation}
% We implement the Minigraph in C++ based on the implementation of Dryadic~\cite{Dryadic} and GraphPi~\cite{GraphPi}, which are the state-of-the-art compilation-based subgraph enumeration systems. Before we describe our implementation, we first compare the two systems to point out some potential improvements. 

% \spara{Comparing State-of-the-Arts}
% GraphPi~\cite{GraphPi} and Dryadic~\cite{Dryadic} varies in their implementation of the query scheduler, which finds optimal matching order of a query, and the query execution backend, which performs set operations and managing intermediate results. 
% Our evaluation shows that when the query schedules generated by the two systems are the same, Dryadic has a better performance due to its more efficient backend implementation. However, GraphPi can generate more efficient schedule, out-performing Dryadic when their schedules differ. 
% Another difference is that Dryadic's backend supports both vertex-induced and edge-induced subgraph enumeration while GraphPi supports edge-induced patterns only. On the other hand, GraphPi implements optimizations for counting that Dryadic does not implement. 

% As a result, we extend GraphPi~\cite{GraphPi} to support both vertex-induced and edge-induced subgraph enumeration using Dryadic's query execution backend. 
% We use this implementation as a baseline for comparison. 
% We then implement auxiliary graphs on top of the baseline with all the optimizations discussed in Section~\ref{section:background} as well as the techniques related to auxiliary graphs discussed in Section~\ref{sec:auxiliarygraph}. 

% % The query scheduler takes as input a query graph and generates an optimal query schedule. The query schedule is consumed by Minigraph's code generator to produce efficient C++ code. 
% % Besides our proposed dual-sort query scheduler, Minigraph also implements the state-of-the-art scheduler from GraphPi \cite{GraphPi}. 
% % The Minigraph code generator is designed to take an arbitrary schedule as an input. It implements all the optimizations discussed in Section~\ref{section:background} as well as the techniques related to auxiliary graphs discussed in Section~\ref{sec:auxiliarygraph}.
% % It implements set operations as linear scans of two sorted sets. 
% \spara{Data Graph}
% Before query execution, the data graph is loaded and its adjacency lists are sorted. The data graph is stored in compressed sparse row (CSR) format. For Dryadic, which is intended to support labeled graphs, we set all vertex labels to be the same label. 

% \spara{Managing Intermediate Results}
% To reduce memory allocation overhead, for each thread we use a memory pool to recycle and reuse the allocated memory for storing intermediate results and auxiliary graphs. We estimate the minimum memory required to build an auxiliary graph using the degrees of the adjacency lists in its selecting set. 

% \spara{Multi-threaded Implementation}
% For all systems for comparison, we use OpenMP (v4.5) to automatically parallelize the generated algorithms on the first loop.
% We use dynamic schedule with a chunk size of 1 for all experiments.
% We partition the top-level vertices into two sets based on their degrees. 
%The threshold can be adjusted at query execution time to allow fine-tuning. 
% We set the threshold to a fixed value of 4096 for all the experiments. 
% For top-level vertices with a degree below the threshold, we parallelize the execution of the first loop, that is, each thread handles one top-level vertex at a time. 
% For top-level vertices with degrees above the threshold, we parallelize the construction of the auxiliary graph in the first loop. 
% We also parallelize the computation of the second loop. 
% In both cases, we use OpenMP's dynamic schedule with a chunk size of 1 to parallelize the loop.

\begin{comment}
\vspace{.1in}\noindent\textbf{Distributed Implementation}
The distributed version of Minigraph statically partitions the top-level vertices among servers.
It approximates the cost of exploring each top-level vertex using its degree. 
%We sort the top-level vertices by degree and them to each server at a fixed step which is equal to the total number of compute nodes available. 
Each server then uses OpenMP to further parallelize its assigned top-level or second-level loop iterations across cores as described previously. We store the data graph in the local memory of each server. 
%We left further optimizations such as dynamic workload balancing as future work.
\end{comment}

==> sigmod-sections/7-Evaluation.tex <==
\section{Evaluation} 
\label{section:evaluation}
\subsection{Implementation}
We implement the Minigraph in C++ based on the implementation of Dryadic~\cite{Dryadic} and GraphPi~\cite{GraphPi}, which are the state-of-the-art compilation-based subgraph enumeration systems. Before we describe our implementation, we first compare the two systems to point out some potential improvements. 

\subsubsection{Comparing the State-of-the-Art Systems}
GraphPi~\cite{GraphPi} and Dryadic~\cite{Dryadic} varies in their implementation of the query scheduler and the query execution backend. 

Our evaluation shows that when the query schedules generated by the two systems are the same, Dryadic has a better performance due to its more efficient backend implementation. However, GraphPi can generate more efficient schedule, out-performing Dryadic when their schedules differ. 
Another difference is that Dryadic's backend supports both vertex-induced and edge-induced subgraph enumeration while GraphPi supports edge-induced patterns only. On the other hand, GraphPi implements optimizations for subgraph counting that Dryadic does not implement. 

We extend GraphPi~\cite{GraphPi} to support both vertex-induced and edge-induced subgraph enumeration using Dryadic's query execution backend. We also use this implementation as a baseline for comparison in this section besides the state-of-the-arts. 

\subsubsection{Minigraph Implementation}
We implement Minigraph on top of the baseline we described above with all the optimizations discussed in Section~\ref{section:background} as well as the techniques related to auxiliary graphs discussed in Section~\ref{sec:auxiliarygraph}. 

% The query scheduler takes as input a query graph and generates an optimal query schedule. The query schedule is consumed by Minigraph's code generator to produce efficient C++ code. 
% Besides our proposed dual-sort query scheduler, Minigraph also implements the state-of-the-art scheduler from GraphPi \cite{GraphPi}. 
% Note that the Minigraph code generator is designed to take an arbitrary schedule as an input. 
% It implements all the optimizations discussed in Section~\ref{section:background} as well as the techniques related to auxiliary graphs discussed in Section~\ref{sec:auxiliarygraph}.
% It implements set operations as linear scans of two sorted sets. 
\subsubsection{Data Graph}
Before query execution, the data graph is loaded and its adjacency lists are sorted. The data graph is stored in compressed sparse row (CSR) format. For Dryadic, which is intended to support labeled graphs, we set all vertex labels to be the same label during pre-processing. 

\subsubsection{Multi-threaded Implementation}
For all systems for comparison, we use OpenMP (v4.5) to automatically parallelize the generated algorithms on the first loop.
We use dynamic schedule with a chunk size of 1 for all experiments.

% Our evaluation shows that Minigraph can consistently outperform state-of-the-art, reaching up to one order of magnitude speedup.
% Its code generation time is negligible and its memory overhead is generally around a few megabytes.
\subsubsection{Memory Allocation}
To reduce memory allocation overhead, for each thread we use a memory pool to recycle and reuse the allocated memory for storing intermediate results and auxiliary graphs. Before building an auxiliary graph, we estimate the minimum memory required using the sum of degrees of the adjacency lists in its selecting set. Then, we allocate enough memory for storing all pruned adjacency lists. 

% This section evaluates the efficacy of Minigraph in subgraph enumerations. 
% Our evaluation shows that using Minigraph with the lazy strategy achieves speed up in most all cases and the code generation overhead of Minigraph is negligible when compared to the entire query execution time. 
% The lazy approach has the overall best performance reaching an order of magnitude in P3 YouTube and the extra memory consumption of Minigraph is a small fraction of the data graph. 
% \hui{if space allowed, it is nice to summarize the main evaluation results here}

\subsection{Experiment Settings}
\subsubsection{Data and Query Graphs}
We use six real-world data graphs from SNAP \cite{SNAP_datasets} in our evaluation. Their statistics are shown in Table \ref{graph-info}. 
%The Twitter graph is only used for memory consumption tests.
All the data graphs and auxiliary graphs are stored in the main memory during query execution. 
We treat all the graphs as undirected graphs. 
That is, if there is an edge $(v_i, v_j)$ in the data set, we assume $v_j \in N(v_i) \text{ and } v_i \in N(v_j)$. 

The query graphs we use in the evaluation are shown in Figure \ref{figure:patterns}.
They come from the benchmarks used in the evaluation of previous work~\cite{GraphPi, GraphZero, Dryadic}.
They are complex patterns meant to stress test the subgraph enumeration algorithms.

\input{tables/graph_info}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.75\linewidth]{sigmod-figures/queries.png}
    \captionof{figure}{Query Graph Patterns.}
    \label{figure:patterns}
\end{figure}

\subsubsection{Systems Used for Evaluation}
We directly compare Minigraph with two state-of-the-art systems Dryadic~\cite{Dryadic} and GraphPi~\cite{GraphPi} in three different settings: vertex-induced subgraph enumeration, edge-induced subgraph enumeration, and edge-induced subgraph counting. All these systems only report the number of matchings in the three settings.

\begin{comment}
\subsubsection{Systems used for evaluation} 
There is no publicly available state-of-the-art subgraph enumeration system available for direct comparison. 
GraphPi~\cite{GraphPi} is open-sourced, but its code generator targets edge-induced subgraph enumeration, a variant of the vertex-induced subgraph enumeration problem we target.
The definition of this problem is similar to the one in Section~
\ref{sec:problem-def} but in Eqn.~\ref{eqn:vertex-centric} the \emph{iff} condition is replaced by an \emph{if} condition.
The edge-induced variant produces different results for general query graphs.
%We can compare the two systems only for the case of cliques

GraphZero~\cite{GraphZero}  and AutoMine~\cite{AutoMine} are state-of-the-art systems that target vertex-induced subgraph enumeration. 
The code generator of GraphZero and AutoMine are very similar, except that AutoMine doesn't perform canonicality checks to prune the automorphisms, which makes AutoMine's query execution slower than GraphZero.  
However, we could not access the source code of either system. 

\vspace{.2cm}\noindent\textbf{Baseline} For the above reasons, we implemented a state-of-the-art system based on GraphZero as our baseline. 
We validated the performance of this baseline using published results and experiments, as we describe shortly.

The baseline adopts the open-sourced GraphPi's schedule and canonicality check to generate query schedules and implement basic, and prefix set optimizations for code generation.
%We compared GraphPi's schedules and GraphZero's schedules and found out GraphPi's schedules constantly outperform GraphZero's schedules.
Both optimizations are introduced in Section~\ref{section:background}.
Note that scheduling is orthogonal to our contribution.
The baseline's code generation does not use auxiliary graphs. 


The performance of our baseline is compatible with the GraphZero results reported in~\cite{FlexMiner}, which runs GraphZero on a system with a 10-core Intel i9-7900X CPU (3.30GHz, Turbo 4.3GHz, 13.75 MB LLC) with 64GB DRAM. 
It reports that GraphZero finishes a 5-clique query using 20 threads on Lj in 192 seconds.
We run our baseline implementation on our system with dual Intel(R) Xeon(R) Silver 4216 CPUs (2.10GHz, Turbo 3.20Ghz) and 128GB of RAM.
Our baseline finishes the same query on Lj in 198 seconds with 10 threads (Turbo enabled) using GraphZero's scheduler.
Despite using slower cores and fewer threads, we can get comparable performance.

We further compared our baseline with the original open-source GraphPi implementation in the special case of clique query patterns, for which both systems return the same results.
We considered cliques of size 3 to 5 and the Wiki, Patents, Lj, and Orkut graphs.
Our baseline implementation outperforms GraphPi by a factor of at least 2.1$\times$ and at most 5.2$\times$, depending on the graph and the query. 

\vspace{.2cm}\noindent\textbf{Minigraph} Minigraph is based on the same code base for set operations as the baseline. The difference is that Minigraph uses auxiliary graphs to accelerate query execution as discussed in Section~\ref{sec:codegeneration}. %Additionally, it uses the dual-sort query scheduler as discussed in Section~\ref{sec:dual-sort}. 
\end{comment}

\subsubsection{Evaluation Metrics}
We compare the following metrics: 
\begin{itemize}
    \item \emph{Query Execution Time} is the time spent executing the subgraph enumeration code given a query graph. We exclude the time to load the input graph into memory to show the direct effects of the auxiliary graphs on accelerating code efficiency.  For Minigraph, the query execution time always includes the construction time of auxiliary graphs, which takes place online during query execution. We ran all the experiments three times and reported the average. 
    % \item \textbf{Query scheduling time} is the time spent to derive the best query schedule.  
    \item \emph{Code Generation Time} is the time required for a code generator to produce the algorithm when a schedule is given.  
    \item \emph{Memory Consumption} is the extra memory required to store the auxiliary graphs in memory besides the data graph. We report the maximum memory overhead per thread of using auxiliary graphs since each thread can build its auxiliary graphs. 
\end{itemize}

\subsubsection{Hardware and Software Setup}
We run all single-server experiments on an AWS c6i.16xlarge instance, which is a server-class machine running Ubuntu 22.04 with 32 cores (64 threads) and 128 GB of RAM. 
The machine has one Intel(R) Xeon(R) Silver 8375C CPU (2.90GHz, Turbo 3.50Ghz). 
All tests use 64 CPU threads unless otherwise stated. 

All software is written in C++ and compiled with GCC 11.3 with -O3 optimization. 
We run all the experiments three times and report the average number.

\subsection{Query Execution Time}
\label{sec:query-execution-time} 
We compare the performance of Minigraph and the baseline systems. 
We discuss the performance comparison with a 64 threads setting. 
% The results under multi-thread and distributed settings are reported in Sections ~\ref{sec:multithread}.
% and ~\ref{sec:distributed}.  
\begin{figure*}
     \centering
    \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/patents.png}
         \caption{Patents}
         \label{patents}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/wiki.png}
         \caption{Wiki}
         \label{wiki}
     \end{subfigure}
    %  \hfill
    
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/pokec.png}
         \caption{Pokec}
         \label{pokec}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/youtube.png}
         \caption{YouTube}
         \label{youtube}
     \end{subfigure}
    \caption{Single thread experiments  where both the baseline and Minigraph use GraphPi's scheduler.}
    \label{fig:singlethread}
\end{figure*}

Figure~\ref{fig:singlethread} shows the query execution time of Minigraph and the baseline. The lazy approach achieves speedups in almost all cases, reaching 8.6 times for query $P3$ running on YouTube whereas the other two approaches exceed the baseline by over an order of magnitude.

\begin{figure*}[t]
     \centering
    \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/patents_P0_sum_log_curve_0.pdf}
         \caption{P1 on Patents at depth 1}
         \label{patents-p0-eager}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/patents_P0_sum_log_curve_1.pdf}
         \caption{P1 on Patents at depth 2}
         \label{patents-p0-lazy}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/patents_P0_sum_log_curve_2.pdf}
         \caption{P1 on Patents at depth 3}
         \label{patents-p0-online-lazy}
     \end{subfigure}
     \caption{Breakdown of the number of comparisons for P0 on Patents. In (a), the curve of the online lazy strategy is overlapped with the lazy strategy. The baseline has always zero comparisons.
     In (b), all variants of Minigraph have zero comparisons because of the auxiliary graph reuse optimization described in Section~\ref{sec:reuse}.}
     \begin{comment}
     X@Di means the \#operations at depth i using the X strategy\ms{we don't need to report the depth in the legend anymore, there is only one depth per plot}. Online means online lazy strategy. \ms{where is the baseline?}\jl{it is all zero, it doesn't do work at loop 1}. 
     \end{comment}
    \label{fig:patents-p0}
\end{figure*}

\begin{figure*}[t]
     \centering
    \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/wiki_P2_sum_log_curve_2.pdf}
         \caption{P6 on Wiki at depth 3}
         \label{wiki-p0-eager}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/wiki_P2_sum_log_curve_3.pdf}
         \caption{P6 on Wiki at depth 4}
         \label{wiki-p0-lazy}
     \end{subfigure}
    %  \hfill
     \begin{subfigure}[b]{0.32\linewidth}
         \centering
         \includegraphics[width=\linewidth]{figures/wiki_P2_sum_log_curve_4.pdf}
         \caption{P6 on Wiki at depth 5}
         \label{wiki-p0-online-lazy}
     \end{subfigure}
     \caption{Breakdown of the number of comparisons for P6 on Wiki}
    \label{fig:wiki-p0}
\end{figure*}
 
Specifically, the speedups increase when the query graphs take longer to process (i.e., query execution time is longer).
It is because executing a query with many vertices requires many nested loops.
The cost of pruning adjacency lists is paid at top-level loops and amortized when executing deeper loops.
Executing a large number of loops offers more opportunities to leverage existing auxiliary graphs and hence amortize their construction cost.
% 
For example, query $P0$ only has four vertices, which correspond to four loops in the query execution code.
In this case, Minigraph builds auxiliary graphs only in the first loop, which are used in the last loop where set operations occur.

Minigraph achieves a slowdown only for queries P0 and P1 on Patents.
Even if it performs no additional comparison compared to the baseline, Minigraph must execute some additional runtime logic to deal with auxiliary graphs, which results in a modest slowdown ($< 10\%$) in a few cases.
% For these reasons, the cost of building auxiliary graphs cannot be amortized on all graphs.
% However, we obtain speedups on all graphs for all other queries using pruning and our own scheduling method, with only the exception of YouTube and $P1$, where the running time slightly decreases.
% Overall, we observe that Minigraph always offers relative speedups for the slowest queries, which are the most critical to optimize in terms of absolute running time.

% Figure~\ref{fig:singlethread-2} shows the query execution time of Minigraph using the schedules generated by the Dual-Sort query scheduler. The Dual-Sort scheduler generates different schedules on $P4$ and $P6$. Thanks to the different schedules generated by Dual-Sort, Minigraph can run faster for $P6$ on Patents, Wiki, Pokec, and YouTube and is also quicker for $P4$ on Patents and Pokec. Yet, using the different schedules, it runs slower for $P4$ on YouTube and Wiki. Despite this slowdown, Minigraph still outperforms the baseline using GraphPi's schedules at least two times in these experiments. 
% For all other queries except $P4$ and $P6$, the Dual-Sort scheduler can produce the same schedules as GraphPi's scheduler without needing data-dependent graph statistics.
% In the second experiment, we use the GraphZero's model to generate the schedules and restrictions for each pattern query. We observe that both GraphPi and GraphZero generate the same schedules and restrictions for $P0$ and $P1$ for all the tested graphs. We omit these results in the table \ref{table:graphzero}, which contains the running time for $P2$, $P3$, $P4$, and $P5$ only. 
% Here, we observe that both the Baseline and Minigraph take longer to run given the same query and graph. Minigraph still outperforms the baseline method in $P4$. It has a relatively worse performance in $P2, P3$. For query $P5$ running on the graph YouTube, Minigraph is significantly slower than the baseline due to the schedule it uses. This is because Minigraph amplifies the influence of the schedule. The schedule impact the size of the prefix sets used to build the pruned graphs. As discussed in GraphPi \cite{GraphPi}, a fast schedule usually has small candidate sets (and prefix sets) in the upper loops, which reduce the number of vertices traversed in the future loops and hence reduce the number of set operations. Minigraph use the prefix sets in upper loops to build the pruned graph, so their sizes have a significant influence on Minigraph's the performance.

\subsection{Comparing Minigraph Variants}
To understand in detail the performance of different variants of Minigraph and the baseline, we measure the number of comparisons used in the set operations they perform.
Figures~\ref{fig:patents-p0} and~\ref{fig:wiki-p0} report the number of comparisons per vertex's adjacency list, summed over all vertices whose degree is in a given interval.
The operations are broken down based on the loop depth at which they occur.

The case of P0 on Patents is one where the eager approach is the least effective.
It performs many more comparisons than the baseline at upper loop depth to build the auxiliary graphs (see Figures~\ref{fig:patents-p0}(a)).
This excessive cost is not amortized later,  especially for lower-degree nodes that form the bulk of the graph and where pruning is less likely to be effective.
The eager approach has similar problems also with P2 on Wiki, as shown in Figure~\ref{fig:wiki-p0}(a).

The lazy strategy avoids this problem because it never performs extra comparisons.
In the cases shown in Figure~\ref{fig:patents-p0} and~\ref{fig:wiki-p0}, a lazy approach performs much less work at upper loop levels to build the auxiliary graphs, but it also performs more work at deeper loop levels.
In some cases like P2 on Wiki (see Figure~\ref{fig:wiki-p0}(c)), the lazy approach, however, misses opportunities for speedups.


The online lazy strategy represents a middle ground. It only prunes an adjacency list upon request, avoiding excessive computation overhead at higher loops. 
However, it might prune adjacency lists that are only used once. The associated computation could be cheaper if conducted in place. P0 on Patents is an example where the online lazy strategy performs more comparisons overall on small adjacency lists than the baseline (see Figure~\ref{fig:patents-p0}(a)).

In general, despite adding no analytical complexity, both lazy approaches require adding some extra logic to the query execution code, for example, to check at runtime whether a given adjacency list has been pruned.
This represents an additional overhead compared to the eager approach when the check can be done at compile-time.

% \subsection{Results on Query Scheduling Time}
% We compare the query scheduling time required by Minigraph and Baseline in table~\ref{tab:schedulingtime}. The baseline implements GraphPi's query schedule, which is the fastest baseline to compare with. 

% GraphPi's query schedule runs a cost model on all possible schedules to select the optimal. Computing the cost model can be expensive when the query graph is large. Although GraphPi optimizes its scheduler by pruning schedules before running the cost model, it still takes more than 2 seconds to compute the schedule for query $P6$, which has seven vertices.

% Minigraph only uses structural information to determine the schedule. 
% It only uses $30$ms to come up with a schedule for $P6$ thanks to its easy-to-compute \emph{score} function.  

% \begin{table}[ht]
% \centering
% \caption{Scheduling Time Comparision}
% \label{tab:schedulingtime}
% \resizebox{0.78 \columnwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|l|l|l|}
% \hline
% Time (ms)  & P0 & P1 & P2 & P3 & P4  & P5    & P6    \\ \hline
% GraphPi   & $<$1  & 40 & 60 & 40 & 160 & 2,090 & 2,800 \\ \hline
% Minigraph & $<$1  & 5  & 10 & 10 & 10  & 30    & 30    \\ \hline
% \end{tabular}%
% }
% \end{table}

\subsection{Results on Code Generation Time}
% Figure~\ref{fig:singlethread} only reports the running time of the query execution code, which takes a data graph as input and enumerates the matches. This is the last step of the workflow of a graph pattern matching system (see  Figure~\ref{figure:workflow}).

% To obtain the query execution code it is necessary to run a scheduling algorithm to find a query schedule and then generate the code.
% These are one-time costs that can often be amortized, since the generated code can be rerun multiple times, but it still needs to be reasonably low.

% To evaluate the running time of the preliminary steps to query execution, we measured the code generation and scheduling time for different queries.
% Table \ref{table:code_generation_time} shows the results.
% Both the baseline and Minigraph use GraphPi's query scheduler, so the scheduling time is the same in both cases and is reported only once.
% The results show that scheduling takes much longer than code generation, both for the baseline and for Minigraph.

Minigraph introduces extra overhead for code generation compared to the baseline because it needs to consider auxiliary graphs. However, Table~\ref{table:code_generation_time} shows that Minigraph's code generation is still orders of magnitude faster than query execution. 
\input{tables/experiments-code-generation}

% \subsection{Scalability}
% \label{sec:multithread}
% \subsubsection{Multi-threaded Scalability}
% % To evaluate the performance of Minigraph on multiple threads and its scalability, we consider the largest graph and the most complex query Minigraph can run within 48 hours using a single thread, which is graph Lj and query $P2$ respectively. 
% % We scale the number of threads up to 64, which is the maximum number of hyper-threading supported by our server, and measure the query execution time. 
% To evaluate the performance of Minigraph on multiple threads and its scalability, we run $P0, P1, P2$ on Lj and $P0, P1$ on Orkut. 
% %We disable Intel Turbo Boosting in our system and run all the experiments three times to report the average number. We turned off turbo boosting because it causes our CPUs' frequencies to change significantly using a different number of threads. 
% We use eager strategy for Minigraph in all the experiments.

% Minigraph and the baseline achieve significant speedup when using multiple threads, showing similar performance trends. 
% Minigraph still shows significantly shorter query execution time due to the auxiliary graph-based optimizations. 
% Specifically, the baseline and Minigraph scales similarly from 1 to 32 threads. Scaling above 32 threads gives diminishing returns because our hardware only has 32 physical cores.
% For $P2$ on Lj, the relative speedup of Minigraph is slightly lower than the baseline with 64 threads. However, its absolute running time is still significantly better: Minigraph takes 342 seconds to complete, a 4.9$\times$ speedup compared to the 1701 seconds required by the baseline. 

% \subsubsection{Distributed Scalability}
% \label{sec:distributed} 
% In distributed experiments, we evaluate the scalability of Minigraph to large graphs with billions of edges. We run $P2$ and $P3$ on Friendster, and the result is shown in Figure~\ref{Friendster}. For those queries, both baseline and Minigraph achieve near linear speed up scaling from 1 to 15 nodes. Minigraph outperforms the baseline 7.6 to 8.1 times on $P2$ and 5.2 to 5.7 times on $P3$.

% We also tested these queries on Orkut. For query $P2$ on Orkut, the baseline does not scale linearly from 4 to 15 nodes due to the unbalanced workload assigned to each node. Minigraph scales better even though it has the same set of top-level vertices assigned to each node. On $P2$, Minigraph outperforms the baseline 5.3 times using 4 nodes and 7.2 times using 15 nodes. On $P3$, both methods scale similarly from 1 to 15 nodes. Minigraph outperforms the baseline 4.6 times on 1 node and 4.1 times with 15 nodes. 

% \begin{figure*}
%      \centering
%     \begin{subfigure}[b]{0.24 \linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/lj-mt.png}
%          \caption{Lj multi-threaded}
%          \label{Lj-mt}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.24 \linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/orkut-mt.png}
%          \caption{Orkut multi-threaded}
%          \label{Orkut-mt}
%      \end{subfigure}
%     \begin{subfigure}[b]{0.24 \linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/orkut-mn.png}
%          \caption{Orkut distributed}
%          \label{Orkut}
%      \end{subfigure}
%      \begin{subfigure}[b]{0.24 \linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{figures/friendster-mn.png}
%          \caption{Friendster distributed}
%          \label{Friendster}
%      \end{subfigure}
%     \caption{Multi-thread and distributed experiments.}
%     \label{fig:multithread}
% \end{figure*}

% The reason for the lower speedups compared to the baseline is the additional data accesses required to proactively build the auxiliary graph  (see for example Algorithm~\ref{algorithms:Q1-Minigraph}, ln~\ref{ln:mini-start}-\ref{ln:mini-end}).

% We observed that Minigraph has a higher last-level cache miss rates than the baseline and it takes less advantage from the additional cache space  available when moving to the second CPU.
% When running query P2 on the Lj graph, for example, the last-level cache miss rates for Minigraph are 11.59\%, 6.45\%, and 7.98\% with 16, 32, and 64 threads respectively, compared to 8.97\%, 3.28\%, and 4.59\% for the baseline.
% This is due to the additional proactive data accesses required to build auxiliary graphs.
% The additional main-memory accesses due to cache misses are more expensive with two CPUs because they can incur NUMA overheads.
% Nonetheless, even if the relative speedups plateau between 16 and 32 threads, building auxiliary graphs allows Minigraph to perform less work, making Minigraph much faster than the baseline in terms of absolute running time. 


% Overall, \cache{} is more beneficial for complex queries taking longer time to execute. Here, the size of the graph is not the main factor of the complexity of the query. 
% Take the experiments for $P_3$ as an example, it takes the baseline 1.4 hours to run on the graph YouTube, but less than 0.84h (2995.4s) to run on the graph Pokec. Pokec has ten times the edges and 50 percent more vertices than YouTube, but it still takes longer time to run this query on YouTube. 
% This is true even after we switch to using GraphPi's schedule and restrictions, which speed up the baseline for 2.6x on Pokec and 3x on YouTube respectively. The reason for this discrepancy is the two graphs have different structural properties and distributions of the edges. The query time spend on the dense regions in the graph is significantly larger than the rest. Using \cache{} reduce the querying time spend on the dense regions, where the pruned adjacency lists can be used for multiple times which reduce the computation time significantly. In YouTube, using \cache{} along speedup the baseline for 2x, whereas it using with GraphPi's schedule and restrictions speed up the baseline for 15x. 

%\subsection{Distributed Scalability}
%\label{sec:distributed} 
% \begin{figure*}
%      \centering
%     \begin{subfigure}[b]{0.45 \linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{evaluation-figures/orkut_distributed.pdf}
%          \caption{Orkut}
%          \label{Orkut}
%      \end{subfigure}
%      \hfill 
%      \begin{subfigure}[b]{0.45 \linewidth}
%          \centering
%          \includegraphics[width=\linewidth]{evaluation-figures/friendster.pdf}
%          \caption{Friendster}
%          \label{Friendster}
%      \end{subfigure}
%     \caption{Distributed Experiments.}
%     \label{fig:distributed}
% \end{figure*}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/multinode_scalability.pdf}
%     \captionof{figure}{Multinodes scalability Test \jl{this will be updated to include the results from Orkut}}
%     \label{figure:multinode_scalability}
% \end{figure}

% \hg{update the content to include figure 6} \jl{updated}
% In the distributed scalability test, we statically assign the top level vertex to each node.
% We assume that the cost of each vertex is closely related to its
% degree. We sort the top-level vertices by degree and and assign to servers accordingly. Each server then uses OpenMP to further parallelize its assigned top-level loop iterations across cores. 
% This workload balancing strategy always assign the same top-level vertices to the same computation node. It has a fixed overhead for each node and is included in the figure. This overhead is pattern independent and only related to the data graph. The scheduling overhead is 0.5s for Orkut and 12s for Friendster. We include the overhead in the Figure~\ref{fig:distributed} and we report the longest time of the running nodes to finish the query.
% In distributed experiments, we evaluate the scalability of Minigraph to large graphs with billions of edges. We run $P2$ and $P3$ on Friendster, and the result is shown in Figure~\ref{Friendster}. For those queries, both baseline and Minigraph achieve near linear speed up scaling from 1 to 15 nodes. Minigraph outperforms the baseline 7.6 to 8.1 times on $P2$ and 5.2 to 5.7 times on $P3$.

% We also tested these queries on Orkut. For query $P2$ on Orkut, the baseline does not scale linearly from 4 to 15 nodes due to the unbalanced workload assigned to each node. Minigraph scales better even though it has the same set of top-level vertices assigned to each node. On $P2$, Minigraph outperforms the baseline 5.3 times using 4 nodes and 7.2 times using 15 nodes. On $P3$, both methods scale similarly from 1 to 15 nodes. Minigraph outperforms the baseline 4.6 times on 1 node and 4.1 times with 15 nodes. 
%Orkut is a more dense graph compared with Friendster. It has a higher average degree and max degree. 
% We observe that this scheduling strategy provides near linear speed up for P2, P3, and P4 on Friendster, P2 and P3 on Lj. It has a worse scalability for P4 on Lj due to unbalanced workload distribution. We also test the baseline using the same strategy on P2 for Lj, it has a less speedup when increasing the nodes from 8 to 15. We plan to solve this problem by implementing dynamic scheduling strategy. 
\input{tables/experiments-memory}
\subsection{Memory Consumption}
We now measure the memory overhead of materializing auxiliary graphs in Minigraph. We use the eager strategy for Minigraph in this experiment.
Table~\ref{table:memory} shows the memory requirement for storing each data graph and the peak memory requirement used by each thread for storing all its auxiliary graphs.
We measure peak memory requirement because Minigraph dynamically scales the memory usage based on the size and number of the pruned adjacency lists, starting from a small memory footprint.

Table~\ref{table:memory} shows that the memory consumption of the auxiliary graphs per thread is usually only a small fraction of the data graph, with the exception of the graph Twitter. 
The size of auxiliary graphs is not directly related to the size of the data graph itself but rather to the density of connections in the graph or part of the graph.  
Some graphs, like Patents or Pokec, only induce auxiliary graphs that are orders of magnitude smaller than the input graph, independent of the query graph. Other graphs show a larger variance. The memory consumption is per-thread because, in the current implementation of our system, we have each thread build auxiliary graphs independently for small degree root vertices. For root vertices with a large degree, we build the auxiliary graphs in the first loop in parallel using multiple threads and share them in the second loops by multiple threads. Since changing the threshold for the first loop and second loop parallelism will affect the result, we set the threshold to be greater than the maximum degree of the data graph when running this test, so we can get the maximum memory consumption result. 

The size of the auxiliary graph depends on many factors, including the connection density of the data graph, the pattern graph, and the schedule. We empirically observe that the memory consumption is correlated to the max degree of the graph for the graph we tested. Table~\ref{table:memory} shows the peak memory consumption per thread for the auxiliary graph on P0 with different data graphs. 
Notably, the peak memory consumption for the auxiliary graph is 0.6GB on Twitter. This is because there is a large densely-connected region in the data graph and the longest adjacency list has a size of six million. 

%The worst case is when the entire data graph is strongly connected, where the auxiliary graph will cache the entire data graph. However, using a bit matrix to store the auxiliary graph/original graph is preferred in this situation. We plan to investigate the techniques to reduce the memory consumption of auxiliary graphs for dense data graph by using binary or hybrid representation instead of simply integer vertex ids. 

==> sigmod-sections/8-Related.tex <==
\section{Related work}
% \hg{group topics together; use \paragraph{XX topic} at the front of each paragraph; goal: by reading the first sentence, you know what each paragraph is about. } 
Several frameworks \cite{Pregel, GraphX, Ligra} tackle general graph processing. 
These frameworks provide an extensible high-level task API while abstracting several low-level components such as scheduling, graph access, and parallelism. However, they are not well suited for graph mining problems such as motif counting and frequent subgraph mining. 
This has motivated the development of dedicated subgraph-centric graph mining frameworks \cite{Arabesque, RStream, Pangolin, Fractal, Peregrine, AutoMine, GraphZero, GraphPi}. 
Recent graph mining systems work uses subgraph query matching as a subroutine \cite{AutoMine, Peregrine}. 
They select the optimal schedules at query time and generate an optimized algorithm or binary to handle query matching. 
State-of-the-art systems use a code generation approach to improve performance further \cite{ AutoMine, GraphZero}. 
Minigraph advances this line of work by proposing a novel direction for performance optimization.
Throughout the paper, we extensively discuss the state-of-the-art to motivate our work and show that Minigraphs outperform it. 

This work considers \emph{subgraph enumeration} using unlabeled data graphs and queries.
Other prior work focuses on \emph{subgraph matching}, where graphs and queries are labeled.
For a recent survey and experimental evaluation of these algorithms, see~\cite{in-depth}.
RapidMatch is another more recent work in this area~\cite{rapidmatch}.
cuTS optimizes subgraph matching on GPUs~\cite{cuTS}. 
A key challenge in subgraph matching is leveraging labels to filter candidate vertices and find a good query schedule, which is not an issue in subgraph enumeration.
Auxiliary data structures are commonly used in subgraph matching \cite{GraphQL,BI,Han,in-depth,CECI,Turboiso,Versatile} and lead to significant speedups \cite{in-depth, Versatile}. 
However, these techniques rely on labels and are not designed for subgraph enumeration. 

This work considers main-memory graphs.
Other work considered algorithms for out-of-core graphs~\cite{DUALSIM}, or large graphs that are partitioned across servers~\cite{yang2021huge}.
Orthogonal optimizations include exploiting symmetry to reuse computation~\cite{ParallelSingleMachine}, or exploring output compression~\cite{cbf}. 
PBE-REUSE shares the results of set intersections across GPU threads by using a BFS matching strategy, which results in a much larger intermediate state than the more common backtracking DFS approach~\cite{guo2020exploiting}. 
None of these algorithms considered proactive online graph pruning,  which is introduced in this work.

Some work proposes accelerating set intersections by using a graph's binary representation and SIMD instructions in the CPUs \cite{EmptyHeaded, SIMD}. 
Some work proposes using specialized hardware to accelerate subgraph matching. FlexMiner \cite{FlexMiner} uses specialized hardware and on-chip memory to accelerate subgraph enumeration. DIMMining  \cite{DIMMining} is a more recent work that uses newly designed instruction sets and hardware to accelerate set operations in subgraph enumeration. Our work also aims to speed up set operations, but it does so by reducing the size of the input sets, independent of how the inputs are represented. These two approaches are complementary, and combining them is an interesting direction.

Graph databases are increasingly used in many applications and have proposed several techniques to optimize the query plan~\cite{GraphProcess,Demystify,EmptyHeaded,JoinProcessing,mhedhbi2019optimizing}.
Query optimization is an orthogonal problem in our work.
% Much work has focused on algorithms for subgraph isomorphism and subgraph enumeration, as for example \cite{Dualism, SubgraphMapReduce}. 

\section{Conclusion}
Subgraph enumeration is an important problem.
Auxiliary graphs represent a novel direction to reduce the running time of graph pattern mining algorithms.
It entails building a pruned representation of the data graph that can be used instead of the original graph to speed up query execution.
Auxiliary graphs are complementary to and can be combined with other state-of-the-art algorithms for query scheduling and code generation.
The Minigraph system shows that auxiliary graphs can speed up query execution time by up to $10\times$ with a low memory cost.
Generating query execution code with auxiliary graphs introduces a negligible compilation overhead.
Proactive graph pruning is a promising avenue to speed up subgraph enumeration and potentially other graph pattern matching problems.
% One promising direction is exploring a binary or compressed representation of the auxiliary graphs.
% New auxiliary graph materialization strategies may outperform our eager and lazy strategies.
% Combining auxiliary graphs with parallel query execution on GPUs is also a promising direction.

% the following is too detailed for future work
% In such a system, the CPU can be responsible for building auxiliary graphs at top levels, and the GPUs can use these auxiliary graphs to continue query execution. 
% The GPUs won't need to keep the entire data graph in memory; instead, they only need to keep the auxiliary graphs which are usually much smaller than the data graph.

==> sigmod-sections/backup/3-Overview-backup.tex <==
\section{Overview} \label{section:graphmini}
We first outline our criteria for pruning adjacency lists online and then its integration with existing compilation based algorithm.
The fundamental idea of Minigraph is to keep multiple compressed versions of the graph consisting of pruned adjacency lists, besides the input graph.
We call this data structure an auxiliary graph.
In this section, we discuss the criteria we use to build auxiliary graphs.
Section~\ref{section:methodology} then discusses how Minigraph applies these criteria for code generation.

Auxiliary graphs are built online during the execution of the backtracking algorithm which consists of a sequence of nested loops.
The fundamental purpose of auxiliary graphs is that \emph{an auxiliary graph built in a nested loop contains pruned adjacency lists that will be used as input for set operations in deeper nested loops.}
At each level of the nested loop, we use the information the algorithm has collected so far about partial matches to proactively build auxiliary graphs.

Using a minigraph requires answering two fundamental questions, which we address in the following:
\begin{enumerate}
    \item Which adjacency lists should be pruned and added to the auxiliary graph?
    \item How to prune these adjacency lists?
\end{enumerate}

\subsection{Properties of Prefix Sets}
Before introducing auxiliary graphs, we discuss some insights and useful properties of prefix sets, which were introduced in Section~\ref{section:prefix-optimization}.
We will leverage these properties to build auxiliary graphs.

First, we argue that \emph{each prefix set for a query vertex is a superset of the candidate set of that vertex}.
The purpose of prefix sets is to restrict the set of vertices that could be potentially matched to a query vertex.
Consider two prefix sets $C_h(v_i)$ and $C_{h+1}(v_i)$ computed at loop $h$ and loop $h+1$ respectively.
We know that $C_{h+1}(v_i)$ can be computed by subtracting $N(u_{h+1})$ from $C_h(v_i)$ or intersecting $C_h(v_i)$ with $N(u_{h+1})$ as shown in Eqns.~\ref{eqn:prefix_prefix_computation-1} and~\ref{eqn:prefix_prefix_computation-2}. 
In either case, the set operation only removes vertices from $C_h(v_i)$. 
Therefore, we have that the following holds:
\begin{equation} \label{lemma-1}
    C_{h+1}(v_i) \subseteq C_h(v_i) \qquad \forall h,i:\: h + 1 < i
\end{equation}
which implies that:
\begin{equation}
    C_f(v_i) \subseteq C_h(v_i) \qquad \forall h,i,f:\: h < f < i
    \label{lemma-2}
\end{equation} 

The candidate set $C(v_i)$ is equivalent to the prefix set $C_{i-1}(v_i)$ as shown by Eqns.~\ref{eqn:naive_candidate_computation} and~\ref{eqn:naive_prefix_computation}. 
Therefore, we have that:
\begin{equation}
    C(v_i) = C_{i-1}(v_i) \subseteq C_h(v_i) \qquad \forall h,i:\: h < i \label{eqn:superset_candidate}
\end{equation}
which amounts to say that each prefix set $C_h(v_i)$ is a superset of the candidate set $C(v_i)$.

% Consider the prefix set $C_h(v_i)$ computed at loop depth $h$ in the previous example.
% the prefix set $C(v_i)^{h}$ represents a \emph{superset} of the data vertices that will match future query vertices $v_i$ with $i > h$.
% In other words, for every partial match $[u_1, \ldots, u_i]$ obtained in the nested loops at depth greater than $h$, we know that $u_i \in C_h(v_i)$. Formally,
% This because $C(v_i)$ can be derived from $C_h(v_i)$ by intersecting and subtracting the adjacency lists of $[u_{h+1}, u_{h+2}, \ldots, u_{i-1}]$ according to equation \ref{eqn:naive_candidate_computation} and \ref{eqn:naive_prefix_computation}. Since both set intersection and set subtraction only remove vertices from $C_h(v_i)$ , the final result must be a subset of $C_h(v_i)$.
% For the same reason, a query vertex $v_i$'s prefix set computed at a deeper loop is a subset of its prefix set computed at an upper loop. Formally,
% \begin{equation}
%     C(v_i)^f \subseteq C_h(v_i) \:\: (i > f > h) \label{eqn:superset_prefix}
% \end{equation}

Second, the prefix set $C_h(v_i)$ is actually the \emph{minimal superset of $C(v_i)$ that can be computed based on the partial match available at loop $h$}. 
% Formally, we have that:
% \begin{gather}
%     \not\exists S \subseteq C_h(v_i): \: S = f(I_n) \text{ and } C(v_i) \subseteq S
%     \label{eqn:minimal}
% \end{gather}
% where $f$ is a combination 
The loop at depth $h$ operates on the partial match $I_h = [u_1, \ldots, u_h]$.
The prefix set $C_h(v_i)$ is the result of executing \emph{all} the set operations involving the adjacency lists $N(u_i)$ for all the vertices in $I_h$, that is, with $i \in[1,h]$.
Any prefix set $C_j(v_i)$ with $j > h$ is obtained by performing set operations between $C_{j-1}(v_i)$ and $N(v_j)$ (see Eqn.~\ref{eqn:prefix_prefix_computation-1} and~\ref{eqn:prefix_prefix_computation-2}). 
Therefore, $C_h(v_i)$ is minimal at loop $h$ because to further remove any vertex from the prefix set, we need to consider the adjacency lists of other vertices which will only be matched in deeper loops. 

\subsection{Selecting Adjacency Lists for the Minigraph}
As discussed previously, the purpose of a minigraph built at loop depth $h$ is to prune the adjacency lists used as input for set operations at loop depths greater than $h$.
Let $v_k$ be a query vertex matched in a deeper loop than $h$, with $k > h$.
Suppose that we want to build an auxiliary graph to speed up the construction of the candidate set $C(v_k)$ in deeper nested loops.
We want to prune and add adjacency lists which will be used in later set operations to compute $C(v_k)$.
How can we identify these adjacency lists?

To answer this question we need to consider operations executed at three different depths of the nested loop indexed as shown in Table~\ref{table:depths}.
We call $h$ the depth of the loop where we want to build a pruned adjacency list to be added to the minigraph, and $k$ the deeper loop where we iterate over the candidate set $C(v_k)$.
The other indices are related to the way we perform pruning and will be described in the following. 
Otherwise, we will use the same notation as in Section~\ref{section:background} (see Table~\ref{table:terminologies}).

To obtain $C(v_k)$, we need to compute the set operations among the adjacency lists of vertices in the partial match $I_{k-1}=[u_1, \ldots, u_{k-1}]$, as shown in Eqn.~\ref{eqn:prefix_prefix_computation-1} and~\ref{eqn:prefix_prefix_computation-2}.
To speed up those set operations, we could prune the adjacency lists of the vertices in $I_{k-1}$.
Remember that we are considering building an auxiliary graph at loop depth $h$ to speed up set operations of the nested loops with a depth greater than $h$.
At loop depth $h$, we have only matched the vertices in $I_h=[u_1, \ldots, u_h]$.
%We can only prune the adjacency lists of vertices in $I_h$ because the remaining vertices $[u_{h+1}, \ldots, u_k]$ are still unknown.

Unfortunately, pruning the adjacency lists of the vertices in $I_h$ at loop $h$ would not speed up the computation of $C(v_k)$ in deeper nested loops.
At loop $h$ we can compute the prefix set $C_h(v_k)$, which is a superset of $C(v_k)$ as shown in Eqn.~\ref{eqn:superset_candidate}.
Because of the minimality property of prefix sets following from Eqn.~\ref{eqn:naive_prefix_computation}, we know that $C_h(v_k)$ already incorporates the results of all set operations involving the adjacency lists of the vertices $[u_1, \ldots, u_h]$.
Pruning the adjacency lists of those vertices would not help to compute the candidate set $C(v_k)$.

Pruning can speed up set operations at loop depth greater than $h$ only if applied to the adjacency lists $N(u_i)$ with $u_i \in [u_{h+1}, \ldots, u_{k-1}]$.
Before we discuss how to prune $N(u_i)$ we need to find $u_i$ in the first place.
The vertex $u_i$ is a match to a query vertex $v_i$, but the matching only occurs at a deeper loop level than $h$, the current level. 
The candidate set $C(v_i)$ contains all vertices $u_i$ to be matched to $v_i$, but we don't have that set available at loop $h$. 
However, we know that the prefix set $C_h(v_i)$ is a superset of $C_{i-1}(v_k)$ because of Eqn.~\ref{eqn:superset_candidate}.
Therefore, the Minigraph adopts the following criterion to build minigraphs:
\begin{criterion}
At nested loop depth $h$, Minigraph prunes the adjacency lists $N(u)$ for each $u \in C_h(v_i)$.
\label{crit-1}
\end{criterion}

\input{tables/loops}


\subsection{How to prune the adjacency lists?}
Now that we have established which adjacency lists to prune at loop depth $h$, we can discuss how to prune these lists.
As we will argue, we prune adjacency lists differently for different query vertices $v_k$ that we will match next.
Given an adjacency list $N(u_i)$, we call $N^h_k(u_i)$ the version of the adjacency list pruned at loop depth $h$ in order to find matches of $v_k$ more efficiently.

When using prefix sets, the set operations on the adjacency list $N(u_i)$ are computed at loop depth $i$.
The prefix set $C_i(v_k)$ is computed using either a set intersection (see Eqn.~\ref{eqn:prefix_prefix_computation-1}) or a set subtraction (see Eqn.~\ref{eqn:prefix_prefix_computation-2}), depending on whether $v_k$ is a neighbor of $v_i$ or not.

Consider first the case where $(v_i, v_j) \in E_q$ and we must compute $C_i(v_k) = C_{i-1}(v_k) \cap N(u_i)$ according to Eqn.~\ref{eqn:prefix_prefix_computation-1}.
How can we prune $N(u_i)$ to speed up this set operation while still preserving correctness?

By Eqn.~\ref{eqn:naive_prefix_computation}, each prefix set $C_j(v_k)$ with $j < i$ is a superset of $C_{i-1}(v_k)$.
In particular, since we are currently at loop depth $h$, we have $C_h(v_k)$ and we know that $C_{i-1}(v_k) \subseteq C_h(v_k)$.

Let $N^h_{k,i}(u_i)$ be a set of data vertices computed as follows:
\begin{equation}
    N^h_{k,i}(u_i) = C_h(v_k) \cap N(u_i)
    \label{eq:intersect}    
\end{equation}
We call the set $N^h_{k,i}(u_i)$ a \emph{pruned adjacency list} of $N(u_i)$ since $N^h_{k,i}(u_i) \subseteq N(u_i)$.
We can use this pruned adjacency to compute $C_i(v_k)$ as follows:
\begin{equation}
    C_i(v_k) = C_{i-1}(v_k) \cap N^h_{k,i}(u_i) \quad \text{if} \quad (v_i, v_j) \in E_q
    \label{eqn:pruned-intersect}
\end{equation}

We now argue that replacing Eqn.~\ref{eqn:prefix_prefix_computation-1} with Eqn.~\ref{eqn:pruned-intersect} leads to the same value of $C_i(v_k)$.

\begin{lemma}
    It holds that $C_{i-1}(v_k) \cap N(u_i) = C_{i-1}(v_k) \cap N^h_{k,i}(u_i)$ for each $h<i<k$.
    \label{lemma-3}
\end{lemma}
\begin{proof}
\noindent
The pruned adjacency list $N^h_{k,i}(u_i)$ is defined as $C_h(v_k) \cap N(u_i)$ in Eqn.~\ref{eq:intersect}.
Therefore, we need to prove that $C_{i-1}(v_k) \cap N(u_i) = C_{i-1}(v_k) \cap C_h(v_k) \cap N(u_i)$.
Since $h < i < k$, it follows from Eqn.~\ref{lemma-2} that $C_{i-1}(v_k) \subseteq C_h(v_k)$, so $C_{i-1}(v_k)=C_{i-1}(v_k) \cap C_h(v_k)$.
\end{proof}

%This equation is correct since $C_{i-1}(v_k) \subseteq C_h(v_k)$ (see Figure \ref{figure:A_B}).

The Minigraph code generator can thus add the pruned adjacency list $N^h_{k,i}(u_i)$ to the auxiliary graph and use it later to reduce the cost of computing set operations at loop depth $i > h$.
Instead of using Eqn.~\ref{eqn:prefix_prefix_computation-1}, we can replace $N(u_i)$ with a smaller pruned adjacency list $N^h_{k,i}(u_i)$.

A similar argument holds for the case where $(v_i, v_j) \notin E_q$ and we must compute $C_i(v_k) = C_{i-1}(v_k) - N(u_i)$ according to Eqn.~\ref{eqn:prefix_prefix_computation-2}.
In this case, we can also compute $N^h_{k,i}(u_i)$ as:
\begin{equation}
    N^h_{k,i}(u_i) = C_h(v_k) \cap N(u_i)
    \label{eq:subtract}    
\end{equation}
and $C_i(v_k)$ as:
\begin{equation}
    C_i(v_k) = C_{i-1}(v_k) - N^h_{k,i}(u_i) \quad \text{if} \quad (v_i, v_j) \notin E_q
    \label{eqn:pruned-subtract}
\end{equation}

We can now replace Eqn.~\ref{eqn:prefix_prefix_computation-2} with Eqn.~\ref{eqn:pruned-subtract} and obtain the same value of $C_i(v_k)$.
The correctness argument is analogous to Lemma~\ref{lemma-3} and can be proved similarly.

\begin{lemma}
    It holds that $C_{i-1}(v_k) - N(u_i) = C_{i-1}(v_k) - N^h_{k,i}(u_i)$ for each $h<i<k$.
    \label{lemma-4}
\end{lemma}

As discussed previously, at loop depth $h$ we don't know the exact set of vertices $u_i$ for which we need to prune $N(u_i)$.
However, we know that these vertices are included in the prefix set $C_h(v_i)$.
According to Criterion~\ref{crit-1}, GraphMini computes a pruned adjacency list $N^h_{k,i}(u)$ of $N(u)$ for each $u \in C_h(v_i)$ at loop depth $h$.
We now have two more criteria for using minigraphs:
\begin{criterion}
GraphMini computes the pruned adjacency list $N^h_{k,i}(u)$ at loop depth level $h$ for each $i,k$ such that $h<i<k$ using Eqn.~\ref{eq:intersect} or~\ref{eq:subtract}. \label{crit-2}
\end{criterion}
\begin{criterion}
GraphMini replaces Eqn.~\ref{eqn:prefix_prefix_computation-1} with Eqn.~\ref{eqn:pruned-intersect} and Eqn.~\ref{eqn:prefix_prefix_computation-2} with Eqn.~\ref{eqn:pruned-subtract} when computing prefix sets $C_j(v_k)$ at all loop levels with depth $j \in [i,k)$. \label{crit-3}
\end{criterion}

% \subsection{Pruning Adjacency Lists With Set Intersection} \label{section:set-property}
% We use a property of sets to prune the adjacency lists. 
% \begin{lemma}
%     \label{eqn:set_property}
%     If $A \subseteq A^*$ and  $T = A^* \cap B$ then:  
%     \begin{gather}
%         A \cap B = A \cap T  \notag \\
%         A - B = A - T 
%     \end{gather}
% \end{lemma}

% \begin{minipage}{\columnwidth}
%     \includegraphics[width=0.9\linewidth]{figures/A_B.pdf}
%     \captionof{figure}{Set Intersection \& Set Subtraction}
%     \label{figure:A_B}
% \end{minipage}

% %\begin{minipage}{\columnwidth}
% %    \includegraphics[width=0.9\linewidth]{figures/A_subtract_B.pdf}
% %    \captionof{figure}{Set Subtraction}
% %    \label{figure:A_minus_B}
% %\end{minipage}

% Here, $T$ is a subset of $B$ as any element in $T$ must also in $B$. Since $T$ is a subset of $B$, computing set operations between $A$ with $T$ can be less expensive compared to computing set operation between $A$ and $B$.

% In the context of adjacency lists pruning:
% \begin{itemize}
%     \item $A$ corresponds the prefix set of $C(v_k)^{i-1}$
%     \item $A^*$ corresponds to $C(v_k)^h$
%     \item $B$ corresponds the original adjacency list $N(u_i)$
%     \item $T$ corresponds the pruned adjacency list $N_{k, i}^h(u_i)$
% \end{itemize}


% \spara{How to store minigraphs?}
% We have discussed how GraphMini prunes at loop depth $h$ the adjacency lists of vertices matched at lower loop depths.
% When GraphMini builds a minigraph at loop depth $h$, it uses it for all deeper nested loops.
% It then discards that minigraph at the next iteration at depth $h$ and rebuilds a new minigraph.

% A minigraph is the union of the adjacency lists computed at that depth. 
% More specifically, a minigraph $M^h$ computed at loop depth $h$ is the union of all pruned adjacency lists $N^h_{k,i}(u)$ for each $k,i$ such that $h < i < k$ and for each $u \in C_h(v_i)$.

% Minigraphs are built incrementally based on the minigraph of the current outer loop.
% For example, the minigraphs at loop depth $h$ are built based on the minigraph at loop depth $h-1$.
% Specifically, suppose that we need to compute $N^h_{k,i}(u)$ using Eqn.~\ref{eq:intersect}.
% The minigraph in the outer loop contains a pruned adjacency list $N^{h-1}_{k,i}(u)$ for $N(u)$.
% Therefore, we can now compute $N^h_{k,i}(u)$ as:
% $$
% N^h_{k,i}(u) = C_h(v_k) \cap N^{h-1}_{k,i}(u)
% $$

% The minigraph for the outer loop must have an entry $N^{h-1}_{k,i}(u)$ for vertex $v$.
% In fact, a minigraph at depth $h$ has pruned adjacency lists for each $u \in C_h(v_k)$ and we know that $C_h(v_k) \in S^{h-1}_k$.

==> sigmod-sections/backup/old-4.tex <==
% =================== OLD =====================
% =================== OLD =====================
% =================== OLD =====================
% =================== OLD =====================
% =================== OLD =====================
% =================== OLD =====================
\section{Auxiliary Graphs - OLD} \label{section:minigraph}
%We first outline our criteria for pruning adjacency lists online and then its integration with the prefix set optimizations. 
Our Minigraph system keeps multiple compressed versions of the input graph consisting of pruned adjacency lists. 
We call this data structure an \emph{auxiliary graph}. 
Auxiliary graphs are built online during the execution of the backtracking algorithm, which consists of a sequence of nested loops.
The fundamental idea is to \emph{build an auxiliary graph in a nested loop and then use its pruned adjacency lists as input to set operations in deeper nested loops.}
At each level of the nested loop, we use the information the algorithm has collected about partial matches to build auxiliary graphs proactively.

This section discusses the criteria we use to build auxiliary graphs.
Section~\ref{section:methodology} then discusses how our Minigraph system uses these criteria to generate code.
We now discuss three fundamental questions that arise when using an auxiliary graph:
\begin{enumerate}
    \item Which adjacency lists should be pruned and added to an auxiliary graph?
    \item How to prune these adjacency lists?
\end{enumerate}



\subsection{Properties of Prefix Sets}
Before introducing auxiliary graphs, we discuss some insights and valuable properties of prefix sets introduced in section ~\ref{section:prefix-optimization}.
We will leverage these properties to build auxiliary graphs.

First, we argue that \emph{each prefix set for a query vertex is a superset of the candidate set of that vertex}.
The purpose of prefix sets is to restrict the set of vertices that could be potentially matched to a query vertex.
Consider two prefix sets $C_h(v_i)$ and $C_{h+1}(v_i)$ computed at loop $h$ and $h+1$ respectively.
The set $C_{h+1}(v_i)$ can be computed by subtracting $N(u_{h+1})$ from $C_h(v_i)$ or intersecting $C_h(v_i)$ with $N(u_{h+1})$ as shown in Eqns.~\ref{eqn:prefix_prefix_computation-1} and~\ref{eqn:prefix_prefix_computation-2}. 
In either case, the set operation only adds a subset of the vertices of $C_h(v_i)$ into $C_{h+1}(v_i)$. 
Therefore, we have that:
\begin{equation} \label{lemma-1}
    C_{h+1}(v_i) \subseteq C_h(v_i) \qquad \forall h,i:\: h + 1 < i
\end{equation}
which implies that:
\begin{equation}
    C_f(v_i) \subseteq C_h(v_i) \qquad \forall h,i,f:\: h < f < i
    \label{lemma-2}
\end{equation} 

The candidate set $C(v_i)$ is equivalent to the prefix set $C_{i-1}(v_i)$ as shown by Eqns.~\ref{eqn:naive_candidate_computation} and~\ref{eqn:naive_prefix_computation}. 
Therefore, we have that:
\begin{equation}
    C(v_i) = C_{i-1}(v_i) \subseteq C_h(v_i) \qquad \forall h,i:\: h < i \label{eqn:superset_candidate}
\end{equation}
which amounts to saying that each prefix set $C_h(v_i)$ is a superset of the candidate set $C(v_i)$.

% Consider the prefix set $C_h(v_i)$ computed at loop depth $h$ in the previous example.
% the prefix set $C(v_i)^{h}$ represents a \emph{superset} of the data vertices that will match future query vertices $v_i$ with $i > h$.
% In other words, for every partial match $[u_1, \ldots, u_i]$ obtained in the nested loops at depth greater than $h$, we know that $u_i \in C_h(v_i)$. Formally,
% This because $C(v_i)$ can be derived from $C_h(v_i)$ by intersecting and subtracting the adjacency lists of $[u_{h+1}, u_{h+2}, \ldots, u_{i-1}]$ according to equation \ref{eqn:naive_candidate_computation} and \ref{eqn:naive_prefix_computation}. Since both set intersection and set subtraction only remove vertices from $C_h(v_i)$ , the final result must be a subset of $C_h(v_i)$.
% For the same reason, a query vertex $v_i$'s prefix set computed at a deeper loop is a subset of its prefix set computed at an upper loop. Formally,
% \begin{equation}
%     C(v_i)^f \subseteq C_h(v_i) \:\: (i > f > h) \label{eqn:superset_prefix}
% \end{equation}

Second, by definition, the prefix set $C_h(v_i)$ is actually the \emph{minimal superset of $C(v_i)$ that can be computed based on the partial match available at loop $h$}. 
By minimal, we mean that to remove any vertex from the prefix set it is necessary to consider the adjacency lists of other vertices that will only be matched in deeper loops. 
% Formally, we have that:
% \begin{gather}
%     \not\exists S \subseteq C_h(v_i): \: S = f(I_n) \text{ and } C(v_i) \subseteq S
%     \label{eqn:minimal}
% \end{gather}
% where $f$ is a combination 
The loop at depth $h$ operates on the partial match $I_h = [u_1, \ldots, u_h]$.
The prefix set $C_h(v_i)$ is the result of executing \emph{all} the set operations involving the adjacency lists $N(u_i)$ for all the vertices in $I_h$, that is, with $i \in[1,h]$.
Any prefix set $C_h(v_i)$ with $j > h$ is obtained by performing set operations between $C_{h-1}(v_i)$ and $N(v_h)$ (see Eqn.~\ref{eqn:prefix_prefix_computation-1} and~\ref{eqn:prefix_prefix_computation-2}). 

\subsection{Selecting Adjacency Lists for Pruning}
As discussed previously, the purpose of an auxiliary graph built at loop depth $h$ is to prune the adjacency lists used as input for set operations at loop depths greater than $h$.
Let $v_k$ be a query vertex matched in a deeper loop than $h$, with $k > h$.
Suppose we want to build an auxiliary graph to speed up the construction of the candidate set $C(v_k)$ in deeper nested loops.
We want to prune and add adjacency lists which will be used in later set operations to compute $C(v_k)$.
How can we identify these adjacency lists?

To answer this question, we need to consider operations executed at three different depths of the nested loop, which are indexed as shown in Table~\ref{notations}.
We call $h$ the depth of the loop where we want to build a pruned adjacency list to be added to the auxiliary graph, and $k$ the deeper loop where we iterate over the candidate set $C(v_k)$.
The other indices are related to the way we perform pruning and will be described in the following. 
%Otherwise, we will use the same notation as in Table~\ref{notations}.

To obtain $C(v_k)$, we need to compute the set operations among the adjacency lists of vertices in the partial match $I_{k-1}$, as shown in Eqn.~\ref{eqn:prefix_prefix_computation-1} and~\ref{eqn:prefix_prefix_computation-2}.
To speed up those set operations, we could prune the adjacency lists of the vertices in $I_{k-1}$.
Remember that we are considering building an auxiliary graph at loop depth $h$ to speed up set operations of the nested loops with a depth greater than $h$.
At loop depth $h$, we have only matched the vertices in $I_h=[u_1, \ldots, u_h]$.
%We can only prune the adjacency lists of vertices in $I_h$ because the remaining vertices $[u_{h+1}, \ldots, u_k]$ are still unknown.

Unfortunately, pruning the adjacency lists of the vertices in $I_h$ at loop $h$ would not speed up the computation of $C(v_k)$ in deeper nested loops.
At loop $h$ we can compute the prefix set $C_h(v_k)$, which is a superset of $C(v_k)$ as shown in Eqn.~\ref{eqn:superset_candidate}.
Because of the minimality property of prefix sets following from Eqn.~\ref{eqn:naive_prefix_computation}, we know that $C_h(v_k)$ already incorporates the results of all set operations involving the adjacency lists of the vertices $[u_1, \ldots, u_h]$.
Pruning the adjacency lists of those vertices would not help to compute the candidate set $C(v_k)$.

Pruning can speed up set operations at loop depth greater than $h$ only if applied to the adjacency lists $N(u_i)$ with $u_i \in [u_{h+1}, \ldots, u_{k-1}]$.
Before we discuss how to prune $N(u_i)$, we need to find $u_i$ in the first place.
The vertex $u_i$ is a match to a query vertex $v_i$, but the matching only occurs at a deeper loop level than $h$, the current level. 
The candidate set $C(v_i)$ contains all vertices $u_i$ to be matched to $v_i$, but we don't have that set available at loop $h$. 
However, we know that the prefix set $C_h(v_i)$ is a superset of $C_{i-1}(v_k)$ because of Eqn.~\ref{eqn:superset_candidate}.
Therefore, the Minigraph adopts the following criterion to build auxiliary graphs:
\begin{criterion}
At nested loop depth $h$, Minigraph prunes the adjacency lists $N(u)$ for each $u \in C_h(v_i)$.
\label{crit-1}
\end{criterion}

\subsection{Pruning Adjacency Lists}
Now that we have established which adjacency lists to prune at loop depth $h$, we can discuss how to prune these lists.
As we will argue, we prune adjacency lists differently for different query vertices $v_k$ that we will match next.
Given an adjacency list $N(u_i)$, we call $N^k_h(u_i)$ the version of the adjacency list pruned at loop depth $h$ in order to find matches of $v_k$ more efficiently.

When using prefix sets, the set operations on the adjacency list $N(u_i)$ are computed at loop depth $i$.
The prefix set $C_i(v_k)$ is computed using either a set intersection (see Eqn.~\ref{eqn:prefix_prefix_computation-1}) or a set subtraction (see Eqn.~\ref{eqn:prefix_prefix_computation-2}), depending on whether $v_k$ is a neighbor of $v_i$ or not.

Consider first the case where $(v_i, v_h) \in E_q$ and we must compute $C_i(v_k) = C_{i-1}(v_k) \cap N(u_i)$ according to Eqn.~\ref{eqn:prefix_prefix_computation-1}.
How can we prune $N(u_i)$ to speed up this set operation while still preserving correctness?
Our method is based on a fundamental property of sets. Formally:
\begin{lemma}
    \label{eqn:set_property}
    If $A \subseteq A^*$ and  $T = A^* \cap B$ then:  
    \begin{gather}
        A \cap B = A \cap T  \notag \\
        A - B = A - T 
    \end{gather}
\end{lemma}
We will discuss how we use this lemma to analyze the candidate sets and its prefix sets and associated adjacency lists in this section. 


By Eqn.~\ref{eqn:naive_prefix_computation}, each prefix set $C_h(v_k)$ with $j < i$ is a superset of $C_{i-1}(v_k)$.
In particular, since we are currently at loop depth $h$, we have $C_h(v_k)$ and we know that $C_{i-1}(v_k) \subseteq C_h(v_k)$.

Let $N^k_h(u_i)$ be a set of data vertices computed as follows:
\begin{equation}
    N^k_h(u_i) = C_h(v_k) \cap N(u_i)
    \label{eq:intersect}    
\end{equation}
We call the set $N^k_h(u_i)$ a \emph{pruned adjacency list} of $N(u_i)$ since $N^k_h(u_i) \subseteq N(u_i)$.
We can use this pruned adjacency to compute $C_i(v_k)$ as follows:
\begin{equation}
    C_i(v_k) = C_{i-1}(v_k) \cap N^k_h(u_i) \quad \text{if} \quad (v_i, v_h) \in E_q
    \label{eqn:pruned-intersect}
\end{equation}

We now argue that replacing Eqn.~\ref{eqn:prefix_prefix_computation-1} with Eqn.~\ref{eqn:pruned-intersect} leads to the same value of $C_i(v_k)$.

\begin{lemma}
    It holds that $C_{i-1}(v_k) \cap N(u_i) = C_{i-1}(v_k) \cap N^k_h(u_i)$ for each $h<i<k$.
    \label{lemma-3}
\end{lemma}
\begin{proof}
\noindent
The pruned adjacency list $N^k_h(u_i)$ is defined as $C_h(v_k) \cap N(u_i)$ in Eqn.~\ref{eq:intersect}.
Therefore, we need to prove that $C_{i-1}(v_k) \cap N(u_i) = C_{i-1}(v_k) \cap C_h(v_k) \cap N(u_i)$.
Since $h < i < k$, it follows from Eqn.~\ref{lemma-2} that $C_{i-1}(v_k) \subseteq C_h(v_k)$, so $C_{i-1}(v_k)=C_{i-1}(v_k) \cap C_h(v_k)$.
\end{proof}

%This equation is correct since $C_{i-1}(v_k) \subseteq C_h(v_k)$ (see Figure \ref{figure:A_B}).

The Minigraph code generator can thus add the pruned adjacency list $N^k_h(u_i)$ to the auxiliary graph and use it later to reduce the cost of computing set operations at loop depth $i > h$.
Instead of using Eqn.~\ref{eqn:prefix_prefix_computation-1}, we can replace $N(u_i)$ with a smaller pruned adjacency list $N^k_h(u_i)$.

A similar argument holds for the case where $(v_i, v_h) \notin E_q$ and we must compute $C_i(v_k) = C_{i-1}(v_k) - N(u_i)$ according to Eqn.~\ref{eqn:prefix_prefix_computation-2}.
In this case, we can also compute $N^k_h(u_i)$ as:
\begin{equation}
    N^k_h(u_i) = C_h(v_k) \cap N(u_i)
    \label{eq:subtract}    
\end{equation}
and $C_i(v_k)$ as:
\begin{equation}
    C_i(v_k) = C_{i-1}(v_k) - N^k_h(u_i) \quad \text{if} \quad (v_i, v_h) \notin E_q
    \label{eqn:pruned-subtract}
\end{equation}

We can now replace Eqn.~\ref{eqn:prefix_prefix_computation-2} with Eqn.~\ref{eqn:pruned-subtract} and obtain the same value of $C_i(v_k)$.
The correctness argument is analogous to Lemma~\ref{lemma-3} and can be proved similarly.

\begin{lemma}
    It holds that $C_{i-1}(v_k) - N(u_i) = C_{i-1}(v_k) - N^k_h(u_i)$ for each $h<i<k$.
    \label{lemma-4}
\end{lemma}

As discussed previously, at loop depth $h$, we don't know the exact set of vertices $u_i$ for which we need to prune $N(u_i)$.
However, we know that these vertices are included in the prefix set $C_h(v_i)$.
According to Criterion~\ref{crit-1}, Minigraph computes a pruned adjacency list $N^k_h(u)$ of $N(u)$ for each $u \in C_h(v_i)$.
We now have two more criteria for using auxiliary graphs:
\begin{criterion}
Minigraph computes the pruned adjacency list \\ $N^k_h(u_i)$ at loop depth level $h$ for each $i,k$ such that $h<i<k$ using Eqn.~\ref{eq:intersect} or~\ref{eq:subtract}. \label{crit-2}
\end{criterion}
\begin{criterion}
Minigraph replaces Eqn.~\ref{eqn:prefix_prefix_computation-1} with Eqn.~\ref{eqn:pruned-intersect} and Eqn.~\ref{eqn:prefix_prefix_computation-2} with Eqn.~\ref{eqn:pruned-subtract} when computing prefix sets $C_h(v_k)$ at all loop levels with depth $j \in [i,k)$. \label{crit-3}
\end{criterion}


==> sigmod-sections/scheduler.tex <==
\section{Dual-Sort Query Scheduler}
\label{sec:dual-sort}
Given a query graph, Minigraph's query scheduler aims to identify the best query schedule that can minimize the cardinality of the candidate sets and maximize the use of the auxiliary graphs. 
We call Minigraph's algorithm ``Dual-Sort" because the same function is used to rank matching orders and also the resulting sets of canonicality checks to eliminate automorphisms.

% explain why we need to develop a new query scheduler 
\subsubsection{Motivation}
Existing query schedulers in state-of-the-art subgraph enumeration systems ~\cite{GraphZero, GraphPi} suffer from two limitations. First, they use rank schedules using cost models that don't consider our auxiliary graph optimizations. Second, their cost model also uses statistics from the data graph as its input.
When processing a new graph or an updated version of a previously-processed graph, these systems will need to calculate these statistics, which can be expensive and add up to the runtime overhead. 

Minigraph's query scheduler addresses these two shortcomings. 
It leverages the structural information of the query pattern to make the most out of using auxiliary graphs. 
Furthermore, it doesn't require statistics from the data graph.
We can therefore generate code to serve a query once and run it on different data graphs as-is.

\subsubsection{Ranking Matching Orders}
The Minigraph scheduler is motivated by the empirical observation that real-world graphs tend to be sparse.
As the number of adjacency lists we intersect grows, the size of the result set decreases quickly.
We use this observation to design our scheduler. We iteratively schedule as next query vertex to match the one that has the most edges with the query vertices that have been matched already. 
We further refine this criterion by prioritizing a query vertex if it has edges to the earliest possible matched query vertices in the scheduling order.
This is because we can materialize a prefix set for that query vertex at an upper loop.
The materialized prefix sets can then be used to build auxiliary graphs in that loop to speed up the construction of the candidate sets at a deeper loop. 

We design our Dual-Sort query scheduler as follows.
The query scheduler enumerates all the possible schedules for a query $q$ and ranks them based on the following auxiliary graph-aware cost model. 
The cost model first assigns a score to each query vertex and then ranks schedules based on the scores of the query vertices, giving higher priority to the score of a query vertex that is matched earlier in the order.

Given a matching order $\phi$, we use $N^{\phi}_{-}(v_i)$ to denote the backward neighbors of $v_i$ such that:
$$v_j \in N^{\phi}_{-}(v_i) \iff j < i \textit{ and } (v_j, v_i) \in E(q).$$
Namely, $N^{\phi}_{-}(v_i)$ contains all the query vertices connected to $v_i$ that have been matched before matching $v_i$. We then compute a score for $v_i$, which is defined as follows:
\begin{equation} \label{score}
    Score(v_i) = \sum_{v_j \in N^{\phi}_{-}(v_i)} 2 ^{ |V(q)| - j}
\end{equation}
The rationale for this scoring function is the following.
At the $i^{th}$ position in the matching order, we aim to match a query vertex that leads to the smallest candidate set to iterate through in the next loop. The data vertices in the candidate set $C(v_i)$ must be the common neighbors of all the data vertices matched to the query vertices in $N^{\phi}_{-}(v_i)$. 
Therefore, we favor a $v_i$ with a large set of $v_j \in N^{\phi}_{-}(v_i)$ whose adjacency lists must be intersected.
We also want to materialize the prefix sets of $C(v_i)$ as early as possible, allowing the algorithm to build auxiliary graphs having it as the selecting-set or the filtering-set. The score function does that by giving $v_i$ a higher score if it is connected to $v_j$ with a small value for $j$, meaning that it is matched at an upper loop level.

Given a matching order, Eqn.~\ref{score} assigns a score to each of its vertices.
The algorithm then ranks different matching orders using lexicographic ordering: first, it ranks based on the score of $v_1$, then if there are ties it considers the score of $v_2$, and so on.
We use the matching order with the highest score to generate the algorithm. 

\subsubsection{Ranking Alternative Sets of Canonicality Checks}
After selecting a matching order, we need to select an associated set of canonicality checks to prune automorphisms.
We use GraphPi's algorithm to generate multiple alternative sets of canonicality checks given a matching order. 
To select a specific set of canonicality checks, we use a ranking function similar to the one used to select a matching order.
We build a graph for each set of canonicality checks, where a canonicality check between two query vertices $v_j, v_i$ is represented as an undirected edge between $v_j$ and $v_i$. Then, we use the same score function of Eqn.~\ref{score} and ranking criteria as discussed previously. The intuition is a canonicality check between $v_j$ and $v_i$ filters the candidate set of $C(v_i)$ by removing the data vertices larger (or smaller) than $u_j$ from it at runtime. We aim to apply this filtering as early as possible for each prefix set, which helps our algorithm to reduce the overhead of building auxiliary graphs using the prefix set. Using the same score function allows us to achieve this goal efficiently. 


==> tables/experiment_data.tex <==
\begin{table}
    \caption{Execution Time for Different Patterns (s)}
    \begin{tabular}{|c|c|c|c|}  \hline
    Patern        & amazon    & youtube  &  lj  \\ \hline
    Automine P1& 0.06      & 0.8      &  51   \\
    Mini-Graph P1 & 0.06      & 0.7      &  37   \\
    Automine P2          & 0.6       & 1072     &  34022   \\
    Mini-Graph P2          & 1.0       & 341      &  10028   \\
    Automine P3          & 0.7       & 1055     &  >48h   \\
    Mini-Graph P3          & 0.8       & 348      &  >48h   \\
    Automine P4          & 1.4       & 11557    &  >48h   \\
    Mini-Graph P4          & 1.8       & 2695     &  >48h   \\
    Automine P5          & 0.9       & 4410     &  >48h   \\
    Mini-Graph P5          & 1.0       & 2010     &  >48h   \\\hline
    \end{tabular}
    \label{exp_data}
\end{table}

==> tables/experiments-code-generation.tex <==
\begin{table}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Pattern}        & \textit{$P_1$} & \textit{$P_2$} & \textit{$P_3$} & \textit{$P_4$} & \textit{$P_5$} & \textit{$P_6$} & \textit{$P_7$} & \textit{$P_8$} \\ \hline
\textit{$T_{base}$}     & 0.3s           & 0.3s           & 0.3s           & 0.3s           & 0.4s           & 0.6s           & 0.6s           & 0.5s           \\ \hline
\textit{$T_{Online+N}$} & 0.9s           & 1.0s           & 1.2s           & 0.8s           & 1.3s           & 1.3s           & 1.2s           & 1.3s           \\ \hline
\end{tabular}
\caption{Code generation time}
\label{tab:code_gen}
\end{table}

==> tables/experiments-graphpi-bk.tex <==
\begin{table*}[t]
\centering
\begin{tabular}{cccccccccc}
\hline
\multicolumn{1}{|c|}{\textbf{Pattern}} & \multicolumn{3}{c|}{\textbf{P0}}                                                                                          & \multicolumn{3}{c|}{\textbf{P1}}                                                                                          & \multicolumn{3}{c|}{\textbf{P2}}                                                                                          \\ \hline
\multicolumn{1}{|c|}{\textit{Graph}}   & \multicolumn{1}{c|}{\textit{Baseline}} & \multicolumn{1}{c|}{\textit{GraphMini}} & \multicolumn{1}{c|}{\textit{Speed Up}} & \multicolumn{1}{c|}{\textit{Baseline}} & \multicolumn{1}{c|}{\textit{GraphMini}} & \multicolumn{1}{c|}{\textit{Speed Up}} & \multicolumn{1}{c|}{\textit{Baseline}} & \multicolumn{1}{c|}{\textit{GraphMini}} & \multicolumn{1}{c|}{\textit{Speed Up}} \\ \hline \hline
\multicolumn{1}{|c|}{Wiki}             & \multicolumn{1}{c|}{0.7s}              & \multicolumn{1}{c|}{0.5s}               & \multicolumn{1}{c|}{1.4x}              & \multicolumn{1}{c|}{0.4s}              & \multicolumn{1}{c|}{0.2s}               & \multicolumn{1}{c|}{2.0x}              & \multicolumn{1}{c|}{157s}              & \multicolumn{1}{c|}{40.9s}              & \multicolumn{1}{c|}{3.8x}              \\ \hline
\multicolumn{1}{|c|}{Patents}          & \multicolumn{1}{c|}{6.8s}              & \multicolumn{1}{c|}{10.5s}              & \multicolumn{1}{c|}{0.6x}              & \multicolumn{1}{c|}{2.5s}              & \multicolumn{1}{c|}{2.7s}               & \multicolumn{1}{c|}{0.9x}              & \multicolumn{1}{c|}{36.1s}             & \multicolumn{1}{c|}{24.2s}              & \multicolumn{1}{c|}{1.5x}              \\ \hline
\multicolumn{1}{|c|}{YouTube}          & \multicolumn{1}{c|}{6.5s}              & \multicolumn{1}{c|}{7.0s}               & \multicolumn{1}{c|}{0.9x}              & \multicolumn{1}{c|}{1.2s}              & \multicolumn{1}{c|}{0.9s}               & \multicolumn{1}{c|}{1.3x}              & \multicolumn{1}{c|}{1,701s}            & \multicolumn{1}{c|}{311s}               & \multicolumn{1}{c|}{5.4x}              \\ \hline
\multicolumn{1}{|c|}{Pokec}            & \multicolumn{1}{c|}{33.5s}             & \multicolumn{1}{c|}{42.1s}              & \multicolumn{1}{c|}{0.8x}              & \multicolumn{1}{c|}{11.9s}             & \multicolumn{1}{c|}{9.7s}               & \multicolumn{1}{c|}{1.2x}              & \multicolumn{1}{c|}{965s}              & \multicolumn{1}{c|}{355s}               & \multicolumn{1}{c|}{2.7x}              \\ \hline
\multicolumn{1}{|c|}{Lj}               & \multicolumn{1}{c|}{273s}              & \multicolumn{1}{c|}{221s}               & \multicolumn{1}{c|}{1.2x}              & \multicolumn{1}{c|}{1,395s}            & \multicolumn{1}{c|}{741s}               & \multicolumn{1}{c|}{1.9x}              & \multicolumn{1}{c|}{64,578s}           & \multicolumn{1}{c|}{10,121}             & \multicolumn{1}{c|}{6.4x}     \\ \hline
\multicolumn{1}{|c|}{Orkut}            & \multicolumn{1}{c|}{1,737s}            & \multicolumn{1}{c|}{954s}               & \multicolumn{1}{c|}{1.8x}     & \multicolumn{1}{c|}{1,071s}            & \multicolumn{1}{c|}{379}                & \multicolumn{1}{c|}{2.7x}     & \multicolumn{1}{c|}{OT}                & \multicolumn{1}{c|}{OT}                 & \multicolumn{1}{c|}{OT}                \\ \hline
\multicolumn{10}{l}{}                                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\multicolumn{1}{|c|}{\textbf{Pattern}} & \multicolumn{3}{c|}{\textbf{P3}}                                                                                          & \multicolumn{3}{c|}{\textbf{P4}}                                                                                          & \multicolumn{3}{c|}{\textbf{P5}}                                                                                          \\ \hline
\multicolumn{1}{|c|}{\textit{Graph}}   & \multicolumn{1}{c|}{\textit{Baseline}} & \multicolumn{1}{c|}{\textit{GraphMini}} & \multicolumn{1}{c|}{\textit{Speed Up}} & \multicolumn{1}{c|}{\textit{Baseline}} & \multicolumn{1}{c|}{\textit{GraphMini}} & \multicolumn{1}{c|}{\textit{Speed Up}} & \multicolumn{1}{c|}{\textit{Baseline}} & \multicolumn{1}{c|}{\textit{GraphMini}} & \multicolumn{1}{c|}{\textit{Speed Up}} \\ \hline \hline
\multicolumn{1}{|c|}{Wiki}             & \multicolumn{1}{c|}{175s}              & \multicolumn{1}{c|}{41.8s}              & \multicolumn{1}{c|}{4.2x}              & \multicolumn{1}{c|}{838s}              & \multicolumn{1}{c|}{124s}               & \multicolumn{1}{c|}{6.7x}     & \multicolumn{1}{c|}{1,188s}            & \multicolumn{1}{c|}{264s}               & \multicolumn{1}{c|}{4.5x}              \\ \hline
\multicolumn{1}{|c|}{Patents}          & \multicolumn{1}{c|}{35.1s}             & \multicolumn{1}{c|}{22.4s}              & \multicolumn{1}{c|}{1.5x}              & \multicolumn{1}{c|}{186s}              & \multicolumn{1}{c|}{114s}               & \multicolumn{1}{c|}{1.6x}              & \multicolumn{1}{c|}{74.5s}             & \multicolumn{1}{c|}{37.5s}              & \multicolumn{1}{c|}{2.0x}              \\ \hline
\multicolumn{1}{|c|}{YouTube}          & \multicolumn{1}{c|}{1,571s}            & \multicolumn{1}{c|}{155s}               & \multicolumn{1}{c|}{10.1x}    & \multicolumn{1}{c|}{29,838s}           & \multicolumn{1}{c|}{4,620s}             & \multicolumn{1}{c|}{6.4x}              & \multicolumn{1}{c|}{7,809s}            & \multicolumn{1}{c|}{1,076s}             & \multicolumn{1}{c|}{7.5x}     \\ \hline
\multicolumn{1}{|c|}{Pokec}            & \multicolumn{1}{c|}{1,019s}            & \multicolumn{1}{c|}{312s}               & \multicolumn{1}{c|}{3.2x}              & \multicolumn{1}{c|}{10,447s}           & \multicolumn{1}{c|}{2,618s}             & \multicolumn{1}{c|}{4.0x}              & \multicolumn{1}{c|}{4,389s}            & \multicolumn{1}{c|}{1,121s}             & \multicolumn{1}{c|}{3.9x}              \\ \hline
\multicolumn{1}{|c|}{Lj}            & 
\multicolumn{1}{c|}{OT}            & \multicolumn{1}{c|}{OT}               & \multicolumn{1}{c|}{OT}              & \multicolumn{1}{c|}{OT}           & \multicolumn{1}{c|}{OT}             & \multicolumn{1}{c|}{OT}              & \multicolumn{1}{c|}{OT}            & \multicolumn{1}{c|}{OT}             & \multicolumn{1}{c|}{OT}              \\ \hline
\multicolumn{1}{|c|}{Orkut}            & 
\multicolumn{1}{c|}{OT}            & \multicolumn{1}{c|}{OT}               & \multicolumn{1}{c|}{OT}              & \multicolumn{1}{c|}{OT}           & \multicolumn{1}{c|}{OT}             & \multicolumn{1}{c|}{OT}              & \multicolumn{1}{c|}{OT}            & \multicolumn{1}{c|}{OT}             & \multicolumn{1}{c|}{OT}              \\ \hline
\end{tabular}
\caption{Comparison of Query Execution Time - Single Thread \ms{add P6}}
\label{table:graphpi}
\end{table*}

==> tables/experiments-graphpi.tex <==
\begin{table*}[]
\centering
\begin{tabular}{ccccccccccccc}
\cline{2-11}
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{\textbf{Pattern}} & \multicolumn{3}{c|}{\textbf{P0}}                                                                               & \multicolumn{3}{c|}{\textbf{P1}}                                                                               & \multicolumn{3}{c|}{\textbf{P2}}                                                                               &                                  &                                     \\ \cline{2-11}
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{\textit{Graph}}   & \multicolumn{1}{c|}{\textit{Base}} & \multicolumn{1}{c|}{\textit{Gm}}    & \multicolumn{1}{c|}{\textit{Base/Gm}} & \multicolumn{1}{c|}{\textit{Base}} & \multicolumn{1}{c|}{\textit{Gm}}    & \multicolumn{1}{c|}{\textit{Base/Gm}} & \multicolumn{1}{c|}{\textit{Base}} & \multicolumn{1}{c|}{\textit{Gm}}    & \multicolumn{1}{c|}{\textit{Base/Gm}} &                                  &                                     \\ \cline{2-11}
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{Wiki}             & \multicolumn{1}{c|}{0.7s}          & \multicolumn{1}{c|}{0.5s}           & \multicolumn{1}{c|}{1.4x}           & \multicolumn{1}{c|}{0.4s}          & \multicolumn{1}{c|}{0.2s}           & \multicolumn{1}{c|}{2.0x}           & \multicolumn{1}{c|}{157s}          & \multicolumn{1}{c|}{40.9s}          & \multicolumn{1}{c|}{3.8x}           &                                  &                                     \\ \cline{2-11}
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{Patents}          & \multicolumn{1}{c|}{6.8s}          & \multicolumn{1}{c|}{10.5s}          & \multicolumn{1}{c|}{0.6x}           & \multicolumn{1}{c|}{2.5s}          & \multicolumn{1}{c|}{2.7s}           & \multicolumn{1}{c|}{0.9x}           & \multicolumn{1}{c|}{36.1s}         & \multicolumn{1}{c|}{24.2s}          & \multicolumn{1}{c|}{1.5x}           &                                  &                                     \\ \cline{2-11}
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{YouTube}          & \multicolumn{1}{c|}{6.5s}          & \multicolumn{1}{c|}{7.0s}           & \multicolumn{1}{c|}{0.9x}           & \multicolumn{1}{c|}{1.2s}          & \multicolumn{1}{c|}{0.9s}           & \multicolumn{1}{c|}{1.3x}           & \multicolumn{1}{c|}{1,701s}        & \multicolumn{1}{c|}{311s}           & \multicolumn{1}{c|}{5.4x}           &                                  &                                     \\ \cline{2-11}
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{Pokec}            & \multicolumn{1}{c|}{33.5s}         & \multicolumn{1}{c|}{42.1s}          & \multicolumn{1}{c|}{0.8x}           & \multicolumn{1}{c|}{11.9s}         & \multicolumn{1}{c|}{9.7s}           & \multicolumn{1}{c|}{1.2x}           & \multicolumn{1}{c|}{965s}          & \multicolumn{1}{c|}{355s}           & \multicolumn{1}{c|}{2.7x}           &                                  &                                     \\ \cline{2-11}
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{Lj}               & \multicolumn{1}{c|}{273s}          & \multicolumn{1}{c|}{221s}           & \multicolumn{1}{c|}{1.2x}           & \multicolumn{1}{c|}{1,395s}        & \multicolumn{1}{c|}{741s}           & \multicolumn{1}{c|}{1.9x}           & \multicolumn{1}{c|}{17.9hrs}       & \multicolumn{1}{c|}{2.8hrs}         & \multicolumn{1}{c|}{6.4x}           &                                  &                                     \\ \cline{2-11}
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{Orkut}            & \multicolumn{1}{c|}{1,737s}        & \multicolumn{1}{c|}{954s}           & \multicolumn{1}{c|}{1.8x}           & \multicolumn{1}{c|}{1,071s}        & \multicolumn{1}{c|}{379s}           & \multicolumn{1}{c|}{2.7x}           & \multicolumn{1}{c|}{OT}            & \multicolumn{1}{c|}{OT}             & \multicolumn{1}{c|}{N/A}            &                                  &                                     \\ \cline{2-11}
\multicolumn{1}{c|}{}                  & \multicolumn{1}{c|}{Friendster}       & \multicolumn{1}{c|}{4.4hrs}        & \multicolumn{1}{c|}{4.0hrs}         & \multicolumn{1}{c|}{1.1x}           & \multicolumn{1}{c|}{5,655s}        & \multicolumn{1}{c|}{3,256s}         & \multicolumn{1}{c|}{1.7x}           & \multicolumn{1}{c|}{OT}            & \multicolumn{1}{c|}{OT}             & \multicolumn{1}{c|}{N/A}            &                                  &                                     \\ \cline{2-11}
                                       &                                       &                                    &                                     &                                     &                                    &                                     &                                     &                                    &                                     &                                     &                                  &                                     \\ \hline
\multicolumn{1}{|c|}{\textbf{Pattern}} & \multicolumn{3}{c|}{\textbf{P3}}                                                                                 & \multicolumn{3}{c|}{\textbf{P4}}                                                                               & \multicolumn{3}{c|}{\textbf{P5}}                                                                               & \multicolumn{3}{c|}{\textbf{P6}}                                                                             \\ \hline
\multicolumn{1}{|c|}{\textit{Graph}}   & \multicolumn{1}{c|}{\textit{Base}}    & \multicolumn{1}{c|}{\textit{Gm}}   & \multicolumn{1}{c|}{\textit{Base/Gm}} & \multicolumn{1}{c|}{\textit{Base}}  & \multicolumn{1}{c|}{\textit{Gm}}   & \multicolumn{1}{c|}{\textit{Base/Gm}} & \multicolumn{1}{c|}{\textit{Base}}  & \multicolumn{1}{c|}{\textit{Gm}}   & \multicolumn{1}{c|}{\textit{Base/Gm}} & \multicolumn{1}{c|}{\textit{Base}}  & \multicolumn{1}{c|}{\textit{Gm}} & \multicolumn{1}{c|}{\textit{Base/Gm}} \\ \hline
\multicolumn{1}{|c|}{Wiki}             & \multicolumn{1}{c|}{175s}             & \multicolumn{1}{c|}{41.8s}         & \multicolumn{1}{c|}{4.2x}           & \multicolumn{1}{c|}{838s}           & \multicolumn{1}{c|}{124s}          & \multicolumn{1}{c|}{6.7x}           & \multicolumn{1}{c|}{1,188s}         & \multicolumn{1}{c|}{264s}          & \multicolumn{1}{c|}{4.5x}           & \multicolumn{1}{c|}{523s}           & \multicolumn{1}{c|}{226s}        & \multicolumn{1}{c|}{2.3x}           \\ \hline
\multicolumn{1}{|c|}{Patents}          & \multicolumn{1}{c|}{35.1s}            & \multicolumn{1}{c|}{22.4s}         & \multicolumn{1}{c|}{1.5x}           & \multicolumn{1}{c|}{186s}           & \multicolumn{1}{c|}{114s}          & \multicolumn{1}{c|}{1.6x}           & \multicolumn{1}{c|}{74.5s}          & \multicolumn{1}{c|}{37.5s}         & \multicolumn{1}{c|}{2.0x}           & \multicolumn{1}{c|}{26.0s}          & \multicolumn{1}{c|}{21.7s}       & \multicolumn{1}{c|}{1.2x}           \\ \hline
\multicolumn{1}{|c|}{YouTube}          & \multicolumn{1}{c|}{1,571s}           & \multicolumn{1}{c|}{155s}          & \multicolumn{1}{c|}{10.1x}          & \multicolumn{1}{c|}{8.3hrs}         & \multicolumn{1}{c|}{1.3hrs}        & \multicolumn{1}{c|}{6.4x}           & \multicolumn{1}{c|}{7,809s}         & \multicolumn{1}{c|}{1,076s}        & \multicolumn{1}{c|}{7.5x}           & \multicolumn{1}{c|}{4,579s}         & \multicolumn{1}{c|}{2,518s}      & \multicolumn{1}{c|}{1.8x}           \\ \hline
\multicolumn{1}{|c|}{Pokec}            & \multicolumn{1}{c|}{1,019s}           & \multicolumn{1}{c|}{312s}          & \multicolumn{1}{c|}{3.2x}           & \multicolumn{1}{c|}{2.9hrs}         & \multicolumn{1}{c|}{0.7hr}         & \multicolumn{1}{c|}{4.0x}           & \multicolumn{1}{c|}{4,389s}         & \multicolumn{1}{c|}{1,121s}        & \multicolumn{1}{c|}{3.9x}           & \multicolumn{1}{c|}{1,603s}         & \multicolumn{1}{c|}{849s}        & \multicolumn{1}{c|}{1.8x}           \\ \hline
\end{tabular}
\caption{Comparison of Query Execution Time - Single Thread}
\label{table:graphpi}
\end{table*}

==> tables/experiments-graphzero.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{|c|ccc|ccc|ccc|ccc|}
\hline
Patterns & \multicolumn{3}{c|}{\textit{\textbf{P2}}}                                                  & \multicolumn{3}{c|}{\textit{\textbf{P3}}}                                                  & \multicolumn{3}{c|}{\textit{\textbf{P4}}}                                                  & \multicolumn{3}{c|}{\textit{\textbf{P5}}}                                                        \\ \hline
Graph    & \multicolumn{1}{c|}{\textit{Base}} & \multicolumn{1}{c|}{\textit{Our}} & \textit{Speed Up} & \multicolumn{1}{c|}{\textit{Base}} & \multicolumn{1}{c|}{\textit{Our}} & \textit{Speed Up} & \multicolumn{1}{c|}{\textit{Base}} & \multicolumn{1}{c|}{\textit{Our}} & \textit{Speed Up} & \multicolumn{1}{c|}{\textit{Base}} & \multicolumn{1}{c|}{\textit{Our}}       & \textit{Speed Up} \\ \hline
Wiki     & \multicolumn{1}{c|}{189s}          & \multicolumn{1}{c|}{96.0s}        & \textbf{2.0x}     & \multicolumn{1}{c|}{397s}          & \multicolumn{1}{c|}{183s}         & \textbf{2.2x}     & \multicolumn{1}{c|}{886s}          & \multicolumn{1}{c|}{283s}         & 3.1x              & \multicolumn{1}{c|}{4,309s}        & \multicolumn{1}{c|}{2,869s}             & 1.5x              \\ \hline
Patents  & \multicolumn{1}{c|}{58.8s}         & \multicolumn{1}{c|}{95.3s}        & 0.6x              & \multicolumn{1}{c|}{85.8s}         & \multicolumn{1}{c|}{101s}         & 0.8x              & \multicolumn{1}{c|}{142s}          & \multicolumn{1}{c|}{92s}          & 1.5x              & \multicolumn{1}{c|}{1,102s}        & \multicolumn{1}{c|}{387s}               & \textbf{2.8x}     \\ \hline
YouTube  & \multicolumn{1}{c|}{2,537s}        & \multicolumn{1}{c|}{7,063s}       & 0.4x              & \multicolumn{1}{c|}{5,277s}        & \multicolumn{1}{c|}{9,615s}       & 0.5x              & \multicolumn{1}{c|}{55,937s}       & \multicolumn{1}{c|}{10,789s}      & \textbf{5.2x}     & \multicolumn{1}{c|}{87,481s}       & \multicolumn{1}{c|}{\textgreater{}100h} & \textless{}0.2x   \\ \hline
Pokec    & \multicolumn{1}{c|}{1,652s}        & \multicolumn{1}{c|}{4,456s}       & 0.4x              & \multicolumn{1}{c|}{3,161s}        & \multicolumn{1}{c|}{5,787s}       & 0.5x              & \multicolumn{1}{c|}{17,300s}       & \multicolumn{1}{c|}{5,268s}       & 3.3x              & \multicolumn{1}{c|}{-}             & \multicolumn{1}{c|}{-}                  & -                 \\ \hline
\end{tabular}
\caption{Experiment Evaluation Using GraphZero's Schedules}
\label{table:graphzero}
\end{table*}

==> tables/loops.tex <==
\begin{table}[t]
\centering
\begin{tabular}{|c|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Depth}} & \multicolumn{1}{c|}{\textbf{Description}}        \\ \hline
$h$                           & Loop where we prune the adjacency list $N(u_i)$. \\ \hline
$i$                           & Loop where we match the query vertex $v_i$ with $u_i$.            \\ \hline
%$j$                           & Loop where we use $N(u_j)$ and to compute the prefix set $S^j_k$.\\ \hline
$k$                         & Loop where we match the query vertex $v_k$.\\ \hline
\end{tabular}
\caption{Indices for loop depths, with $h <i < k$.}
\label{table:depths}
\end{table}

==> tables/terms.tex <==
\begin{table}[t]
\centering
\begin{tabular}{|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Term}} & \multicolumn{1}{c|}{\textbf{Description}}        \\ \hline
$G(V, E)$                           & The data graph.                                  \\ \hline
$G_q(V_q, \: E_q)$                  & The query graph.                                 \\ \hline
$G_s(V_s, \: E_s)$                  & A subgraph of the data graph.                    \\ \hline
$v_i$                               & The $i^{th}$ query vertex in the matching order ($v_i \in V_q$).       \\ \hline
%$u_i$                               & A data vertex matching to $v_i$ ($u_i \in V$ ). \\ \hline
$N(d)$                            & The adjacency list of a data vertex $d\in V$.                     \\ \hline
$S_i$                               & The candidate vertices that can match to $v_i$.  \\ \hline
$S^j_i$                             & The prefix set for $S_i$ at loop depth $j$.  \\ \hline
\end{tabular}
\caption{Notation}
\label{table:terminologies}
\end{table}

==> tables/triangles.tex <==
\begin{table}[!htbp]
    \begin{tabular}{|c|c|c|c|}  \hline
          Graph      & Triangles & V scanned      & Time (ms) \\ \hline
          wiki-input & 60k       & 6.9M           & 34              \\
          youtube    & 3.0M      & 129M           & 516             \\
          patents    & 7.5M      & 158M           & 2099            \\
          pokec      & 32.5M	 & 905M           & 6566            \\
        %   lj         & 4.0M      & 34.7M         \\
        %   orkut      & 3.1M      & 117.2M        \\ 
          \hline
    \end{tabular}
    \caption{Triangle Counting}
    \label{table:tri_counting}
\end{table}
